Diverse Why-Provenance for Datalog Queries

Datalog is a powerful rule-based language that allows us to express complex recursive queries and has found numerous applications over the years. Explaining why a result to a Datalog query is obtained is an essential task towards explainable and transparent data-intensive applications that rely on Datalog. A standard way of explaining a query result is the so-called why-provenance, which provides information about the witnesses to a query result in the form of subsets of the input database that as a whole can be used to derive that result. The state-of-the-art approach for efficiently computing the why-provenance explanations of a certain query result aims at enumerating, without repetitions, the relevant explanations by relying on off-the-shelf SAT solvers. However, whenever the set of explanations is very large, outputting the entire set might be prohibitively expensive. Moreover, it is questionable the practical usefulness of flooding the user with a very large number of explanations, many of them possibly differing only marginally. In this case, one can argue that it would be practically more useful to compute a small, sufficiently diverse subset of the set of why-provenance explanations. The present work initiates the study of the latter problem. In particular, we formalize the problem of interest as an optimization problem, and, after showing that it is highly intractable (it is NP-hard even in data complexity), we investigate whether ILP optimization solvers can be employed towards practical solutions. Our main finding is that this is achievable as long as we keep the requested set of explanations small, or we employ approximation algorithms (with error guarantees).

==> experiments.tex <==
\section{Experiments}

We now proceed to experimentally evaluate the SAT-based framework for computing diverse why-provenance explanations. Our evaluation has three main objectives. First, we compare the two solution strategies introduced earlier, namely the \emph{optimal} approach that computes a diversity-maximizing set of explanations in a single step, and the \emph{greedy} approach that incrementally constructs such a set, in terms of both runtime and achieved diversity. Second, we assess the impact of the underlying encoding technique used for constructing the Boolean formula, namely the \emph{DAG-based} encoding and the \emph{hypergraph-based} encoding, on performance and scalability. Third, we study the effect of the provenance semantics, by comparing standard why-provenance with its refinement based on unambiguous proof trees (see Section~\ref{sec:why-prov}), on both the size and the quality of the generated explanations.

\medskip
\noindent \textbf{Experimental Setup.}

\smallskip
\noindent \emph{Datasets.}
We consider a variety of scenarios from the Datalog literature consisting of a query $Q = (\dep,R)$ and a family of databases $\mathcal{D}$ over $\esch{\dep}$. All the considered scenarios are summarized in Table~\ref{tab:scenarios}; further details about the scenarios can be found in the appendix.

\smallskip
\noindent \emph{Configurations.}
Our evaluation considers all combinations of the design choices introduced in the previous sections. In particular, we compare the \emph{optimal} and \emph{greedy} strategies for computing a set of $k$ explanations, two alternative encodings of the problem into Boolean formulas, namely the \emph{DAG-based} and \emph{hypergraph-based} encodings, and two provenance semantics, namely standard why-provenance and its restriction to unambiguous proof trees. Each experimental result corresponds to one such configuration.

\smallskip
\noindent \emph{Evaluation Measures.}
We evaluate each configuration along two main dimensions. The first is \emph{runtime}, measured as the total end-to-end time required to compute a set of $k$ explanations for a given answer tuple, including the construction of the downward closure, the generation of the Boolean formula, and the execution of the SAT solver. The second is \emph{diversity}, measured using the diversity function $\delta(\cdot)$ defined in Section~4, which captures the pairwise symmetric differences between the selected explanations. When full enumeration is not feasible, we also report the number of explanations generated within the given time budget.

\smallskip
\noindent \emph{Procedure.}
For each scenario $s$ and each $D \in \mathcal{D}$, we compute $Q(D)$ using DLV and select 100 tuples $\bar t^1_{s,D},\ldots,\bar t^{100}_{s,D}$ uniformly at random, leading to a total of 1500 why-provenance instances. For each tuple $\bar t^i_{s,D}$, we construct the downward closure of $R(\bar t^i_{s,D})$ with respect to $D$ and $\dep$ by first computing the adapted query $Q_{\downarrow}$ and database $D_{\downarrow}$ via a Python 3 implementation, and then evaluating it using DLV. Based on the resulting closure, we generate a Boolean formula $\phi_{(\bar t^i_{s,D},D,Q)}$ using a C++ implementation.

We then invoke the SAT solver \emph{Glucose} (version 4.2.1)~\cite{Audemard18} to enumerate explanations. Depending on the configuration, the solver is used either to compute an optimal set of $k$ explanations or to iteratively construct such a set via the greedy strategy. Since the size of the why-provenance can be extremely large, we limit the enumeration phase to at most 10K explanations or a timeout of 5 minutes per tuple, whichever occurs first.

\smallskip
\noindent \emph{System Details.}
All experiments were conducted on a laptop equipped with an Intel(R) Core(TM) i7-10750H CPU @ 2.60GHz and 32GB of RAM, running Fedora Linux 37. The Python components were executed using Python 3.11.2, while the C++ code was compiled with \texttt{g++} 12.2.1 using the \texttt{-O3} optimization flag.

{\footnotesize 
	\begingroup
	\setlength{\tabcolsep}{5pt} % Default value: 6pt
	\renewcommand{\arraystretch}{1.4} % Default value: 1
	\begin{table}[t]
		\centering
		\begin{tabular}{|c||c|c|c|}
			\hline
			\small \textbf{Scenario} & \small \textbf{Databases} & \small \textbf{\#Rules} & \small \textbf{Recursive}\\ \hline
			\hline
			$\substack{\mathsf{TransClosure}}$ & $\substack{D_\mathsf{bitcoin} \text{(235K)}, D_\mathsf{facebook} \text{(88.2K)}}$ & \small 2 & \small {51}\\ \hline
			$\substack{\mathsf{Doctors\text{-}}i,\\ i \in [7]}$& $\substack{D_1 \text{(100K)}}$ & \small 6 & \small {55}\\ \hline
			$\substack{\mathsf{Galen}}$ & $\substack{D_1 \text{(26.5K)}, D_2 \text{(30.5K)},\\D_3 \text{(67K)}, D_4 \text{(82K)}}$ & \small 14 & \small {51}\\ \hline
			$\substack{\mathsf{Andersen}}$ & $\substack{D_1 \text{(68K)}, D_2 \text{(340K)},\\D_3 \text{(680K)}, D_4 \text{(3.4M)}, D_5 \text{(6.8M)}}$ & \small4 & \small {51}\\ \hline
			$\substack{\mathsf{CSDA}}$ & $\substack{D_\mathsf{httpd} \text{(10M)}, D_\mathsf{postgresql} \text{(34.8M)},\\ D_\mathsf{linux} \text{(44M)}}$ & \small 2 & \small {51}\\ \hline
		\end{tabular}
		\caption{Experimental scenarios. For each database $D$, we give in parenthesis the number of tuples occurring in $D$.}
		\label{tab:scenarios}
	\end{table}
	\endgroup
}



\medskip
\noindent \textbf{Experimental Results.} 
Missing...

\input{exact-exp}

\input{approximate-exp}

\input{ratios-exp}








==> extras.tex <==
% With not much additional overhead, we can find useful, unambiguous ones

% downward closure size and its impact on, trying plots with downward closure size in x and time in y

% Beyond the overall scalability trend, the results also reveal differences in runtime variability and encoding behavior. For small values of $k$, runtimes are tightly concentrated, indicating stable and predictable performance (e.g., Figures~\ref{fig:csda-postgresql-exact} and~\ref{fig:csda-linux-exact}). As $k$ increases, the distributions become wider and more skewed, showing substantially higher variance across instances, even before reaching the timeout threshold, which is typical for combinatorial optimization problems such as ILP.

% The number of evaluated goals also varies across configurations. In general, arbitrary semantics produce more explanations than unambiguous semantics, making larger values of $k$ more likely. Consequently, some settings contain more evaluated goals under arbitrary semantics (e.g., the \forty and \fifty databases in \galen; Figures~\ref{fig:galen-40-exact} and~\ref{fig:galen-50-exact}).

% Finally, there is no consistent winner between the hypergraph- and DAG-based encodings. Hypergraph encodings are faster in some cases (e.g., \doctors in Figures~\ref{fig:doctors-q01-100k-exact}-\ref{fig:doctors-q07-100k-exact}), while DAG encodings perform better in others (e.g., Figures~\ref{fig:csda-linux-exact} and~\ref{fig:galen-50-exact}). This suggests that performance depends more on the structure of the downward closure and the resulting ILP instance than on the encoding itself.

==> figures/approximate-results-10.tex <==
\begin{figure*}[t]
\centering
\small

\begin{subfigure}[t]{0.36\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/k10/csda-httpd-approximate-arbitrary-hypergraph.pdf}
    \caption{\arbitrary, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/k10/csda-httpd-approximate-unambigous-hypergraph.pdf}
    \caption{\unambiguous, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/k10/csda-httpd-approximate-unambigous-dag.pdf}
    \caption{\unambiguous, \dagEnc}
\end{subfigure}

\caption{Runtime distribution for the \approximate\ strategy on the \httpd\ dataset under the \csda\ scenario.}
\label{fig:k10-csda-httpd-approximate}
\end{figure*}

\begin{figure*}[t]
\centering
\small

\begin{subfigure}[t]{0.36\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/k10/csda-postgresql-approximate-arbitrary-hypergraph.pdf}
    \caption{\arbitrary, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/k10/csda-postgresql-approximate-unambigous-hypergraph.pdf}
    \caption{\unambiguous, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/k10/csda-postgresql-approximate-unambigous-dag.pdf}
    \caption{\unambiguous, \dagEnc}
\end{subfigure}

\caption{Runtime distribution for the \approximate\ strategy on the \postgres\ dataset under the \csda\ scenario.}
\label{fig:k10-csda-postgresql-approximate}
\end{figure*}

\begin{figure*}[t]
\centering
\small

\begin{subfigure}[t]{0.36\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/k10/csda-linux-approximate-arbitrary-hypergraph.pdf}
    \caption{\arbitrary, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/k10/csda-linux-approximate-unambigous-hypergraph.pdf}
    \caption{\unambiguous, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/k10/csda-linux-approximate-unambigous-dag.pdf}
    \caption{\unambiguous, \dagEnc}
\end{subfigure}

\caption{Runtime distribution for the \approximate\ strategy on the \linux\ dataset under the \csda\ scenario.}
\label{fig:k10-csda-linux-approximate}
\end{figure*}

% =========================
% Graph analytics
% =========================

\begin{figure*}[t]
\centering
\small

\begin{subfigure}[t]{0.36\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/k10/graph_analytics-facebook-approximate-arbitrary-hypergraph.pdf}
    \caption{\arbitrary, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/k10/graph_analytics-facebook-approximate-unambigous-hypergraph.pdf}
    \caption{\unambiguous, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/k10/graph_analytics-facebook-approximate-unambigous-dag.pdf}
    \caption{\unambiguous, \dagEnc}
\end{subfigure}

\caption{Runtime distribution for the \approximate\ strategy on the \facebook\ dataset under the \plotlabel{graph\_analytics} scenario.}
\label{fig:k10-graph-analytics-facebook-approximate}
\end{figure*}


==> figures/approximate-results.tex <==
\begin{figure*}[t]
\centering
\small

\begin{subfigure}[t]{0.36\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/csda-httpd-approximate-arbitrary-hypergraph.pdf}
    \caption{\arbitrary, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/csda-httpd-approximate-unambigous-hypergraph.pdf}
    \caption{\unambiguous, \hypergraph}
    \label{fig:csda-httpd-approximate-b}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/csda-httpd-approximate-unambigous-dag.pdf}
    \caption{\unambiguous, \dagEnc}
\end{subfigure}

\caption{Runtime distribution for the \approximate\ strategy on the \httpd\ dataset under the \csda\ scenario.}
\label{fig:csda-httpd-approximate}
\end{figure*}

\begin{figure*}[t]
\centering
\small

\begin{subfigure}[t]{0.36\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/csda-postgresql-approximate-arbitrary-hypergraph.pdf}
    \caption{\arbitrary, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/csda-postgresql-approximate-unambigous-hypergraph.pdf}
    \caption{\unambiguous, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/csda-postgresql-approximate-unambigous-dag.pdf}
    \caption{\unambiguous, \dagEnc}
\end{subfigure}

\caption{Runtime distribution for the \approximate\ strategy on the \postgres\ dataset under the \csda\ scenario.}
\label{fig:csda-postgresql-approximate}
\end{figure*}

\begin{figure*}[t]
\centering
\small

\begin{subfigure}[t]{0.36\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/csda-linux-approximate-arbitrary-hypergraph.pdf}
    \caption{\arbitrary, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/csda-linux-approximate-unambigous-hypergraph.pdf}
    \caption{\unambiguous, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/csda-linux-approximate-unambigous-dag.pdf}
    \caption{\unambiguous, \dagEnc}
\end{subfigure}

\caption{Runtime distribution for the \approximate\ strategy on the \linux\ dataset under the \csda\ scenario.}
\label{fig:csda-linux-approximate}
\end{figure*}

% =========================
% Graph analytics
% =========================

\begin{figure*}[t]
\centering
\small

\begin{subfigure}[t]{0.36\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/graph_analytics-facebook-approximate-arbitrary-hypergraph.pdf}
    \caption{\arbitrary, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/graph_analytics-facebook-approximate-unambigous-hypergraph.pdf}
    \caption{\unambiguous, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/graph_analytics-facebook-approximate-unambigous-dag.pdf}
    \caption{\unambiguous, \dagEnc}
\end{subfigure}

\caption{Runtime distribution for the \approximate\ strategy on the \facebook\ dataset under the \plotlabel{graph\_analytics} scenario.}
\label{fig:graph-analytics-facebook-approximate}
\end{figure*}

\begin{figure*}[t]
\centering
\small

\begin{subfigure}[t]{0.36\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/graph_analytics-bitcoin-approximate-arbitrary-hypergraph.pdf}
    \caption{\arbitrary, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/graph_analytics-bitcoin-approximate-unambigous-hypergraph.pdf}
    \caption{\unambiguous, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/graph_analytics-bitcoin-approximate-unambigous-dag.pdf}
    \caption{\unambiguous, \dagEnc}
\end{subfigure}

\caption{Runtime distribution for the \approximate\ strategy on the \bitcoin\ dataset under the \plotlabel{graph\_analytics} scenario.}
\label{fig:graph-analytics-bitcoin-approximate}
\end{figure*}

% =========================
% Doctors
% =========================

\begin{figure*}[t]
\centering
\small

\begin{subfigure}[t]{0.36\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/doctors_q01-100k-approximate-arbitrary-hypergraph.pdf}
    \caption{\arbitrary, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/doctors_q01-100k-approximate-unambigous-hypergraph.pdf}
    \caption{\unambiguous, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/doctors_q01-100k-approximate-unambigous-dag.pdf}
    \caption{\unambiguous, \dagEnc}
    \label{fig:doctors-q01-100k-approximate-c}
\end{subfigure}

\caption{Runtime distribution for the \approximate\ strategy on the \factsk\ dataset under the \doctors\ (\texttt{q01}) scenario.}
\label{fig:doctors-q01-100k-approximate}
\end{figure*}

\begin{figure*}[t]
\centering
\small

\begin{subfigure}[t]{0.36\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/doctors_q02-100k-approximate-arbitrary-hypergraph.pdf}
    \caption{\arbitrary, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/doctors_q02-100k-approximate-unambigous-hypergraph.pdf}
    \caption{\unambiguous, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/doctors_q02-100k-approximate-unambigous-dag.pdf}
    \caption{\unambiguous, \dagEnc}
\end{subfigure}

\caption{Runtime distribution for the \approximate\ strategy on the \factsk\ dataset under the \doctors\ (\texttt{q02}) scenario.}
\label{fig:doctors-q02-100k-approximate}
\end{figure*}

\begin{figure*}[t]
\centering
\small

\begin{subfigure}[t]{0.36\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/doctors_q03-100k-approximate-arbitrary-hypergraph.pdf}
    \caption{\arbitrary, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/doctors_q03-100k-approximate-unambigous-hypergraph.pdf}
    \caption{\unambiguous, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/doctors_q03-100k-approximate-unambigous-dag.pdf}
    \caption{\unambiguous, \dagEnc}
\end{subfigure}

\caption{Runtime distribution for the \approximate\ strategy on the \factsk\ dataset under the \doctors\ (\texttt{q03}) scenario.}
\label{fig:doctors-q03-100k-approximate}
\end{figure*}

\begin{figure*}[t]
\centering
\small

\begin{subfigure}[t]{0.36\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/doctors_q04-100k-approximate-arbitrary-hypergraph.pdf}
    \caption{\arbitrary, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/doctors_q04-100k-approximate-unambigous-hypergraph.pdf}
    \caption{\unambiguous, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/doctors_q04-100k-approximate-unambigous-dag.pdf}
    \caption{\unambiguous, \dagEnc}
\end{subfigure}

\caption{Runtime distribution for the \approximate\ strategy on the \factsk\ dataset under the \doctors\ (\texttt{q04}) scenario.}
\label{fig:doctors-q04-100k-approximate}
\end{figure*}

\begin{figure*}[t]
\centering
\small

\begin{subfigure}[t]{0.36\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/doctors_q05-100k-approximate-arbitrary-hypergraph.pdf}
    \caption{\arbitrary, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/doctors_q05-100k-approximate-unambigous-hypergraph.pdf}
    \caption{\unambiguous, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/doctors_q05-100k-approximate-unambigous-dag.pdf}
    \caption{\unambiguous, \dagEnc}
\end{subfigure}

\caption{Runtime distribution for the \approximate\ strategy on the \factsk\ dataset under the \doctors\ (\texttt{q05}) scenario.}
\label{fig:doctors-q05-100k-approximate}
\end{figure*}

\begin{figure*}[t]
\centering
\small

\begin{subfigure}[t]{0.36\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/doctors_q06-100k-approximate-arbitrary-hypergraph.pdf}
    \caption{\arbitrary, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/doctors_q06-100k-approximate-unambigous-hypergraph.pdf}
    \caption{\unambiguous, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/doctors_q06-100k-approximate-unambigous-dag.pdf}
    \caption{\unambiguous, \dagEnc}
\end{subfigure}

\caption{Runtime distribution for the \approximate\ strategy on the \factsk\ dataset under the \doctors\ (\texttt{q06}) scenario.}
\label{fig:doctors-q06-100k-approximate}
\end{figure*}

\begin{figure*}[t]
\centering
\small

\begin{subfigure}[t]{0.36\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/doctors_q07-100k-approximate-arbitrary-hypergraph.pdf}
    \caption{\arbitrary, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/doctors_q07-100k-approximate-unambigous-hypergraph.pdf}
    \caption{\unambiguous, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/doctors_q07-100k-approximate-unambigous-dag.pdf}
    \caption{\unambiguous, \dagEnc}
    \label{fig:doctors-q07-100k-approximate-c}
\end{subfigure}

\caption{Runtime distribution for the \approximate\ strategy on the \factsk\ dataset under the \doctors\ (\texttt{q07}) scenario.}
\label{fig:doctors-q07-100k-approximate}
\end{figure*}

% =========================
% Galen
% =========================



\begin{figure*}[t]
\centering
\small

\begin{subfigure}[t]{0.36\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/galen-40-approximate-arbitrary-hypergraph.pdf}
    \caption{\arbitrary, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/galen-40-approximate-unambigous-hypergraph.pdf}
    \caption{\unambiguous, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/galen-40-approximate-unambigous-dag.pdf}
    \caption{\unambiguous, \dagEnc}
\end{subfigure}

\caption{Runtime distribution for the \approximate\ strategy on the \plotlabel{40} dataset under the \galen\ scenario.}
\label{fig:galen-40-approximate}
\end{figure*}

\begin{figure*}[t]
\centering
\small

\begin{subfigure}[t]{0.36\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/galen-50-approximate-arbitrary-hypergraph.pdf}
    \caption{\arbitrary, \hypergraph}
    \label{fig:galen-50-approximate-a}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/galen-50-approximate-unambigous-hypergraph.pdf}
    \caption{\unambiguous, \hypergraph}
    \label{fig:galen-50-approximate-b}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/galen-50-approximate-unambigous-dag.pdf}
    \caption{\unambiguous, \dagEnc}
\end{subfigure}

\caption{Runtime distribution for the \approximate\ strategy on the \plotlabel{50} dataset under the \galen\ scenario.}
\label{fig:galen-50-approximate}
\end{figure*}


























==> figures/approximation.tex <==
\section{Approximation Algorithm for Diverse Why-Provenance}\label{sec:approximations}

We proceed to present an approximation algorithm for the problem $\star\text{-}\mathsf{DiverseWhyProvenance}$, where $\star \in \{\mathsf{ALL},\mathsf{UN}\}$. In particular, our goal is to devise a procedure that, given as input a Datalog query $Q =(\dep,R)$, a database $D$ over $\esch{\dep}$, a tuple $\bar t \in \adom{D}^{\arity{R}}$, and an integer $k > 0$, on the one hand it computes a set $\hat{\mathcal{S}} \in \starwhyk{k}{\bar t}{D}{Q}$ whose diversity is an approximation of the optimal diversity, but on the other hand it performs much faster, in practice, than the approach discussed in Section~\ref{sec:characterizations} that aims for an exact computation.
%
We first formalize the kind of approximation algorithm we aim for, and then explain how we obtain such an algorithm.

\begin{definition}
For any $\beta \in (0,1)$, a \emph{$\beta$-approximation algorithm for $\star\text{-}\mathsf{DiverseWhyProvenance}$}, where $\star \in \{\mathsf{ALL},\mathsf{UN}\}$, is an algorithm that, given as input a Datalog query $Q = (\dep,R)$, a database $D$ over $\esch{\dep}$, a tuple $\bar t \in \adom{D}^{\arity{R}}$, and an integer $k > 0$, outputs a set $\hat{\mathcal{S}} \in \starwhyk{k}{\bar t}{D}{Q}$ of $k$ databases such that
$$\diversity{\hat{\mathcal{S}}} \ge \beta \cdot\diversity{\mathcal{S}_{\mathsf{opt}}},$$
if there is $\mathcal{S}_{\mathsf{opt}} \in \argmax\limits_{\mathcal{S} \in \whyk{k}{\bar t}{D}{Q}} \diversity{\mathcal{S}}$; otherwise, it fails.\hfill\markfull
\end{definition}

\medskip
\noindent
\textbf{Diverse Why-Provenance as a Remote-Clique Problem.}
To devise the desired approximation algorithm, we first observe that $\star\text{-}\mathsf{DiverseWhyProvenance}$ can be seen as a (succinct) encoding of the remote-clique problem, a well-studied optimization problem in graph theory. Consider an edge-weighted, undirected graph $G = (V,E,w)$, where $w : E \rightarrow \mathbb{N}$ assigns a non-negative weight to each edge of $G$. By abuse of notation, for an edge $\{u,v\} \in E$, we may write $w(u,v)$ or $w(v,u)$ instead of $w(\{u,v\})$. We further assume that $w(v,v) = 0$, for each node $v \in V$.
%
We say that $G$ is \emph{complete} if, for every pair of distinct nodes $u,v \in V$, there is an edge $\{u,v\} \in E$. For an edge-weighted, complete, undirected graph $G = (V,E,w)$, we say that $w$ \emph{satisfies the triangle inequality} if, for every three nodes $v_1,v_2,v_3 \in V$, $w(v_1,v_3) \le w(v_1,v_2) + w(v_2,v_3)$,
%
For an integer $k > 0$, we denote by $\cliques{k}{G}$ the family of all sets $V' \subseteq V$ of $k$ nodes of $G$. Finally, for a set $V'= \{v_1,\ldots,v_k\} \in \cliques{k}{G}$, the \emph{diversity} of $V'$ is defined as the integer
\[
\diversity{V'} = \sum\limits_{i,j \in [|V'|] \text{ and }i<j} w(v_i,v_j).
\]
The remote-clique problem is defined as follows:

\medskip

\begin{center}
	\fbox{\begin{tabular}{ll}
			{\small PROBLEM} : & $\mathsf{Remote\text{-}Clique}$
			\\[2mm]
			{\small INPUT} : & A complete, edge-weighted, undirected graph \\
			& $G = (V,E,w)$, where $w$ satisfies the triangle \\
			& inequality, and an integer $k > 0$\\[2mm]
			{\small OUTPUT} : & A member of $\argmax\limits_{V' \in \cliques{k}{G}} \diversity{V'}$ if it exists;\\
			&  otherwise \textbf{fail} 
	\end{tabular}}
\end{center}

\medskip


It is easy to see that the problem $\star\text{-}\mathsf{DiverseWhyProvenance}$, where $\star \in \{\mathsf{ALL},\mathsf{UN}\}$, can be reduced to $\mathsf{Remote\text{-}Clique}$. In particular, given a Datalog query $Q = (\dep, R)$, a database $D \in \esch{\dep}$, a tuple $\bar t \in \adom{D}^{\arity{R}}$, and an integer $k > 0$, we can construct the edge-weighted, complete, undirected graph $G = (V,E,w)$, where $V = \starwhy{\bar t}{D}{Q}$, such that $w(D_1,D_2) = |\diff{D_1}{D_2}|$, for each $D_1,D_2 \in V$.\footnote{The weight function $w$ defined as $w(D_1,D_2) = |\diff{D_1}{D_2}|$ satisfies the triangle inequality by definition, since the symmetric difference is such that $\diff{A}{C} \subseteq \diff{A}{B} \cup \diff{B}{C}$, for any three sets $A,B,C$.}
%
It is clear that the output of $\mathsf{Remote\text{-}Clique}$ with input the graph $G$ as defined above and the integer $k$, coincides with the output of $\star\text{-}\mathsf{DiverseWhyProvenance}$ with input $Q$, $D$, $\bar t$, and $k$.

\medskip
\noindent
\textbf{Approximation Algorithm for $\mathsf{Remote\text{-}Clique}$.}
Due to the connection between our problem and the  $\mathsf{Remote\text{-}Clique}$ problem discussed above, we can exploit exiting approximation algorithms for  $\mathsf{Remote\text{-}Clique}$ to provide an approximation algorithm for our problem.
%
The state of the art approximation algorithm for $\mathsf{Remote\text{-}Clique}$ is a greedy algorithm defined as follows. Given an input $G,k$ of the problem $\mathsf{Remote\text{-}Clique}$, the algorithm performs $k$ iterations, where at each iteration $i \in [k]$, the algorithm picks a node $v_i \in V$ such that $v_i$ is different from all previously selected nodes $v_{j}$, with $j < i$, and $v_{i}$ is such that the quantity $\diversity{\{v_1,\ldots,v_{i}\}} - \diversity{\{v_1,\ldots,v_{i-1}\}}$ is maximized, namely $v_i$ maximizes the \emph{marginal diversity}, i.e., the increase in diversity w.r.t.\ the set of nodes constructed so far. For each $i \in [k]$, if $v_{i}$ cannot be found with the above constraints, the algorithm halts failing. If instead all $k$ iterations complete without failing, the algorithm outputs the set $\{v_1,\ldots,v_{k}\}$, and halts.
The above algorithm is a $\frac{1}{2}$-approximation algorithm for $\mathsf{Remote\text{-}Clique}$, where for any $\beta \in (0,1)$, a $\beta$-approximation algorithm for $\mathsf{Remote\text{-}Clique}$ is an algorithm that, given $G$ and $k$, outputs a set $\hat{V}$ of $k$ nodes such that $\diversity{\hat{V}} \ge \beta \cdot \diversity{V_\mathsf{opt}}$, if there is $V_\mathsf{opt} \in \argmax\limits_{V' \in \cliques{k}{G}} \diversity{V'}$; otherwise, it fails.
%
Moreover, the factor $\frac{1}{2}$ is \emph{tight} for the approximation algorithm, i.e., there exist families of inputs $G,k$ for which the algorithm returns a set $\hat{V}$ of $k$ nodes with $\diversity{\hat{V}} = \frac{1}{2} \cdot \diversity{V_{\mathsf{opt}}}$.

\medskip
\noindent
\textbf{Approximation Algorithm for Diverse Why-Provenance.} A naive adaptation of the greedy $\frac{1}{2}$-approximation algorithm discussed above to the problem $\star\text{-}\mathsf{DiverseWhyProvenance}$ would be as follows: given a Datalog query $Q = (\dep,R)$, a database $D$ over $\esch{\dep}$, a tuple $\bar t \in \adom{D}^{\arity{R}}$, and an integer $k > 0$, (i) first construct the set $\starwhy{\bar t}{D}{Q}$, (ii) then construct the graph $G = (V,E,w)$ with $V = \starwhy{\bar t}{D}{Q}$ and $w(D_1,D_2) = |\diff{D_1}{D_2}|$, for $D_1,D_2 \in V$, and (iii) finally execute the $\frac{1}{2}$-approximation algorithm for the problem $\mathsf{Remote\text{-}Clique}$ with input $G,k$.
%
However, this naive approach would never scale in practice since it requires to construct the whole graph $G$ explicitly, which in turn requires the construction of the whole set $\starwhy{\bar t}{D}{Q}$ upfront; the latter can be very large in practice. Hence, we need a more sophisticated approach that does not require an explicit construction of the graph $G$. To this end, we observe that for the the approximation algorithm to work, the only requirement is to have a strategy for selecting a node $v_i$ at each iteration $i \in [k]$ that maximizes the integer $\diversity{\{v_1,\ldots,v_{i}\}} - \diversity{\{v_1,\ldots,v_{i-1}\}}$. In terms of our problem, this means that we need a way, given an already constructed set of $i-1$ databases $D_1,\ldots,D_{i-1}$ from $\starwhy{\bar t}{D}{Q}$, to construct a new database $D_i \in \starwhy{\bar t}{D}{Q}$ that differs from all $D_1,\ldots,D_{i-1}$, and the marginal diversity $\diversity{\{D_1,\ldots,D_i\}} - \diversity{\{D_1,\ldots,D_{i-1}\}}$ is maximized.
%
We show that we can perform the above steps without explicitly constructing $\starwhy{\bar t}{D}{Q}$, by exploiting once again our ILP-based framework introduced above.

Consider a Datalog query $Q = (\dep,R)$, a database $D$ over $\esch{\dep}$, a tuple $\bar t \in \adom{D}^{\arity{R}}$, and an integer $k > 0$. 
%
%We now discuss how the approximation algorithm for $\mathsf{Remote\text{-}Clique}$ can be implemented for the problem $\star\text{-}\mathsf{DiverseWhyProvenance}$, without explicitly constructing $\starwhy{\bar t}{D}{Q}$, by exploiting our ILP-based machinery, and then show that our algorithm is indeed a $\frac{1}{2}$-approximation algorithm for $\star\text{-}\mathsf{DiverseWhyProvenance}$.
%
Let $T$ be an ILP encoding for $\starwhy{\bar t}{D}{Q}$, where $\star \in \{\mathsf{ALL},\mathsf{UN}\}$, and let $\mu$ be an assignment whose domain mentions the database variables $x_{\alpha_1},\ldots,x_{\alpha_n}$ of $T$. For each integer $i \in [n]$, we use $g_{\mu,i}$ to denote the ``opposite'' of $x_{\alpha_i}$ w.r.t. $\mu$, i.e., the expression $1 - x_{\alpha_i}$ if $\mu(x_{\alpha_i}) = 1$, and the expression $x_{\alpha_i}$, if $\mu(x_{\alpha_i}) = 0$.
The approximation algorithm, called $\star\text{-}\mathsf{Approx}$, is depicted in Algorithm~\ref{alg:generic-approximation}.
%
\begin{algorithm}[t]
	\caption{The $\frac{1}{2}$-approximation algorithm $\star\text{-}\mathsf{Approx}$}
	\label{alg:generic-approximation}
	
	\BlankLine
	
	\KwIn{A Datalog query $Q = (\dep,R)$, a database $D = \{\alpha_1,\ldots,\alpha_n\}$ over $\esch{\dep}$, a tuple $\bar t \in \adom{D}^{\arity{R}}$, and an integer $k >0 $.}
	\KwOut{A set of $k$ databases, or \textbf{fail}}
	
	\BlankLine
	
	$T :=$ an ILP encoding for $\starwhy{\bar t}{D}{Q}$\;
	$f := 0$\;
	$D_1 := \emptyset$; \ldots ; $D_k := \emptyset$\;
	\For{$i = 1$ \textbf{\text{to}} $k$}{
		$\mu :=$ an optimal solution of $(f,T)$ \textbf{if} exists, \textbf{else} \textbf{fail}\;
		$D_i := \db{\mu}$\;\ \\

		$T := T \cup \left\{\sum\limits^n_{\ell = 1} g_{\mu,\ell} \ge 1\right\}$;\hfill\tcp{\footnotesize Force $D_{i+1}$ to be new}
		$f := f + \sum\limits^n_{\ell = 1} g_{\mu,\ell}$;\hfill\tcp{\footnotesize Maximize $\diversity{\{D_1,\ldots,D_{i+1}\}} - \diversity{\{D_1,\ldots,D_{i}\}}$}
	}
	\textbf{return} $\{D_1,\ldots,D_{k}\}$;
\end{algorithm}
%
We can show the following:
\begin{theorem}\label{thm:approximation-quality}
For $\star \in \{\mathsf{ALL},\mathsf{UN}\}$, $\star\text{-}\mathsf{Approx}$ is a $\frac{1}{2}$-approximation algorithm for $\star\text{-}\mathsf{DiverseWhyProvenance}$.
\end{theorem}
\begin{proof}
	\textcolor{red}{Missing...}
\end{proof}


% Moreover, we can prove that $\mathsf{Approx}$ is optimal:
% \begin{theorem}\label{thm:approximation-optimal}
% 	There is no $\beta$-approximation algorithm for $\mathsf{Diversity}$ with $\beta > \frac{1}{2}$.
% \end{theorem}
% \begin{proof}
% 	\textcolor{red}{Missing...}
% \end{proof}

==> figures/characterizations.tex <==
\section{ILP Encodings of Why-Provenance}\label{sec:characterizations}

Theorem~\ref{thm:generic-encoding} essentially states that we can compute a solution of $\star\text{-}\mathsf{DiverseWhyProvenance}$, where $\star \in  \{\mathsf{ALL},\mathsf{UN}\}$, on input $Q = (\dep,R)$, $D$, $\bar t$, and $k > 0$, by simply finding an optimal solution of the $(T,k)$-problem, where $T$ is any ILP encoding of $\starwhy{\bar t}{D}{Q}$.
%
In this section, we provide concrete ILP encodings of $\starwhy{\bar t}{D}{Q}$.
%
To this end, we present the main characterizations from the literature of when a database $D' \subseteq D$ is a member of $\starwhy{\bar t}{D}{Q}$, or equivalently, when there is an arbitrary (resp., unambiguous) proof tree $T$ of the fact $R(\bar t)$ w.r.t.~$D$ and $\dep$ with $\support{T} = D'$.
%
For each such characterization, we discuss how it can be used to devise ILP encodings of $\starwhy{\bar t}{D}{Q}$.
%
Before we proceed further, we need to discuss some basic assumptions and recall some auxiliary notions.


%In this section, we present the main characterizations for the existence of a standard (resp., unambiguous) proof tree of a fact $R(\bar t)$ w.r.t.\ a database $D$ and program $\dep$ with a given support that we inherit from the literature, and show how to exploit such characterizations to devise ILP encodings for $\allwhy{\bar t}{D}{\dep}$ (resp., $\unwhy{\bar t}{D}{\dep})$.
%For this we first need to discuss some basic assumptions, and recall some notions. 

\medskip
\noindent
\textbf{Programs.} In order to simplify the technical definitions, in the rest of this section, for a Datalog program $\dep$,
we assume that for each rule $\sigma \in \dep$ of the form $R_0(\bar x_0) \ \assign\ R_1(\bar x_1),\ldots,R_n(\bar x_n)$, the predicates $R_1,\ldots,R_n$ are all distinct, i.e., rule-bodies are self-join-free. The latter assumption can be done w.l.o.g.~since we can always convert $\dep$ into $\dep'$ that satisfies the desired condition without affecting the why-provenance of $R(\bar t)$ w.r.t.~$D$ and $\dep$ relative to both arbitrary and unambiguous proof trees. In particular, for each rule $\sigma$ as above, and for each $i \in [n]$, let $\text{\rm Aux}^\sigma_i \not\in \sch{\dep}$ be an auxiliary predicate of arity $\arity{R_i}$, replace $R_i$ with $\text{\rm Aux}^\sigma_i$ in the body of $\sigma$, and add to $\dep$ the rule $\text{\rm Aux}^\sigma_i(x_1,\ldots,x_{\arity{R_i}})\ \assign\ R_i(x_1,\ldots,x_{\arity{R_i}})$. Clearly, for $\star \in \{\mathsf{ALL},\mathsf{UN}\}$, $\starwhy{\bar t}{D}{Q} = \starwhy{\bar t}{D}{Q'}$, where $Q'=(\dep',R)$.

\medskip
\noindent
\textbf{Multisets.}
A \emph{multiset} $M$ is a pair $(S,\mu)$, where $S$ is a set and $\mu : S \rightarrow \mathbb{N}$ is a function assigning to each element $a \in S$ a strictly positive integer, called the \emph{multiplicity of $a$ in $S$}. We say that $M$ is \emph{empty} if $S$ is empty, otherwise it is non-empty.
The \emph{cardinality} of $M$, denoted $|M|$, is $\sum\limits_{a \in S} \mu(a)$. By abuse of notation, we may write $a \in M$ meaning that $a \in S$. Moreover, we may write $\card{a}{M}$ for $\mu(a)$, if $a \in S$, and $0$ if $a \not \in S$. 
%
Finally, for a sequence of (not necessarily distinct) objects $o_1,\ldots,o_n$, we write $\multiset{o_1,\ldots,o_n}$ to denote the multiset $(S,\mu)$, where $S = \{o_1,\ldots,o_n\}$ and $\mu$ assigns to each element of $S$ the number of times the element occurs in the sequence $o_1,\ldots,o_n$.


\medskip

\noindent
\textbf{Downward Closure.} We now introduce the so-called {\em downward closure} of a fact w.r.t.~a database and a Datalog program, taken from~\cite{ElKM22}, that will play a key role in all the characterizations we are going to discuss.
Roughly, the downward closure of a fact $\alpha$ w.r.t.~a database $D$ and a Datalog program $\dep$ is a hypergraph that encodes all possible proof trees of $\alpha$ w.r.t.~$D$ and $\dep$. 
%
For our purposes, a \emph{(directed) hypergraph} $\mathcal{H}$ is a pair $(V,E)$, where $V$ is the set of its \emph{nodes} and $E$ is the set of its \emph{hyperedges}, i.e., pairs of the form $(u,T)$, where $u \in V$ and $T \subseteq V$ is a non-empty set of nodes.

%\emph{multiset} of nodes from $V$.
%
For $u,v \in V$, we say that \emph{$u$ reaches $v$ in $\mathcal{H}$} if either $u=v$, or there exists a sequence of hyperedges $(u_1,T_1),\ldots,(u_n,T_n)$ with $u_1=u$, $v \in T_n$, and $u_i \in T_{i-1}$ for each $i \in \{2,\ldots,n\}$. For a node $u$, we write $\downof{\mathcal{H}}{u}$ for the hypergraph $(V',E')$ obtained from $\mathcal{H}$ where $V'$ contains $u$ and all nodes reachable from $u$, and $E'$ collects all the hyperedges mentioning only nodes of $V'$.

For a Datalog program $\dep$ and a database $D$ over $\esch{\dep}$, the \emph{graph of rule instances (GRI)} of $D$ and $\dep$ is the hypergraph $\gri{D}{\dep}=(V,E)$, with $V \subseteq \base{D,\dep}$, such that
\begin{enumerate}
	\item $D \subseteq V$, and 
	\item if there exists a rule $R_0(\bar x_0)\ \assign\ R_1(\bar x_1),\ldots,R_n(\bar x_n)$ in $\dep$ and a function $h : \bigcup_{i \in [n]} \bar x_i \ra \ins{C}$ such that $\alpha_i = R_i(h(\bar x_i)) \in V$, for $i \in [n]$, then $\alpha_0 = R_0(h(\bar x_0)) \in V$ and $(\alpha_0,\{\alpha_1,\ldots,\alpha_n\})$ is an hyperedge of $E$.
%	$(\alpha_0,\multiset{\alpha_1,\ldots,\alpha_n})$ is an hyperedge of $E$.
\end{enumerate}
Intuitively, $\gri{D}{\dep}$ encodes all proof trees of some fact $\alpha$ w.r.t.\ $D$ and $\dep$.
%
Since we are interested only in the proof trees of a specific fact $\alpha$, we do not need to consider $\gri{D}{\dep}$ in its entirety, but only the subhypergraph of $\gri{D}{\dep}$ containing $\alpha$ and all nodes reachable from it. This leads to the notion of downward closure, which simply keeps from $\gri{D}{\dep}$ the part that is relevant to derive the fact in question. 

\begin{definition}[\textbf{Downward Closure}]\label{def:downward-closure}
	Consider a Datalog program $\dep$, a database $D$ over $\esch{\dep}$, and a fact $\alpha$ occurring in $\gri{D}{\dep}$. The \emph{downward closure of $\alpha$ w.r.t.~$D$ and $\dep$}, denoted $\downc{\alpha}{D}{\dep}$, is the hypergraph $\downof{\gri{D}{\dep}}{\alpha}$. \hfill\markfull
\end{definition}


%The key property of the downward closure is the following
%
%
%\begin{lemma}[\cite{CLPS24aaai}]\label{lem:dag-in-down}
%	Consider a Datalog program $\dep$, a database $D$ over $\esch{\dep}$, a fact $\alpha$ over $\sch{\dep}$, and a proof tree $T=(V,E,\lambda)$ of $\alpha$ w.r.t.\ $D$ and $\dep$. Then, for every node $u \in V$ with outgoing edges $(u,v_1),\ldots,(u,v_n)$ in $T$, we have that $(\lambda(u),\multiset{\lambda(v_1),\ldots,\lambda(v_n)})$ is a hyperedge of $\downc{\alpha}{D}{\dep}$.
%\end{lemma}


We are now ready to present the ILP encodings of interest. Those encodings are classified into two main categories, namely the hypergaph- and the graph-based ones, depending on whether the underlying characterization of when a database is a member of $\starwhy{\bar t}{D}{Q}$, for $\star \in  \{\mathsf{ALL},\mathsf{UN}\}$, uses a hypergraph or a (directed acyclic) graph as a way for compactly representing proof trees.


\subsection{Hypergraph-based ILP Encodings}\label{sec:hypergraph-based}

We start by recalling the characterizations of interest that rely on hypergraphs, and then use them to devise the hypergraph-based ILP encodings of why-provenance.


\medskip
\noindent
\underline{\textbf{Hypergraph-based Characterizations}}

\smallskip
\noindent Consider a Datalog query $Q = (\dep,R)$, a database $D$ over $\esch{\dep}$, and a tuple $\bar t \in \adom{D}^{\arity{R}}$.
%
For a multiset $E = (E',\mu)$ of hyperedges from $\downc{R(\bar t)}{D}{\dep}$, we denote by $\nodes{E}$ the \emph{set} of nodes occurring in the hyperedges of $E$ and by $\hypergraphof{E}$ the hypergraph $(\nodes{E},E')$. For a node $\alpha \in \nodes{E}$, we define the \emph{in-degree of $\alpha$ in $E$}, denoted $\indegree{\alpha}{E}$, as 
the number of (possibly repeated) hyperedges of $E$ in which $\alpha$ appears as a target, namely
\[
\indegree{\alpha}{E} = \sum\limits_{(\beta,T) \in E' \text{ with } \alpha \in T} \mu((\beta,T)).
\]
%the number of times $\alpha$ appears as a target in all (possibly repeated) hyperedges of $E$, i.e.,
%$$\indegree{\alpha}{E} = \sum\limits_{(\beta,T) \in E'} \card{\alpha}{T} \cdot \mu((\beta,T)).$$
%
Moreover, the \emph{out-degree of $\alpha$ in $E$}, denoted $\outdegree{\alpha}{E}$, is the number of (possibly repeated) hyperedges in $E$ having $\alpha$ as the source, i.e.,
$$\outdegree{\alpha}{E} = \sum\limits_{(\alpha,T) \in E'} \mu((\alpha,T)).$$
%
We are now ready to recall the hypergraph-based characterization of when there is a proof tree of $R(\bar t)$ w.r.t.\ $D$ and $\dep$ with a certain support $D' \subseteq D$. This relies on the existence of a multiset of hyperedges with certain properties that one can extract from $\downc{R(\bar t)}{D}{\dep}$. We proceed to introduce those properties.
%define when a multiset of hyperedges enjoys these properties and then present the characterization.

\begin{definition}[\textbf{ (Unambiguous) Proof Tree Description}]\label{def:hypergraph-properties}
	Consider a Datalog query $Q=(\dep,R)$, a database $D$ over $\esch{\dep}$, a tuple $\bar t \in \adom{D}^{\arity{R}}$, and a  database $D' \subseteq D$. We say that a multiset $E$ of hyperedges from $\downc{R(\bar t)}{D}{\dep}$ is a \emph{description of a proof tree of $R(\bar t)$ w.r.t.~$D$ and $\dep$ with support $D'$} if the following hold:
	\begin{enumerate}
		\item $R(\bar t) \in V_E$ and $\outdegree{R(\bar t)}{E} - \indegree{R(\bar t)}{E} = 1$,
		\item $\outdegree{\alpha}{E} - \indegree{\alpha}{E} = 0$, for each $\alpha \in \nodes{E} \setminus (D \cup \{R(\bar t)\})$,
		\item $\sum\limits_{\alpha \in \nodes{E} \cap D} \indegree{\alpha}{E} \ge 1$,
		\item $R(\bar t)$ reaches all nodes of $\hypergraphof{E}$ in $\hypergraphof{E}$, and
		\item $D' = \nodes{E} \cap D$.
	\end{enumerate}
    We say that $E$ is a \emph{description of an unambiguous proof tree of $R(\bar t)$ w.r.t.~$D$ and $\dep$ with support $D'$} if, in addition to the above conditions, for every pair $(\alpha,T),(\alpha,T') \in E$, it holds that $T = T'$. \hfill\markfull
\end{definition}

The desired hypergraph-based characterizations follows:
%, which we call the \emph{hypergraph-based characterization}, follows:

\begin{theorem}[\cite{CalauttiLPS24b}]\label{thm:arbitrary-hypergraph}
	Consider a Datalog query $Q=(\dep,R)$, a database $D$ over $\esch{\dep}$, a tuple $\bar t \in \adom{D}^{\arity{R}}$, and a database $D' \subseteq D$. The following are equivalent:
	\begin{enumerate}
		\item There is a proof tree (resp., an unambiguous proof tree) of $R(\bar t)$ w.r.t.~$D$ and $\dep$ with support $D'$.
		\item There is a description $E$ of a proof tree (resp., an unambiguous proof tree) of $R(\bar t)$ w.r.t.~$D$ and $\dep$ with support $D'$.
	\end{enumerate}
\end{theorem}

Note that the version of Theorem~\ref{thm:arbitrary-hypergraph} for unambiguous proof trees has not been explicitly stated in~\cite{CalauttiLPS24b}, but it is an easy adaptation of its version for arbitrary proof trees.
\begin{comment}
One can easily adapt the above characterization to unambiguous proof trees by additionally requiring that no two hyperedges $(\alpha,T)$ and $(\alpha,T')$ with $T \neq T'$ appear in the multiset $E$.

\begin{definition}[\textbf{Unambiguous Proof Tree Description}]\label{def:un-hypergraph-properties}
	Consider a Datalog query $Q=(\dep,R)$, a database $D$ over $\esch{\dep}$, a tuple $\bar t \in \adom{D}^{\arity{R}}$, and a  database $D' \subseteq D$. We say that a multiset $E$ of hyperedges from $\downc{R(\bar t)}{D}{\dep}$ is a \emph{description of an unambiguous proof tree of $R(\bar t)$ w.r.t.~$D$ and $\dep$ with support $D'$} if:
    \begin{enumerate}
    \item $E$ is a description of a proof tree of $R(\bar t)$ w.r.t.~$D$ and $\dep$ with support $D'$, and 
    \item for every pair $(\alpha,T),(\alpha,T') \in E$, it holds that $T = T'$.\hfill\markfull
    \end{enumerate}
\end{definition}

The unambiguous hypergraph-based characterization follows:

\begin{theorem}[{\normalfont Implicit in }\cite{CalauttiLPS24b}]\label{thm:unambiguous-hypergraph}
	Consider a Datalog query $Q=(\dep,R)$, a database $D$ over $\esch{\dep}$, a tuple $\bar t \in \adom{D}^{\arity{R}}$, and a database $D' \subseteq D$. The following are equivalent:
	\begin{enumerate}
		\item There is an unambiguous proof tree of $R(\bar t)$ w.r.t.~$D$ and $\dep$ with support $D'$.
		\item There is a description $E$ of an unambiguous proof tree of $R(\bar t)$ w.r.t.~$D$ and $\dep$ with support $D'$.
	\end{enumerate}
\end{theorem}
\end{comment}
We now show
%, given a Datalog query $Q = (\dep,R)$, a database $D$ over $\esch{\dep}$, and a tuple $\bar t \in \adom{D}^{\arity{R}}$, 
how to exploit Theorem~\ref{thm:arbitrary-hypergraph} to devise an ILP encoding of why-provenance.
%$\starwhy{\bar t}{D}{Q}$, where $\star \in \{\mathsf{ALL},\mathsf{UN}\}$.
%$\allwhy{\bar t}{D}{Q}$ and $\unwhy{\bar t}{D}{Q}$, respectively, 

\medskip
\noindent
\underline{\textbf{Hypergraph-based ILP Encoding}}

\smallskip
\noindent In what follows, fix a Datalog query $Q=(\dep,R)$, a database $D$ over $\esch{\dep}$, a tuple $\bar t \in \adom{D}^{\arity{R}}$, and assume $\downc{R(\bar t)}{D}{\dep} = (V,E)$.
We start with the ILP encoding for $\allwhy{\bar t}{D}{Q}$, which we dub the \emph{hypergraph-based ILP encoding of $\allwhy{\bar t}{D}{Q}$}, and denote it by $\ilphypergraph{\bar t}{D}{Q}$.
%	
The high-level idea is to devise $\ilphypergraph{\bar t}{D}{Q}$ as a set of constraints whose solutions correspond to definitions of proof trees of $R(\bar t)$ w.r.t.\ $D$ and $\dep$ with \emph{some} support $D'$. This will imply that from each solution of $\ilphypergraph{\bar t}{D}{Q}$ one can extract the support $D'$ of a proof tree of $R(\bar t)$ w.r.t.\ $D$ and $\dep$, and thus $\ilphypergraph{\bar t}{D}{Q}$ would indeed be an ILP encoding for $\allwhy{\bar t}{D}{Q}$.
%
More formally, we construct $\ilphypergraph{\bar t}{D}{Q}$ as a system of constraints over integer variables $X$ and binary variables $B$ as follows.

\smallskip
\noindent
\textbf{The Variables of $\ilphypergraph{\bar t}{D}{Q}$.} For each hyperedge $(\alpha,T)$ of $\downc{R(\bar t)}{D}{\dep}$, the set $X$ contains one integer variable $x_{(\alpha,T)}$. Intuitively, the value of $x_{(\alpha,T)}$ in a solution of $\ilphypergraph{\bar t}{D}{Q}$ denotes the multiplicity of $(\alpha,T)$ in the underlying multiset that is a description of a proof tree of $R(\bar t)$ w.r.t.\ $D$ and $\dep$ with some support $D'$. Let us denote this multiset as $E^*$. In particular, when $x_{(\alpha,T)}$ is $0$, it means that the hyperedge is not part of $E^*$ at all. 
%
Moreover, assuming $\hat{E}$ denotes the set of (standard) edges induced by the hyperedges of $\downc{R(\bar t)}{D}{\dep}$, i.e., 
$\hat{E} = \{(\alpha,\beta) \mid (\alpha,\{\ldots,\beta,\ldots\}) \in E\}$,
%$\hat{E} = \{(\alpha,\beta) \mid (\alpha,\multiset{\ldots,\beta,\ldots}) \in E\}$, 
$X$ contains an integer variable 
$y_{(\alpha,\beta)}$, for each edge $(\alpha,\beta) \in \hat{E}$. Such a variable will be used in some constraints of $\ilphypergraph{\bar t}{D}{Q}$ to guarantee that $R(\bar t)$ reaches all nodes of $\hypergraphof{E^*}$.
Finally, the set $B$ contains one binary variable $z_\alpha$ for each fact $\alpha \in V \cup D$.

% each node $\alpha \in V$ of $\downc{R(\bar t)}{D}{\dep}$.

\smallskip
\noindent
\textbf{The Constraints of $\ilphypergraph{\bar t}{D}{Q}$.} We now move to the constraints. In particular, the system $\ilphypergraph{\bar t}{D}{Q}$ is a set of constraints of the form
$$ T_{\mathsf{degree}} \cup T_{\mathsf{reach}} \cup T_{\mathsf{bind}}.$$
The constraints of $T_{\mathsf{degree}}$ force the in and out degrees of the nodes of the multiset $E^*$ to enjoy the properties (1)-(3) of Definition~\ref{def:hypergraph-properties}. 
%
The constraints $T_{\mathsf{reach}}$ enforce property (4) of Definition~\ref{def:hypergraph-properties}, i.e., that $R(\bar t)$ reaches all nodes of $\hypergraphof{E^*}$; this latter set exploits the variables of the form $y_{(\alpha,\beta)}$ discussed above.
%
Finally, the constraints of $T_\mathsf{bind}$ simply force each binary variable $z_\alpha$ with $\alpha \in V$ to be true iff at least one hyperedge mentioning $\alpha$ belongs to $E^*$, and in case $\alpha \not \in V$, i.e., $\alpha \in D \setminus V$, force $z_\alpha$ to be always false; this is needed to enforce property~(5) of Definition~\ref{def:hypergraph-properties}, guaranteeing that only database facts occurring in $V$ can form a member of $\allwhy{\bar t}{D}{Q}$.\footnote{Note that we do not refer to any specific set $D'$ of facts when implementing property~(5) of Definition~\ref{def:hypergraph-properties}. This is because we want the solutions of our system to induce all possible members of $\allwhy{\bar t}{D}{Q}$, rather than a specific database $D'$.} We proceed to formalize the above informal description.


%\footnote{Note that no constraint enforces property (5) of Definition~\ref{def:hypergraph-properties}, since we want the solutions of our system to induce all possible members of $\allwhy{\bar t}{D}{Q}$, rather than a specific one. Such a property will be crucial, however, for proving that $\ilphypergraph{\bar t}{D}{Q}$ is indeed an ILP encoding of $\allwhy{\bar t}{D}{Q}$.}


For each node $\alpha \in V$ of $\downc{R(\bar t)}{D}{\dep}$, 
let $\mathcal{I}_\alpha$ and $\mathcal{O}_\alpha$ be the following expressions:
$$
\mathcal{I}_\alpha = \sum\limits_{(\beta,T) \in E \text{ with } \alpha \in T} x_{(\beta,T)} \qquad \qquad 
\mathcal{O}_\alpha = \sum\limits_{(\alpha,T) \in E} x_{(\alpha,T)}.
$$
%$$
%\mathcal{I}_\alpha = \sum\limits_{(\beta,T) \in E} \card{\alpha}{T} \cdot x_{(\beta,T)} \qquad \qquad 
%\mathcal{O}_\alpha = \sum\limits_{(\alpha,T) \in E} x_{(\alpha,T)}.
%$$
The expressions $\mathcal{I}_\alpha$ and $\mathcal{O}_\alpha$ essentially compute the integers $\indegree{\alpha}{E^*}$ and $\outdegree{\alpha}{E^*}$, respectively. With those expressions in place, $T_{\mathsf{degree}}$ and $T_\mathsf{bind}$ are easily defined. In particular, $T_\mathsf{degree}$ is the set
\begin{multline*}
	\left\{ \mathcal{O}_{R(\bar t)} - \mathcal{I}_{R(\bar t)} = 1 \right\} \cup \\
	\left\{ \mathcal{O}_\alpha - \mathcal{I}_\alpha = 0\mid \alpha  \in V \setminus (D \cup \{R(\bar t)\})\right\} \cup \\
	\left\{ \sum\limits_{\alpha \in V \cap D} \mathcal{I}_\alpha \ge 1 \right\},
\end{multline*}
whereas $T_\mathsf{bind}$ is the set of constraints
$$ \left\{ z_\alpha \equiv \mathcal{I}_\alpha + \mathcal{O}_\alpha \ge 1 \mid \alpha \in V \right\} \cup \left\{z_\alpha = 0 \mid \alpha \in D \setminus V \right\}.$$ 

We are now only left to explain how $T_\mathsf{reach}$ is constructed. For this, we exploit the variables of the form $y_{(\alpha,\beta)}$, for each $(\alpha,\beta) \in \hat{E}$. Intuitively, each variable $y_{(\alpha,\beta)}$ denotes the amount of ``flow'' the edge carries when traversing it. The constraints of $T_\mathsf{reach}$ will exploit these variables to solve the reachability problem on the (standard) directed graph induced by the hyperedges of $E^*$. We do this using a flow-based encoding. Informally, $T_\mathsf{reach}$ will enforce three constraints (i) every edge $(\alpha,\beta) \in \hat{E}$ either carries zero flow when $\alpha$ does not appear in $E^*$, or it can carry an amount of flow that is enough to be distributed to all other nodes, (ii) the net outgoing flow of node $R(\bar t)$, i.e., the difference between the total outgoing flow and the total incoming flow of $R(\bar t)$, is enough to be distributed \emph{evenly} to all other nodes of $E^*$, and (iii) for every other node $\alpha$ that appears in $E^*$, the total outgoing flow of $\alpha$ must decrease by 1 w.r.t.\ the total incoming flow of $\alpha$ (this is to guarantee that $\alpha$ consumes precisely its share of the total flow).

We now formalize the above intuitive discussion.
%
For a node $\alpha \in V$, let $\inflow{\alpha}$ and $\outflow{\alpha}$ be the following expressions:
$$ \inflow{\alpha} = \sum\limits_{(\beta,\alpha) \in \hat{E}} y_{(\beta,\alpha)} \qquad \qquad \outflow{\alpha} = \sum\limits_{(\alpha,\beta) \in \hat{E}} y_{(\alpha,\beta)},$$
denoting the total incoming and outgoing flow of node $\alpha$, respectively.
%
The set $T_\mathsf{reach}$ is defined as follows\footnote{Note that, for the sake of clarity, the constraints do not strictly follow the syntax defined in Section~\ref{sec:ILP} for linear constraints, since we allow linear expressions on both sides of the (in)equalities. However, these can be easily converted to constraints of the form $a_1 x_1 + \cdots + a_n x_n \diamond a_0$, in the obvious way.}:
\begin{multline*}
	\left\{ y_{(\alpha,\beta)} \le (|V| - 1) \cdot z_\alpha \mid (\alpha,\beta) \in \hat{E} \right\} \cup \\
	\left\{ \outflow{R(\bar t)} - \inflow{R(\bar t)} = \sum\limits_{\alpha \in V} z_\alpha - 1 \right\} \cup \\
	\left\{ \outflow{\alpha} = \inflow{\alpha} - z_\alpha \mid \alpha \in V \setminus \{R(\bar t)\} \right\}.
\end{multline*}

This completes the definition of $\ilphypergraph{\bar t}{D}{Q}$ and we can formally show that is an ILP encoding of why-provenance:
%We now formally show that is complete, and we can prove our crucial result:



\begin{theorem}\label{thm:hyper-correct}
	Consider a Datalog query $Q = (\dep,R)$, a database $D = \{\alpha_1,\ldots,\alpha_n\}$ over $\esch{\dep}$, and a tuple $\bar t \in \adom{D}^{\arity{R}}$. The system of ILP constraints $\ilphypergraph{\bar t}{D}{Q}$ is an ILP encoding of $\allwhy{\bar t}{D}{Q}$ with database variables $z_{\alpha_1},\ldots,z_{\alpha_n}$.
\end{theorem}
\begin{proof}
	\textcolor{red}{Missing...}
\end{proof}

\noindent
\underline{\textbf{Unambiguous Hypergraph-based ILP Encoding}}

\smallskip
\noindent In what follows, fix a Datalog query $Q=(\dep,R)$, a database $D$ over $\esch{\dep}$, a tuple $\bar t \in \adom{D}^{\arity{R}}$, and assume $\downc{R(\bar t)}{D}{\dep} = (V,E)$.
We proceed to show how to construct the ILP encoding of $\unwhy{\bar t}{D}{Q}$. Recall that the unambiguous hypergraph-based characterization only requires one additional property compared to the hypergraph-based characterization. Hence, we can easily define the ILP encoding of $\unwhy{\bar t}{D}{Q}$, dubbed $\ilpunhypergraph{\bar t}{D}{Q}$, by simply adding the required constraints to $\ilphypergraph{\bar t}{D}{Q}$.
%
Let $X$ and $B$ be the sets of integer and binary variables, respectively, of $\ilphypergraph{\bar t}{D}{Q}$. 
%
Now, the variables of 
%We obtain 
$\ilpunhypergraph{\bar t}{D}{Q}$ are $X \cup B \cup B'$, where $B'$ is the set of binary variables
%by extending $\ilphypergraph{\bar t}{D}{Q}$ with an additional set $B'$ 
%of binary variables of the form
\[
\{\hat{x}_{(\alpha,T)} \mid (\alpha,T) \in E\}.
\]
Intuitively, in a solution of $\ilpunhypergraph{\bar t}{D}{Q}$, which induces a multiset $E^*$ of hyperedges of $\downc{R(\bar t)}{D}{\dep}$ that is a description of an unambiguous proof tree of $R(\bar t)$ w.r.t.\ $D$ and $\dep$ with some support $D'$, each variable $\hat{x}_{(\alpha,T)}$ is true iff the hyperedge $(\alpha,T)$ occurs in $E^*$. 
%Hence, $\ilpunhypergraph{\bar t}{D}{Q}$ is over the integer variables $X$ and the binary variables $B \cup B'$. 
Finally, $\ilpunhypergraph{\bar t}{D}{Q}$ is defined as
%the set of constraints of the form
\[
\ilphypergraph{\bar t}{D}{Q} \cup T_{\mathsf{UN}},
\]
where $T_{\mathsf{UN}}$ is the set of constraints enforcing the additional required condition, that is, no two hyperedges $(\alpha,T),(\alpha,T')$ appear in $E^*$ with $T \neq T'$. This is achieved by defining $T_{\mathsf{UN}}$ as follows:
\[
	\left\{ \hat{x}_{(\alpha,T)} \equiv x_{(\alpha,T)} \ge 1 \mid (\alpha,T) \in E \right\} \cup 
	\left\{ \sum\limits_{(\alpha,T) \in E} \hat{x}_{(\alpha,T)} \le 1 \mid \alpha \in V \right\}.
\]
%\begin{multline*}
%	\left\{ \hat{x}_{(\alpha,T)} \equiv x_{(\alpha,T)} \ge 1 \mid (\alpha,T) \in E \right\} \cup \\ \left\{ \sum\limits_{(\alpha,T) \in E} \hat{x}_{(\alpha,T)} \le 1 \mid \alpha \in V \right\}.
%\end{multline*}


We can now formally show that $\ilpunhypergraph{\bar t}{D}{Q}$ is indeed an ILP encoding of why-provenance:
%The crucial result follows:
\begin{theorem}\label{thm:un-hyper-correct}
	Consider a Datalog query $Q = (\dep,R)$, a database $D = \{\alpha_1,\ldots,\alpha_n\}$ over $\esch{\dep}$, and a tuple $\bar t \in \adom{D}^{\arity{R}}$. The system of ILP constraints $\ilpunhypergraph{\bar t}{D}{Q}$ is an ILP encoding of $\unwhy{\bar t}{D}{Q}$ with database variables $z_{\alpha_1},\ldots,z_{\alpha_n}$.
\end{theorem}
\begin{proof}
	\textcolor{red}{Missing...}
\end{proof}


\subsection{Graph-based ILP Encodings}\label{sec:proofdag-based}

We now recall the characterizations of when there exists an (unambiguous) proof tree of some fact $R(\bar t)$ w.r.t.~some database $D$ and Datalog program $\dep$ with some support $D'$ that rely on the existence of a directed acyclic graph (DAG) with certain properties, called a proof DAG of $R(\bar t)$ w.r.t.~$D$ and $\dep$, and then use them to devise the graph-based ILP encodings of why-provenance.


\medskip
\noindent
\underline{\textbf{Graph-based Characterizations}}

\smallskip
\noindent 
%In this last section we recall the other characterizations for the existence of an (unambiguous) proof tree of some fact $R(\bar t)$ w.r.t.\ some database $D$ and Datalog program $\dep$ with some support $D'$. These characterizations rely on the existence of a directed acyclic graph (DAG) with certain properties, called a proof DAG of $R(\bar t)$ w.r.t.\ $D$ and $\dep$. Roughly, a proof DAG is a compact way of encoding a proof tree. 
%
The characterizations of interest state that every (unambiguous) proof tree admits a corresponding (unambiguous) proof DAG $G$, where for each fact $\alpha$, only a ``small'' number of nodes of $G$ are labeled with $\alpha$. In fact, in the case of arbitrary proof DAGs, this number is bounded by a certain polynomial that depends on some parameters of the downward closure of $\alpha$ w.r.t.~$D$ and $\dep$, whereas in the case of unambiguous proof DAGs, this number is either $0$ or $1$.
%the number of nodes of the proof DAG labeled with $\alpha$ is bounded by a certain polynomial, and this polynomial depends on the family of proof trees we consider and on some parameters of the downward closure of $\alpha$ w.r.t.~$D$ and $\dep$.
%
We proceed to recall (unambiguous) proof DAGs and then present the actual characterizations. We recall that a DAG $G$ is \emph{rooted} if it has exactly one node, the \emph{root}, with no incoming edges. A node of $G$ is a \emph{leaf} if it has no outgoing edges.

\begin{definition}[\textbf{(Unambiguous) Proof DAG}]\label{def:proof-dag}
	Consider a Datalog program $\dep$, a database $D$ over $\esch{\dep}$, and a fact $\alpha$ over $\sch{\dep}$. A \emph{proof DAG} of $\alpha$ w.r.t.\ $D$ and $\dep$ is a finite labeled rooted DAG $G = (V,E,\lambda)$, with $\lambda : V \rightarrow \base{D,\dep}$, such that:
	\begin{enumerate}
		\item If $v \in V$ is the root, then $\lambda(v) = \alpha$.
		
		\item If $v \in V$ is a leaf, then $\lambda(v) \in D$.
		
		\item If $v \in V$ has $n\ge1$ outgoing edges $(v,u_1),\ldots,(v,u_n)$, then there exists a rule $R_0(\bar x_0)\ \assign\ R_1(\bar x_1),\ldots,R_n(\bar x_n) \in \dep$ and a function $h : \bigcup_{i \in [n]} \bar x_i \ra \ins{C}$ such that $\lambda(v) = R_0(h(\bar x_0))$, and $\lambda(u_i) = R_i(h(\bar x_i))$ for each $i \in [n]$. 
	\end{enumerate}
    We say that $G$ is an \emph{unambiguous proof DAG of $\alpha$ w.r.t.~$D$ and $\dep$} if, in addition to the above conditions, for every two nodes $u,v \in V$, it holds that $\lambda(u) = \lambda(v)$ implies $u=v$. \hfill\markfull
\end{definition}

The difference between a proof tree and a proof DAG is that a proof DAG might reuse nodes to compactly represent a proof tree. In fact, every proof tree is a proof DAG where each node has at most one parent. As for proof trees, given a proof DAG $G$ (of some fact w.r.t. some database and Datalog program), its support, denoted $\support{G}$, is the set of facts that label the leaves of $G$.


We can now recall the desired graph-based characterizations. In the following, assuming $\downc{R(\bar t)}{D}{\dep} = (V,E)$, for some  Datalog program $\dep$, database $D$ over $\esch{\dep}$, and fact $R(\bar t)$, let 
\begin{eqnarray*}
\boundall{R(\bar t)}{D}{\dep} &=& ( |V| \cdot d + 1) \cdot d \cdot b,\\
\boundun{R(\bar t)}{D}{\dep} &=& 1,
\end{eqnarray*}
where $d = |V \cap D|$, i.e., $d$ is the number of nodes of $\downc{R(\bar t)}{D}{\dep}$ that correspond to database facts, and $b = \max\{|T| \mid (\alpha,T) \in E\}$ is the maximum ``branching'' of a hyperedge of $\downc{R(\bar t)}{D}{\dep}$.

%the downward closure.
%Finally, we let $\boundun{R(\bar t)}{D}{\dep} = 1$.

\begin{theorem}[\cite{CLPS24,CLPS24aaai}]\label{thm:arbitrary-proof-dag}
	Consider a Datalog query $Q=(\dep,R)$, a database $D$ over $\esch{\dep}$, a tuple $\bar t \in \adom{D}^{\arity{R}}$, and a database $D' \subseteq D$. The following are equivalent:
	\begin{enumerate}
		\item There is a proof tree (resp., an unambiguous proof tree) $T$ of $R(\bar t)$ w.r.t.\ $D$ and $\dep$ with support $D'$.
		\item There is a proof DAG (resp., an unambiguous proof DAG) $G = (V,E,\lambda)$ of $R(\bar t)$ w.r.t.\ $D$ and $\dep$ with support $D'$ such that the following hold:
		\begin{enumerate}
			\item For each $v \in V$, $\lambda(v)$ is a node of $\downc{R(\bar t)}{D}{\dep}$.
			\item For each $v \in V$ with outgoing edges $(v,u_1),\ldots,(v,u_n)$,
			$(\lambda(v),\{\lambda(u_1),\ldots,\lambda(u_n)\})$ belongs to $\downc{R(\bar t)}{D}{\dep}$.
%			$(\lambda(v),\multiset{\lambda(u_1),\ldots,\lambda(u_n)})$ belongs to $\downc{R(\bar t)}{D}{\dep}$.
			\item For each fact $\alpha$, it holds that $|\{v \in V \mid \lambda(v) = \alpha\}| \le \boundall{R(\bar t)}{D}{\dep}$ (resp., $\boundun{R(\bar t)}{D}{\dep}$).\hfill\markfull
		\end{enumerate} 
	\end{enumerate}
\end{theorem}

\begin{comment}
We call the above result the \emph{proof DAG-based characterization}.
The characterization for unambiguous proof trees, which we dub \emph{unambiguous proof DAG-based characterization}, is similar. The only difference is that the number of nodes in the proof DAG labeled with a certain fact $\alpha$ must be one. That is:

\begin{theorem}[\cite{CLPS24,CLPS24aaai}]\label{thm:unambiguous-proof-dag}
	Consider a Datalog query $Q=(\dep,R)$, a database $D$ over $\esch{\dep}$, a tuple $\bar t \in \adom{D}^{\arity{R}}$, and a database $D' \subseteq D$. The following are equivalent:
	\begin{enumerate}
		\item There is an unambiguous proof tree $T$ of $R(\bar t)$ w.r.t.\ $D$ and $\dep$ with support $D'$.
		\item There is a proof DAG $G = (V,E,\lambda)$ of $R(\bar t)$ w.r.t.\ $D$ and $\dep$ with support $D'$ such that the following hold:
		\begin{enumerate}
			\item For each $v \in V$, $\lambda(v)$ is a node of $\downc{R(\bar t)}{D}{\dep}$.
			\item For each $v \in V$ with outgoing edges $(v,u_1),\ldots,(v,u_n)$,
			$(\lambda(v),\{\lambda(u_1),\ldots,\lambda(u_n)\})$ belongs to $\downc{R(\bar t)}{D}{\dep}$.
%			$(\lambda(v),\multiset{\lambda(u_1),\ldots,\lambda(u_n)})$ belongs to $\downc{R(\bar t)}{D}{\dep}$.
			\item For each fact $\alpha$, it holds that $|\{v \in V \mid \lambda(v) = \alpha\}| \le 1$.\hfill\markfull
		\end{enumerate} 
	\end{enumerate}
\end{theorem}
\end{comment}


Let us now discuss how Theorem~\ref{thm:arbitrary-proof-dag} can be used in order to devise an ILP encoding of why-provenance. 
%, given a Datalog query $Q = (\dep,R)$, a database $D$ over $\esch{\dep}$, and a tuple $\bar t \in \adom{D}^{\arity{R}}$, 
%how to use  Theorem~\ref{thm:arbitrary-proof-dag} to devise an ILP encoding of why-provenance.
%$\starwhy{\bar t}{D}{Q}$, where $\star \in \{\mathsf{ALL},\mathsf{UN}\}$.

%As we did for the hypergraph-based characterizations, we now show how to use the above proof DAG-based characterizations to devise ILP encodings for $\allwhy{\bar t}{D}{Q}$ and $\unwhy{\bar t}{D}{Q}$, for a given Datalog query $Q = (\dep,R)$, database $D$ over $\esch{\dep}$, and tuple $\bar t \in \adom{D}^{\arity{R}}$.

\medskip
\noindent
\underline{\textbf{Graph-based ILP Encoding}}

\smallskip
\noindent Fix a Datalog query $Q=(\dep,R)$, a database $D$ over $\esch{\dep}$, a tuple $\bar t \in \adom{D}^{\arity{R}}$, and let $\downc{R(\bar t)}{D}{\dep} = (V,E)$.
We start with the ILP encoding for $\allwhy{\bar t}{D}{Q}$, which we dub the \emph{graph-based ILP encoding of $\allwhy{\bar t}{D}{Q}$}, and denote it by $\ilpproofdag{\bar t}{D}{Q}$. The encoding is a direct implementation of Theorem~\ref{thm:arbitrary-proof-dag}, namely the set of constraints $\ilpproofdag{\bar t}{D}{Q}$ searches for a proof DAG of $R(\bar t)$ w.r.t.\ $D$ and $\dep$ with \emph{some} support, where no more than $\boundall{R(\bar t)}{D}{\dep}$ nodes are labeled with the same fact.
%
Formally, we construct $\ilpproofdag{\bar t}{D}{Q}$ as a system of constraints over integer variables $X$ and binary variables $B$ as follows.

\medskip
\noindent
\textbf{The Variables of $\ilpproofdag{\bar t}{D}{Q}$.} Let $\hat{E}$ be the set of (standard) edges induced by the hyperedges of $\downc{R(\bar t)}{D}{\dep}$, i.e., 
$\hat{E} = \{(\alpha,\beta) \mid (\alpha,\{\ldots,\beta,\ldots\}) \in E\}$. For a fact $\alpha$,
%node $\alpha \in V$ of $\downc{R(\bar t)}{D}{\dep}$, 
%
an \emph{amplified copy of $\alpha$} is an expression of the form $\alpha^i$, with $i \in [\boundall{R(\bar t)}{D}{\dep}]$. Moreover, for a hyperedge $(\alpha,T) \in E$, with $T = \{\beta_1,\ldots,\beta_n\}$, of $\downc{R(\bar t)}{D}{\dep}$, an \emph{amplified copy of $(\alpha,T)$} is an expression of the form $(\alpha^i,T')$, with $T' = \{\beta_1^{k_1},\ldots,\beta_n^{k_n}\}$, where $\alpha^i$ is an amplified copy of $\alpha$, and $\beta_j^{k_j}$ is an amplified copy of $\beta_j$, for $j \in [n]$. We can now discuss how the variables of $\ilpproofdag{\bar t}{D}{Q}$ are defined.

The set $X$ is empty, whereas $B$ is the union of three disjoint sets $B_N$, $B_H$, and $B_E$ defined as follows:
\begin{itemize}
\item[-] The set $B_N$ contains a binary variable $x_{\alpha^i}$ for each amplified copy $\alpha^i$ of a fact $\alpha \in V \cup D$. 

\item[-] The set $B_H$ contains a binary variable $y_{(\alpha^i,T')}$ for each amplified copy $(\alpha^i,T')$ of an hyperedge $(\alpha,T) \in E$.

\item[-] The set $B_E$ contains a binary variable $z_{(\alpha^i,\beta^j)}$ for each pair of amplified copies $\alpha^i,\beta^j$ of facts $\alpha,\beta$ such that $(\alpha,\beta) \in \hat{E}$.
\end{itemize}

\noindent 
Intuitively, when $x_{\alpha^i}$ is true, for a fact $\alpha \in V \cup D$, it means that a node of the underlying proof DAG $G$ is labeled with $\alpha$, and among all nodes of $G$ labeled with $\alpha$, this node has $i$ as its identifier. In other words, $\alpha^i$ is the unique name of such a node labeled with $\alpha$ in $G$.
%
Moreover, the variables of $B_N$ and $B_E$ that become true via a solution of $\ilpproofdag{R(\bar t)}{D}{\dep}$ induce the nodes and the edges of a proof DAG $G$ for $R(\bar t)$ w.r.t.~$D$ and $\dep$, where each true variable of the form $x_{\alpha^i}$ means that among all possible nodes of a proof DAG that can be labeled with $\alpha$, the node with identifier $i$ is part of $G$, and a true variable of the form $z_{(\alpha^i,\beta^j)}$ means that the node with identifier $i$ labeled with $\alpha$ and the node with identifier $j$ labeled with $\beta$ are connected by an edge in $G$.


\medskip
\noindent
\textbf{The Constraints of $\ilpproofdag{\bar t}{D}{Q}$.} We now move to the constraints. In particular, the system $\ilpproofdag{\bar t}{D}{Q}$ is a set of constraints of the form
%
\[
T_{\mathsf{graph}} \cup T_{\mathsf{root}} \cup T_{\mathsf{proof}} \cup T_{\mathsf{acyclic}}.
\]


The set of constraints $T_{\mathsf{graph}}$ is in charge of guaranteeing consistency between the truth value of the variables in $B_N$ and the variables in $B_E$, i.e., if an edge between two nodes is part of $G$, then the two nodes must belong to $G$ as well. Formally, $T_{\mathsf{graph}}$ is the set
\[
\left\{ z_{(\alpha^i,\beta^j)} \le x_{\alpha^i} \mid z_{(\alpha^i,\beta^j)} \in B_E \right\}\ \cup\
 \left\{ z_{(\alpha^i,\beta^j)} \le x_{\beta^j} \mid z_{(\alpha^i,\beta^j)} \in B_E \right\}.
\]


The set of constraints $T_{\mathsf{root}}$ guarantees that $G$ contains a distinguished node labeled with the fact $R(\bar t)$, which is the root of $G$, and no other node of $G$ can be the root (i.e., every other node must have at least one incoming edge). For this, we pick $R(\bar t)^1$, which we denote as $\rho$, as the representative node labeled with $R(\bar t)$ to play the role of the root. Formally, $T_{\mathsf{root}}$ is the set
\begin{multline*}
	\{x_{\rho} = 1\} \cup
	\left\{ z_{(\alpha^i,\rho)} = 0 \mid z_{(\alpha^i,\rho)} \in B_E \right\} \cup \\
	\left\{ x_{\alpha^i} \le \sum\limits_{ z_{(\beta^j,\alpha^i)} \in B_E} z_{(\beta^j,\alpha^i)} \mid x_{\alpha^i} \in B_N \text{ with } \alpha \in V \text{ and } \alpha^i \neq \rho \right\}.
\end{multline*}



We now discuss $T_{\mathsf{proof}}$. Roughly, this set of constraints is in charge of guaranteeing that the nodes and edges induced by the true variables of $B_N$ and $B_E$ form a valid proof DAG. For this, the constraints ensure, for each fact $\alpha \in D \setminus V$, that each variable of the form $x_{\alpha^i}$ is always false, and, for all other facts $\alpha \in V$, ensure that (i) when a node $\alpha^i$ belongs to $G$, i.e., it is a node labeled with $\alpha$, and (ii) $\alpha$ is an intensional atom $\alpha$, then $\alpha^i$ must have the correct children in $G$. The latter means that the labels of the children of $\alpha^i$ form the target of some hyperedge of $\downc{R(\bar t)}{D}{Q}$ having $\alpha$ as the source. Moreover, no other nodes can be the children of $\alpha^i$.
% 
This is achieved with two families of constraints in $T_{\mathsf{proof}}$. The first set of constraints is in charge of choosing which nodes should the children of $\alpha^i$ in $G$, assuming $\alpha^i$ occurs in $G$. This is done by forcing one of the variables of the form $y_{(\alpha^i,T)} \in B_H$ to be true, whenever $x_{\alpha^i}$ is true. The second set of constraints guarantees that whenever the variable $y_{(\alpha^i,T)} \in B_H$ is true, \emph{all and only} the nodes in $T$ are children of $\alpha^i$ in $G$. Formally, $T_{\mathsf{proof}}$ is the set
\begin{multline*}
	\left\{x_{\alpha^i} = 0 \mid \alpha \in D \setminus V \right\} \cup \\ 
	\left\{ x_{\alpha^i} \le \sum\limits_{y_{(\alpha^i,T)} \in B_H} y_{(\alpha^i,T)} \mid x_{\alpha^i} \in B_N \text{ with }  \alpha \in V \text{ intensional }\right\} \cup  \\
	\left\{ y_{e} \le \ell_{e,\beta^j} \mid y_{e} \in B_H \text{ with } e = (\alpha^i,T) \text{ and } z_{(\alpha^i,\beta^j)} \in B_E \right\},
\end{multline*}
where, for each $e=(\alpha^i,T)$, $\ell_{e,\beta^j}$ denotes $z_{(\alpha^i,\beta^j)}$ if $\beta^j \in T$, and $1- z_{(\alpha^i,\beta^j)}$ otherwise.
%

We finally discuss $T_{\mathsf{acyclic}}$, which is in charge of checking that $G$, namely the graph whose edges correspond to the true variables in $B_E$, is acyclic.
%
Checking the acyclicity of a graph via a set of constraints over binary variables defining the edges of the graph is a well-studied problem in different fields with a plethora of encodings. For our construction, we employ an encoding based on vertex elimination~\cite{RankoohR22}, which is much more efficient than other encodings that compute the full transitive closure of the graph.

This completes the definition of $\ilpproofdag{\bar t}{D}{Q}$ and we can formally show that is an ILP encoding of why-provenance:

%The construction of $\ilpproofdag{\bar t}{D}{Q}$ is now complete, and we can prove the key result of this section:

\begin{theorem}\label{thm:dag-correct}
	Consider a Datalog query $Q = (\dep,R)$, a database $D = \{\alpha_1,\ldots,\alpha_n\}$ over $\esch{\dep}$, and a tuple $\bar t \in \adom{D}^{\arity{R}}$. The system of ILP constraints $\ilpproofdag{\bar t}{D}{Q}$ is an ILP encoding of $\allwhy{\bar t}{D}{Q}$ with database variables $x_{\alpha_1^1},\ldots,x_{\alpha^1_n}$.
\end{theorem}
\begin{proof}
	\textcolor{red}{Missing...}
\end{proof}

%\medskip
\noindent
\underline{\textbf{Unambiguous Graph-based ILP Encoding}}

\smallskip
\noindent Consider a Datalog query $Q=(\dep,R)$, a database $D$ over $\esch{\dep}$, and a tuple $\bar t \in \adom{D}^{\arity{R}}$.
%, and assume $\downc{R(\bar t)}{D}{\dep} = (V,E)$. 
We proceed to show how to construct the ILP encoding of $\unwhy{\bar t}{D}{Q}$.
%
Recall that the only difference between the graph-based and the unambiguous graph-based characterization, both presented in Theorem~\ref{thm:arbitrary-proof-dag}, concerns only the number of nodes in the proof DAG that can be labeled with the same fact; for unambiguous proof DAGs this bound is $1$.
%We observe that the only difference between the graph-based characterization of Theorem~\ref{thm:arbitrary-proof-dag}, and the unambiguous graph-based characterization of Theorem~\ref{thm:unambiguous-proof-dag} regards only the number of nodes in the proof DAG that can be labeled with the same fact; for unambiguous proof DAGs, this bound is one. 
Hence, we can define the ILP encoding of $\unwhy{\bar t}{D}{Q}$, called $\ilpunproofdag{\bar t}{D}{Q}$, by adopting the same construction of $\ilpproofdag{\bar t}{D}{Q}$ with the difference that each fact $\alpha$ admits exactly one amplified copy, i.e., the amplified copy $\alpha^1$. We can the show the following:
%Our last key result follows:


\begin{theorem}\label{thm:unambiguous-dag-correct}
	Consider a Datalog query $Q = (\dep,R)$, a database $D = \{\alpha_1,\ldots,\alpha_n\}$ over $\esch{\dep}$, and a tuple $\bar t \in \adom{D}^{\arity{R}}$. The system of ILP constraints $\ilpunproofdag{\bar t}{D}{Q}$ is an ILP encoding of $\unwhy{\bar t}{D}{Q}$ with database variables $x_{\alpha_1^1},\ldots,x_{\alpha^1_n}$.
\end{theorem}

\begin{proof}
	\textcolor{red}{Missing...}
\end{proof}

==> figures/complexity.tex <==
\section{Diverse Why-Provenance}
\label{sec:diverse-why-provenance}

As discussed in the Introduction, our goal is, given a Datalog query $Q = (\dep,R)$, a database $D$ over $\esch{\dep}$, and a tuple ${\bar t} \in \adom{D}^{\arity{R}}$, to compute a set of $k > 0$ diverse explanations of why $\bar t \in Q(D)$ according to the notion of why-provenance (relative to arbitrary or unambiguous proof trees) introduced in the previous section. 
%
To formalize this task, we transfer the general diversity framework from~\cite{AMPR24} to the setting of why-provenance.


Consider a non-empty subset $\mathcal{S}$ of $\starwhy{\bar t}{D}{Q}$, where $\star \in \{\mathsf{ALL},\mathsf{UN}\}$, if it exists. To determine the diversity of $\mathcal{S}$, we first determine how different the pairs of databases are in $\mathcal{S}$. This is done by using their symmetric difference. For two databases $D_1,D_2 \in \mathcal{S}$, the \emph{symmetric difference between $D_1$ and $D_2$}, denoted $\diff{D_1}{D_2}$, is the set $(D_1 \setminus D_2) \cup (D_2 \setminus D_1)$. We then define the \emph{distance between $D_1$ and $D_2$}, written $\dist{D_1}{D_2}$, as the integer $|\diff{D_1}{D_2}|$. Finally, the \emph{diversity of $\mathcal{S} = \{D_1,\ldots,D_k\}$}, denoted $\diversity{\mathcal{S}}$, is defined as
\[
\sum\limits_{i,j \in [|\mathcal{S}|] \text{ and }i<j} \dist{D_i}{D_j}.
\]


We are now ready to introduce the main problems of interest. For a Datalog query $Q = (\dep,R)$, a database $D$ over $\esch{\dep}$, a tuple $\bar t \in \adom{D}^{\arity{R}}$, and an integer $k > 0$, we write $\starwhyk{k}{\bar t}{D}{Q}$, for $\star \in \{\mathsf{ALL},\mathsf{UN}\}$, to denote the collection of all sets $\mathcal{S} \subseteq \starwhy{\bar t}{D}{Q}$ with $|\mathcal{S}| = k$, i.e., each element of $\starwhyk{k}{\bar t}{D}{Q}$ contains exactly $k$ members of $\starwhy{\bar t}{D}{Q}$. 
%
The main problems of interest are optimization problems that essentially ask to compute a set of $\starwhyk{k}{\bar t}{D}{Q}$ with maximal diversity:

\medskip

\begin{center}
	\fbox{\begin{tabular}{ll}
			{\small PROBLEM} : & $\star\text{-}\mathsf{DiverseWhyProvenance}$
			\\[2mm]
			{\small INPUT} : & A Datalog query $Q = (\dep,R)$, \\
			& a database $D$ over $\esch{\dep}$,\\
			& a tuple ${\bar t} \in \adom{D}^{\arity{R}}$, and\\
			& an integer $k > 0$\\[2mm]
			{\small OUTPUT} : & A member of $\argmax\limits_{\mathcal{S} \in \starwhyk{k}{\bar t}{D}{Q}} \diversity{\mathcal{S}}$ if it exists;\\
			&  otherwise \textbf{fail} 
	\end{tabular}}
\end{center}

\medskip

Let us clarify that there may be several sets $\mathcal{S} \in \starwhyk{k}{\bar t}{D}{Q}$ with maximal diversity. Our problems simply ask to compute one of those sets.
%
Observe that in the above definition all the relevant components are part of the input, but we are also interested in the scenario where the Datalog query is fixed. In other words, for each Datalog query $Q = (\dep,R)$, we are interested in the problem:  



\medskip

\begin{center}
	\fbox{\begin{tabular}{ll}
			{\small PROBLEM} : & $\star\text{-}\mathsf{DiverseWhyProvenance}[Q]$
			\\[2mm]
			{\small INPUT} : & A database $D$ over $\esch{\dep}$,\\
			& a tuple ${\bar t} \in \adom{D}^{\arity{R}}$, and\\
			& an integer $k > 0$\\[2mm]
			{\small OUTPUT} : & A member of $\argmax\limits_{\mathcal{S} \in \starwhyk{k}{\bar t}{D}{Q}} \diversity{\mathcal{S}}$ if it exists;\\
			&  otherwise \textbf{fail} 
	\end{tabular}}
\end{center}

\medskip

We proceed to show that we are dealing with intractable optimization problems, no matter the underlying class of proof trees (arbitrary or unambiguous), even if the Datalog query is fixed and consists of a single Datalog rule.

\begin{theorem}\label{the:diversity-complexity}
For each $\star \in \{\mathsf{ALL},\mathsf{UN}\}$, there exists a Datalog query $Q = (\dep,R)$, where $\dep$ consists of a single Datalog rule, such that $\star\text{-}\mathsf{DiverseWhyProvenance}[Q]$ is NP-hard.
\end{theorem}

The rest of the section is devoted to proving the above complexity result. To this end, we first introduce the decision problem of checking whether a fixed Datalog query has $k$ answers over a given database $D$ such that their diversity is above a certain threshold; we know from~\cite{MerklPS25} that this is an NP-hard problem. We then reduce this problem via a polynomial-time Turing reduction to our problems, which in turn establishes Theorem~\ref{the:diversity-complexity}.


\subsection{Diverse Answers}

%\medskip
%\noindent
%\textbf{Diverse Answers.}
Consider an integer $n > 0$. For an $n$-tuple $\bar t = (t_1,\ldots,t_n)$, let $\bar t[i]$ be the term $t_i$, with $i \in [n]$. For two $n$-tuples $\bar t$ and $\bar u$, the \emph{Hamming distance between $\bar t$ and $\bar u$}, denoted $\hammd{\bar t}{\bar u}$, is defined as the integer $|\{i \in [n] \mid  \bar t[i] \neq \bar u[i]\}|$. Moreover, for a set $\mathcal{A} = \{\bar t_1,\ldots,\bar t_k\}$ of $n$-tuples, the \emph{diversity of $\mathcal{A}$}, denoted $\diversitytup{\mathcal{A}}$, is defined as
	\[
	\sum\limits_{i,j \in [|\mathcal{A}|] \text{ and }i<j} \hammd{\bar t_i}{\bar t_j}.
	\]
	
	For a Datalog query $Q = (\dep,R)$, a database $D$ over $\esch{\dep}$, and an integer $k > 0$, we define $\ansk{k}{D}{Q}$ as the collection of all sets $\mathcal{A} \subseteq Q(D)$ of tuples with $|\mathcal{A}| = k$. For a fixed Datalog query $Q = (\dep,R)$, we consider the following decision problem:

    \medskip
    
	\begin{center}
	 	\fbox{\begin{tabular}{ll}
	 			{\small PROBLEM} : & $\mathsf{DiverseAnswersCheck}[Q]$
	 			\\[2mm]
	 			{\small INPUT} : & A database $D$ over $\esch{\dep}$,\\
	 			& an integer $k > 0$ encoded in unary, and \\
	 			& an integer $d \ge 0$\\[2mm]
	 			{\small QUESTION} : & Is there a set $\mathcal{A} \in \ansk{k}{D}{Q}$ with $\diversitytup{\mathcal{A}} \ge d?$
	 	\end{tabular}}
	\end{center}

    \medskip

    We know that there is a Datalog query for which the above problem is NP-hard; this is a consequence of~\cite[Theorem 3.13]{MerklPS25}.

    \begin{theorem}\label{the:diverse-answers}
    $\mathsf{DiverseAnswersCheck}[Q^*]$ is NP-complete, where $Q^* = (\dep^*,R)$ with $\dep^* = \{R(x_1,\ldots,x_5)\ \assign\ P(x_1,\ldots,x_5)\}$.
    \end{theorem}

\subsection{The Reduction}
	%\medskip
	%\noindent
	%\textbf{The Reduction.}
	Consider now the Datalog query $\hat{Q} = (\hat{\dep},\hat{R})$, where $\hat{R}$ is a $0$-ary predicate and $\hat{\dep}$ contains only the rule:
	\[
    \hat{R}\ \assign\ P(x_1,\ldots,x_5),P_1(x_1),\ldots,P_5(x_5).
    \]
	We proceed to show that, for every $\star \in \{\mathsf{ALL},\mathsf{UN}\}$, there exists a polynomial-time Turing reduction from $\mathsf{DiverseAnswersCheck}[Q^*]$ to $\star\text{-}\mathsf{DiverseWhyProvenance}[\hat{Q}]$, i.e., there is a procedure with access to an oracle for the problem $\star\text{-}\mathsf{DiverseWhyProvenance}[\hat{Q}]$ that decides $\mathsf{DiverseAnswersCheck}[Q^*]$ in polynomial time.
	
%	First, we note that for the Datalog query $\hat{Q}$, $\unwhy{\bar t}{D}{\hat{Q}}$ and $\allwhy{\bar t}{D}{\hat{Q}}$ coincide, for every database $D$ over $\esch{\hat{\dep}}$, and (thee only) tuple $\bar t \in \adom{D}^{\arity{\hat{R}}}$. Hence, it is enough to prove the claim for $\star = \mathsf{ALL}$. We now proceed by describing the desired polynomial-time procedure.
	
	%For a database $D$ over $\esch{\dep^*}$, we define the database $\hat{D}$ over $\esch{\hat{\dep}}$ as the set:
	%
	%$$ \hat{D} = D \cup \{P_1(t_1),\ldots,P_5(t_5) \mid P(t_1,\ldots,t_5) \in D\}.$$
	%
	%Fix any $\star \in \{\mathsf{ALL},\mathsf{UN}\}$, and 
    Consider an input to $\mathsf{DiverseAnswersCheck}[Q^*]$, i.e., a database $D$ over $\esch{\dep^*}$, an integer $k > 0$ encoded in unary, and an integer $d \ge 0$.
	%
	The procedure deciding $\mathsf{DiverseAnswersCheck}[Q^*]$, which we dub $\mathsf{DecideDiverseAnswers}$, does the following:
	\begin{enumerate}
		\item Construct the database 
        $$ \hat{D}\ =\ D \cup \{P_1(t_1),\ldots,P_5(t_5) \mid P(t_1,\ldots,t_5) \in D\}.$$
        %$\hat{D}$ over $\esch{\hat{\dep}}$.
		\item Ask the oracle to compute some $\mathcal{\hat{S}}$ in $\argmax\limits_{\mathcal{S} \in \starwhyk{k}{()}{\hat{D}}{\hat{Q}}} \diversity{\mathcal{S}}$. 
		\item If the oracle returns \textbf{fail}, then reject. 
		\item Accept if $\diversity{\mathcal{\hat{S}}} \ge k(k-1) + 2\cdot d$; otherwise, reject.
	\end{enumerate} 
	
	\medskip
	\noindent
	\textbf{Running Time.}
	The procedure $\mathsf{DecideDiverseAnswers}$ clearly runs in polynomial time since constructing $\hat{D}$ only requires iterating over the facts in $D$. Moreover, the set $\mathcal{\hat{S}}$ returned by the oracle, when it exists, contains linearly many elements w.r.t.\ the size of the encoding of $k$, and each element in $\mathcal{\hat{S}}$ is no larger than $|\hat{D}|$. Finally, computing $\diversity{\mathcal{\hat{S}}}$ requires adding $k(k-1)$ symmetric distances, and the number $k(k-1) + 2\cdot d$ can be easily computed.
	
	\medskip
	\noindent
	\textbf{Correctness.} We proceed to show that the procedure indeed decides $\mathsf{DiverseAnswersCheck}[Q^*]$.
    %
    We first make some observations. 	For a $5$-tuple $\bar t$, let $D_{\bar t} = \{P(\bar t),P_1(\bar t[1]),\ldots,P_5(\bar t[5])\}$.
    %
	It is not difficult to verify that by construction of $\hat{D}$ and by definition of $\hat{Q} = (\hat{\dep},\hat{R})$, we have that:
	\begin{observation}\label{obs:why-ans}
		For each $\star \in \{\mathsf{ALL},\mathsf{UN}\}$,
		$$ \starwhy{()}{\hat{D}}{\hat{Q}}\ =\ \{D_{\bar t} \mid \bar t \in Q^*(D)\}.$$
	\end{observation}
	
	Moreover, for two distinct databases $D_{\bar t},D_{\bar u} \in \starwhy{()}{\hat{D}}{\hat{Q}}$, the symmetric difference between $D_{\bar t}$ and $D_{\bar u}$ is of the form
	%
	\begin{multline*}
		\diff{D_{\bar t}}{D_{\bar u}}\ =\ \{P(\bar t),P(\bar u)\} \cup 
		\diff{(D_{\bar t} \setminus \{P(\bar t)\})}{(D_{\bar u} \setminus \{P(\bar u)\})},
	\end{multline*}
	%
	and thus
	$$\dist{D_{\bar t}}{D_{\bar u}}\ =\ |\diff{D_{\bar t}}{D_{\bar u}}|\ =\ 2 + 2 \cdot \hammd{\bar t}{\bar u}.$$
	The above allows us to conclude the following:
	\begin{observation}\label{obs:diversity-ans}
	For each $\mathcal{S} = \{D_{\bar t_1},\ldots,D_{\bar t_k}\} \in \starwhyk{k}{()}{\hat{D}}{\hat{Q}}$, 
    %the diversity of $\mathcal{S}$ is:
	$$\diversity{\mathcal{{S}}} = \sum\limits_{i,j \in [k] \text{ and } i<j} (2 + 2 \cdot \hammd{\bar t_i}{\bar t_j}) = k(k-1) + 2 \cdot \diversitytup{\{\bar t_1,\ldots,\bar t_k\}}.$$
	\end{observation}

	
	We now proceed with the proof of correctness. Let $D$, $k$, and $d$ be an input to $\mathsf{DecideDiverseAnswers}$. 

    \medskip
    
	($\Rightarrow$) Assume first that there exists a set $\mathcal{A} \in \ansk{k}{D}{Q^*}$ with $\diversitytup{\mathcal{A}} \ge d$. We argue that $\mathsf{DecideDiverseAnswers}$ accepts with input $D$, $k$, and $d$. First, note that by the existence of $\mathcal{A}$, there also exists $\mathcal{A}^* \in \argmax\limits_{\mathcal{A} \in \ansk{k}{D}{Q^*}} \diversitytup{\mathcal{A}}$, and all such $\mathcal{A}^*$ have the same diversity which is such that $\diversitytup{\mathcal{A}^*} \ge d$. Let $d^* = \diversitytup{\mathcal{A}^*}$.
	%
	By the existence of $\mathcal{A}$, and by Observation~\ref{obs:why-ans}, the oracle call does not fail, and returns a set $\mathcal{\hat{S}} \in \starwhyk{k}{()}{\hat{D}}{\hat{Q}}$. Moreover, by Observation~\ref{obs:why-ans}, Observation~\ref{obs:diversity-ans}, and the fact that $\mathcal{\hat{S}}$ maximizes the diversity, i.e., $\mathcal{\hat{S}} \in \argmax\limits_{\mathcal{S} \in \starwhyk{k}{()}{\hat{D}}{\hat{Q}}} \diversity{\mathcal{S}}$, we conclude that
	$$\diversity{\mathcal{\hat{S}}}\ =\ k(k-1) + 2\cdot d^*.$$
	%
	Since $d^* \ge d$, we have that $\diversity{\mathcal{\hat{S}}} \ge k(k-1) + 2\cdot d$, and thus $\mathsf{DecideDiverseAnswers}$ accepts, as needed.

    \medskip
    
	($\Leftarrow$) Assume now that there is no set $\mathcal{A} \in \ansk{k}{D}{Q^*}$ with $\diversitytup{\mathcal{A}} \ge d$, i.e., either $\ansk{k}{D}{Q^*}$ is empty, or $\ansk{k}{D}{Q^*}$ is not empty but every set $\mathcal{A}^* \in \argmax\limits_{\mathcal{A} \in \ansk{k}{D}{Q^*}} \diversitytup{\mathcal{A}}$ is such that $\diversitytup{\mathcal{A}^*} < d$. We argue that $\mathsf{DecideDiverseAnswers}$ rejects with input $D$, $k$, and $d$. If $\ansk{k}{D}{Q^*}$ is empty then, by Observation~\ref{obs:why-ans}, $\starwhyk{k}{()}{\hat{D}}{\hat{Q}}$ is also empty, and thus the oracle call will fail, and $\mathsf{DecideDiverseAnswers}$ rejects, as needed. Assume instead that $\ansk{k}{D}{Q^*}$ is not empty, but every $\mathcal{A}^* \in \argmax\limits_{\mathcal{A} \in \ansk{k}{D}{Q^*}} \diversitytup{\mathcal{A}}$ is such that $\diversitytup{\mathcal{A}^*} < d$. Let $d^* = \diversitytup{\mathcal{A}^*}$, for an arbitrarily chosen $\mathcal{A}^* \in \argmax\limits_{\mathcal{A} \in \ansk{k}{D}{Q^*}} \diversitytup{\mathcal{A}}$.
	By Observation~\ref{obs:why-ans}, and the fact that $\ansk{k}{D}{Q^*}$ is not empty, the oracle call will succeed and the set $\mathcal{\hat{S}} \in \argmax\limits_{\mathcal{S} \in \starwhyk{k}{()}{\hat{D}}{\hat{Q}}} \diversity{\mathcal{S}}$ is constructed.
	By Observation~\ref{obs:why-ans}, Observation~\ref{obs:diversity-ans}, and the fact that $\mathcal{\hat{S}}$ has maximum diversity, we get that
	$$\diversity{\mathcal{\hat{S}}}\ =\ k(k-1) + 2\cdot d^*.$$
	Since $d^* < d$, we have that $\diversity{\mathcal{\hat{S}}} < k(k-1) + 2\cdot d$, and thus $\mathsf{DecideDiverseAnswers}$ rejects, as needed.

\medskip

Theorem~\ref{the:diversity-complexity} suggests that for providing practical solutions to our problems we need to exploit existing optimization methods that are able to solve hard problems. We proceed in the next section to discuss how this can be achieved via Integer Linear Programming.


\begin{comment}
Consider two databases $D_1,D_2$ over the same schema $\ins{S}$. We use $\diff{D_1}{D_2}$ to denote the \emph{symmetric difference between $D_1$ and $D_2$}, i.e., the set $(D_1 \setminus D_2) \cup (D_2 \setminus D_1)$. Moreover, the \emph{distance between $D_1$ and $D_2$}, written $\dist{D_1}{D_2}$, is the number $|\diff{D_1}{D_2}|$.

Finally, for a finite set $\mathcal{S} = \{D_1,\ldots,D_k\}$ of databases, all over the same schema $\ins{S}$, we define the \emph{diversity of $\mathcal{S}$}, denoted as $\diversity{\mathcal{S}}$, as the following quantity:
$$ \sum\limits_{i<j \in [k]} \dist{D_i}{D_j}.$$

In what follows, for a Datalog query $Q = (\dep,R)$, a database $D$ over $\esch{\dep}$, a tuple $\bar t \in \adom{D}^{\arity{R}}$, and an integer $k \ge 0$, we use $\whyk{k}{\bar t}{D}{Q}$ to denote the collection of all sets $\mathcal{S} \subseteq \why{\bar t}{D}{Q}$ with $|\mathcal{S}| = k$, i.e., each element of $\whyk{k}{\bar t}{D}{Q}$ contains exactly $k$ members of the why-provenance of $\bar t$ w.r.t. $D$ and $Q$.
 
With the above notions in place, we can now define our problem of interest.
\begin{center}
	\fbox{\begin{tabular}{ll}
			{\small PROBLEM} : & $\mathsf{Diversity}$
			\\[2mm]
			{\small INPUT} : & A Datalog query $Q = (\dep,R)$, \\
			& a database $D$ over $\esch{\dep}$,\\
			& a tuple ${\bar t} \in \adom{D}^{\arity{R}}$, and\\
			& an integer $k > 0$\\[2mm]
			{\small OUTPUT} : & A member of $\argmax\limits_{\mathcal{S} \in \whyk{k}{\bar t}{D}{Q}} \diversity{\mathcal{S}}$ if it exists,\\
			&  otherwise \textbf{fail} 
	\end{tabular}}
\end{center}

Note that in the definition above, there can be many sets $\mathcal{S} \in \whyk{k}{\bar t}{D}{Q}$ which maximize the diversity $\diversity{\mathcal{S}}$, and thus the problem requires computing an arbitrary such a set.

%We can similarly define the set $\unwhyk{k}{\bar t}{D}{Q}$, where we consider the unambiguous why-provenance $\unwhy{\bar t}{D}{Q}$, instead of the standard why-provenance $\why{\bar t}{D}{Q}$. This leads to the definition of the problem $\mathsf{Diversity}_\mathsf{UN}$, which is defined exactly as $\mathsf{Diversity}$ with the only difference that we consider $\unwhyk{k}{\bar t}{D}{Q}$ instead.
%
%\begin{theorem}
%	$\mathsf{Diversity}$ and $\mathsf{Diversity}_\mathsf{UN}$ are $\NP\hard$ in data complexity.
%\end{theorem}
\end{comment}

==> figures/conclusion.tex <==
\section{Conclusion}
Missing...

==> figures/downward-results.tex <==

% \begin{figure*}[t]
% \centering
% \small

% \begin{subfigure}[t]{0.32\textwidth}
% \centering
% \safeincludegraphics[width=\linewidth]{figures/no-vars/vars-runtime-k2-doctors_q01-100k-exact.pdf}
% \caption{\doctors(1), $k=2$}
% \end{subfigure}\hfill
% \begin{subfigure}[t]{0.32\textwidth}
% \centering
% \safeincludegraphics[width=\linewidth]{figures/no-vars/vars-runtime-k3-doctors_q01-100k-exact.pdf}
% \caption{\doctors(1), $k=3$}
% \end{subfigure}\hfill
% \begin{subfigure}[t]{0.32\textwidth}
% \centering
% \safeincludegraphics[width=\linewidth]{figures/no-vars/vars-runtime-k4-doctors_q01-100k-exact.pdf}
% \caption{\doctors(1), $k=4$}
% \end{subfigure}

% \vspace{2mm}

% \begin{subfigure}[t]{0.32\textwidth}
% \centering
% \safeincludegraphics[width=\linewidth]{figures/no-vars/vars-runtime-k5-doctors_q01-100k-exact.pdf}
% \caption{\doctors(1), $k=5$}
% \end{subfigure}\hfill
% \begin{subfigure}[t]{0.32\textwidth}
% \centering
% \safeincludegraphics[width=\linewidth]{figures/no-vars/vars-runtime-k4-doctors_q05-100k-exact.pdf}
% \caption{\doctors(5), $k=4$}
% \end{subfigure}\hfill
% \begin{subfigure}[t]{0.32\textwidth}
% \centering
% \safeincludegraphics[width=\linewidth]{figures/no-vars/vars-runtime-k5-doctors_q05-100k-exact.pdf}
% \caption{\doctors(5), $k=5$}
% \end{subfigure}

% \vspace{2mm}

% \begin{subfigure}[t]{0.32\textwidth}
% \centering
% \safeincludegraphics[width=\linewidth]{figures/no-vars/vars-runtime-k2-doctors_q07-100k-exact.pdf}
% \caption{\doctors(7), $k=2$}
% \end{subfigure}\hfill
% \begin{subfigure}[t]{0.32\textwidth}
% \centering
% \safeincludegraphics[width=\linewidth]{figures/no-vars/vars-runtime-k3-doctors_q07-100k-exact.pdf}
% \caption{\doctors(7), $k=3$}
% \end{subfigure}\hfill
% \begin{subfigure}[t]{0.32\textwidth}
% \centering
% \safeincludegraphics[width=\linewidth]{figures/no-vars/vars-runtime-k4-doctors_q07-100k-exact.pdf}
% \caption{\doctors(7), $k=4$}
% \end{subfigure}

% \caption{Runtime as a function of variable count for the exact method across the selected \doctors configurations.}
% \label{fig:vars-runtime-doctors-exact}
% \end{figure*}

% \begin{figure*}[t]
% \ContinuedFloat
% \centering
% \small

% \begin{subfigure}[t]{0.32\textwidth}
% \centering
% \safeincludegraphics[width=\linewidth]{figures/no-vars/vars-runtime-k5-doctors_q07-100k-exact.pdf}
% \caption{\doctors(7), $k=5$}
% \end{subfigure}

% \caption[]{Runtime as a function of variable count for the exact method across the selected \doctors configurations (continued).}
% \end{figure*}


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/no-vars/vars-boxplot-doctors-selected-k.pdf}
    \caption{Variable-count distributions for the exact method. Red points denote timeouts, which occur predominantly in scenarios with a larger number of variables.}
    \label{fig:timeouts}
\end{figure}













% \begin{figure*}[t]
% \centering
% \small

% \begin{subfigure}[t]{0.32\textwidth}
% \centering
% \safeincludegraphics[width=\linewidth]{figures/no-vars/vars-runtime-k3-csda-httpd-exact.pdf}
% \caption{\csda: \httpd}
% \end{subfigure}\hfill
% \begin{subfigure}[t]{0.32\textwidth}
% \centering
% \safeincludegraphics[width=\linewidth]{figures/no-vars/vars-runtime-k3-csda-linux-exact.pdf}
% \caption{\csda: \linux}
% \end{subfigure}\hfill
% \begin{subfigure}[t]{0.32\textwidth}
% \centering
% \safeincludegraphics[width=\linewidth]{figures/no-vars/vars-runtime-k3-csda-postgresql-exact.pdf}
% \caption{\csda: \postgres}
% \end{subfigure}

% \vspace{2mm}

% \begin{subfigure}[t]{0.32\textwidth}
% \centering
% \safeincludegraphics[width=\linewidth]{figures/no-vars/vars-runtime-k3-doctors_q01-100k-exact.pdf}
% \caption{\doctors(1): \factsk}
% \end{subfigure}\hfill
% \begin{subfigure}[t]{0.32\textwidth}
% \centering
% \safeincludegraphics[width=\linewidth]{figures/no-vars/vars-runtime-k3-doctors_q02-100k-exact.pdf}
% \caption{\doctors(2): \factsk}
% \end{subfigure}\hfill
% \begin{subfigure}[t]{0.32\textwidth}
% \centering
% \safeincludegraphics[width=\linewidth]{figures/no-vars/vars-runtime-k3-doctors_q03-100k-exact.pdf}
% \caption{\doctors(3): \factsk}
% \end{subfigure}

% \vspace{2mm}

% \begin{subfigure}[t]{0.32\textwidth}
% \centering
% \safeincludegraphics[width=\linewidth]{figures/no-vars/vars-runtime-k3-doctors_q04-100k-exact.pdf}
% \caption{\doctors(4): \factsk}
% \end{subfigure}\hfill
% \begin{subfigure}[t]{0.32\textwidth}
% \centering
% \safeincludegraphics[width=\linewidth]{figures/no-vars/vars-runtime-k3-doctors_q05-100k-exact.pdf}
% \caption{\doctors(5): \factsk}
% \end{subfigure}\hfill
% \begin{subfigure}[t]{0.32\textwidth}
% \centering
% \safeincludegraphics[width=\linewidth]{figures/no-vars/vars-runtime-k3-doctors_q06-100k-exact.pdf}
% \caption{\doctors(6): \factsk}
% \end{subfigure}

% \caption{Runtime as a function of variable count for the exact method with $k=3$ across scenarios and datasets.}
% \label{fig:vars-runtime-k3-exact}
% \end{figure*}


% \begin{figure*}[t]
% \ContinuedFloat
% \centering
% \small

% \begin{subfigure}[t]{0.32\textwidth}
% \centering
% \safeincludegraphics[width=\linewidth]{figures/no-vars/vars-runtime-k3-doctors_q07-100k-exact.pdf}
% \caption{\doctors(7): \factsk}
% \end{subfigure}\hfill\begin{subfigure}[t]{0.32\textwidth}
% \centering
% \safeincludegraphics[width=\linewidth]{figures/no-vars/vars-runtime-k3-graph_analytics-bitcoin-exact.pdf}
% \caption{\graphanalytics: \bitcoin}
% \end{subfigure}\hfill
% \begin{subfigure}[t]{0.32\textwidth}
% \centering
% \safeincludegraphics[width=\linewidth]{figures/no-vars/vars-runtime-k3-graph_analytics-facebook-exact.pdf}
% \caption{\graphanalytics: \facebook}
% \end{subfigure}

% \caption[]{Runtime as a function of variable count for the exact method with $k=3$ across scenarios and datasets (continued).}
% \end{figure*}







% \begin{figure*}[t]
% \centering
% \small

% \begin{subfigure}[t]{0.32\textwidth}
% \centering
% \safeincludegraphics[width=\linewidth]{figures/downward/closure-runtime-csda-httpd-exact.pdf}
% \caption{\csda: \httpd}
% \end{subfigure}\hfill
% \begin{subfigure}[t]{0.32\textwidth}
% \centering
% \safeincludegraphics[width=\linewidth]{figures/downward/closure-runtime-csda-linux-exact.pdf}
% \caption{\csda: \linux}
% \end{subfigure}\hfill
% \begin{subfigure}[t]{0.32\textwidth}
% \centering
% \safeincludegraphics[width=\linewidth]{figures/downward/closure-runtime-csda-postgresql-exact.pdf}
% \caption{\csda: \postgres}
% \end{subfigure}

% \vspace{2mm}

% \begin{subfigure}[t]{0.32\textwidth}
% \centering
% \safeincludegraphics[width=\linewidth]{figures/downward/closure-runtime-doctors_q01-100k-exact.pdf}
% \caption{\doctors(1): \factsk}
% \end{subfigure}\hfill
% \begin{subfigure}[t]{0.32\textwidth}
% \centering
% \safeincludegraphics[width=\linewidth]{figures/downward/closure-runtime-doctors_q02-100k-exact.pdf}
% \caption{\doctors(2): \factsk}
% \end{subfigure}\hfill
% \begin{subfigure}[t]{0.32\textwidth}
% \centering
% \safeincludegraphics[width=\linewidth]{figures/downward/closure-runtime-doctors_q03-100k-exact.pdf}
% \caption{\doctors(3): \factsk}
% \end{subfigure}

% \vspace{2mm}

% \begin{subfigure}[t]{0.32\textwidth}
% \centering
% \safeincludegraphics[width=\linewidth]{figures/downward/closure-runtime-doctors_q04-100k-exact.pdf}
% \caption{\doctors(4): \factsk}
% \end{subfigure}\hfill
% \begin{subfigure}[t]{0.32\textwidth}
% \centering
% \safeincludegraphics[width=\linewidth]{figures/downward/closure-runtime-doctors_q05-100k-exact.pdf}
% \caption{\doctors(5): \factsk}
% \end{subfigure}\hfill
% \begin{subfigure}[t]{0.32\textwidth}
% \centering
% \safeincludegraphics[width=\linewidth]{figures/downward/closure-runtime-doctors_q06-100k-exact.pdf}
% \caption{\doctors(6): \factsk}
% \end{subfigure}

% \caption{Runtime as a function of downward-closure size for the exact method across scenarios and datasets.}
% \label{fig:downward-runtime-exact}
% \end{figure*}


% \begin{figure*}[t]
% \ContinuedFloat
% \centering
% \small

% \begin{subfigure}[t]{0.32\textwidth}
% \centering
% \safeincludegraphics[width=\linewidth]{figures/downward/closure-runtime-doctors_q07-100k-exact.pdf}
% \caption{\doctors(7): \factsk}
% \end{subfigure}\hfill
% \begin{subfigure}[t]{0.32\textwidth}
% \centering
% \safeincludegraphics[width=\linewidth]{figures/downward/closure-runtime-galen-40-exact.pdf}
% \caption{\galen: \forty}
% \end{subfigure}\hfill
% \begin{subfigure}[t]{0.32\textwidth}
% \centering
% \safeincludegraphics[width=\linewidth]{figures/downward/closure-runtime-galen-50-exact.pdf}
% \caption{\galen: \fifty}
% \end{subfigure}

% \vspace{2mm}

% \begin{subfigure}[t]{0.32\textwidth}
% \centering
% \safeincludegraphics[width=\linewidth]{figures/downward/closure-runtime-graph_analytics-bitcoin-exact.pdf}
% \caption{\graphanalytics: \bitcoin}
% \end{subfigure}\hspace{1cm}
% \begin{subfigure}[t]{0.32\textwidth}
% \centering
% \safeincludegraphics[width=\linewidth]{figures/downward/closure-runtime-graph_analytics-facebook-exact.pdf}
% \caption{\graphanalytics: \facebook}
% \end{subfigure}

% \caption[]{Runtime as a function of downward-closure size for the exact method across scenarios and datasets (continued).}
% \end{figure*}

==> figures/exact-encoding.tex <==
\section{Diverse Why-provenance via Integer Linear Programming}\label{sec:exact-encoding}


We aim to encode $\star\text{-}\mathsf{DiverseWhyProvenance}$, for $\star \in \{\mathsf{ALL},\mathsf{UN}\}$, as an Integer Linear Programming (ILP) maximization problem $\Pi$ in such a way that each set $\mathcal{S} \in \starwhyk{k}{\bar t}{D}{Q}$, for some Datalog query $Q = (\dep,R)$, database $D$ over $\esch{\dep}$, tuple $\bar t \in \adom{D}^{\arity{R}}$, and integer $k > 0$, that maximizes $\diversity{\mathcal{S}}$ can be extracted from one of the optimal solutions of $\Pi$.
%
Of course, as we shall see in the next section, there are multiple ways to construct such an encoding, relying on different characterizations of when a database $D'$ is a member of $\starwhy{\bar t}{D}{Q}$.
%
Hence, in this section, we first define a general framework for devising such ILP maximization problems in a uniform way, which will then be instantiated with concrete encodings. We start by recalling the basics of ILP, and then introduce the key properties that an ILP encoding should enjoy to allow us to cast $\star\text{-}\mathsf{DiverseWhyProvenance}$ as an ILP maximization problem.



\begin{comment}
In this section, we discuss how to solve the problem $\mathsf{Diversity}$ by exploiting Integer Linear Programming (ILP). In particular,  our goal is to encode $\mathsf{Diversity}$ as an integer linear programming maximization problem, where each set $\mathcal{S} \in \whyk{k}{\bar t}{D}{Q}$ that maximizes $\diversity{\mathcal{S}}$ can be retrieved from one of the optimal solutions of the optimization problem.

As we are going to see, there can be multiple ways to construct this encoding, depending on different characterizations of when a database $D'$ is a member of the why-provenance $\why{\bar t}{D}{Q}$, for some Datalog query $Q = (\dep,R)$, a database $D$ over $\esch{\dep}$, and tuple $\bar t \in \adom{D}^{\arity{R}}$.

Hence, we first define a general framework for devising such maximization problems, and then we will show how to instantiate this framework with concrete characterizations. We start by defining ILP, and then move to define the key properties that an ILP encoding should have in order to allow us to solve the problem $\mathsf{Diversity}$.
\end{comment}

\subsection{Integer Linear Programming}\label{sec:ILP}

%\medskip
%\noindent
%\textbf{Integer Linear Programming (ILP).} 
Consider the disjoint sets $X$ and $B$ of integer variables and binary variables, respectively. An \emph{assignment for $X$ and $B$} is a function $\mu : X \cup B \rightarrow \mathbb{Z}$ such that, for each $x \in B$, $\mu(x) \in \{0,1\}$. 

%For a set $Y \subseteq X \cup B$, we write $\proj{\mu}{Y}$ for the restriction of $\mu$ over $Y$.
%Given a set $S$ of assignments for $X$ and $B$, we write $\proj{S}{Y}$ for the set of assignments $\{\proj{\mu}{Y} \mid \mu \in S\}$.
%for the function $\tau : Y \rightarrow \mathbb{Z}$ with $\tau(y) = \mu(y)$, for all $y \in Y$. 
%We extend the notation $\proj{S}{Y}$ to \emph{sets} $S$ of assignments in the natural way. 
An \emph{ILP constraint over $X$ and $B$} is an expression 
\[
a_1 x_1 + \cdots + a_n  x_n\ \diamond\ a_0,
\]
where, for each $i \in [n]$, $a_i \in \mathbb{Q}$, $x_i \in X \cup B$, $\diamond \in \{ \ge, \le, =\}$, and $a_0 \in \mathbb{Q}$. We say that an assignment $\mu$ for $X$ and $B$ \emph{satisfies} the constraint $a_1 x_1 + \cdots + a_n  x_n \diamond a_0$ over $X$ and $B$ if it holds that
\[
a_1 \mu(x_1) + \cdots + a_n \mu(x_n) \diamond a_0.
\]
A \emph{system of ILP constraints over $X$ and $B$} is a set $T$ of ILP constraints over $X$ and $B$. A \emph{solution of $T$} is an assignment for $X$ and $B$ that satisfies all the constraints in $T$; we write $\sol{T}$ for the set that collects all the solutions of $T$. If $T$ admits a solution, i.e., $\sol{T} \neq \emptyset$, then we say that $T$ is \emph{feasible}; otherwise, $T$ is \emph{unfeasible}.

An \emph{ILP maximization problem over $X$ and $B$} is a pair $(f,T)$, where $f$ is an expression of the form
$c_1 z_1 + \cdots + c_m z_m$,
with $c_1,\ldots,c_n \in \mathbb{Q}$ and $z_1,\ldots,z_n \in X \cup B$, and $T$ is a system of ILP constraints over $X$ and $B$. 
An \emph{optimal solution} of $(f,T)$ is a solution $\mu$ of $T$ that maximizes $f$ among all solutions of $T$, i.e., for every $\mu' \in \sol{T}$, it holds that $c_1 \mu(z_1) + \cdots + c_m \mu(z_m) \geq c_1 \mu'(z_1) + \cdots + c_m \mu'(z_m)$. We write $\opt{f,T}$ for the set of all optimal solutions of $(f,T)$.

\medskip
\noindent
\textbf{XOR and Indicator Constraints.} For the sake of technical clarity, apart from linear constraints as defined above, we are going to also use xor constraints and indicator constraints, which we introduce below. It is well-known that xor and indicator constraints can be easily defined by means of linear constraints. Hence, in our technical development, we will directly use xor and indicator constraints to simplify the presentation, and we will refer to linear, xor, and indicator constraints simply as constraints.

An \emph{xor constraint over $B$} is an expression of the form
\[
x \oplus y\ =\ z,
\]
where $x,y,z$ are binary variables from $B$ and $\oplus$ denotes the xor operator. An assignment $\mu$ for $B$ satisfies the above xor constraint if $\mu(x) \oplus \mu(y) = \mu(z)$. 
%
Now, an \emph{indicator constraint over $X$ and $B$} is an expression of the form
\[
z\ \equiv\ a_1 x_1 + \cdots a_n x_n \diamond a_0,
\]
where $z \in B$ and $a_1 x_1 + \cdots a_n x_n \diamond a_0$ is a linear constraint over $X$ and $B$. An assignment $\mu$ for $X$ and $B$ satisfies the above indicator constraint when $\mu(z) = 1$ iff $\mu$ satisfies the linear constraint.

\begin{comment}
For integer variables $X$ and binary variables $B$, these include two kind of constraints. One is a \emph{xor constraint} of the form:
$$ x \oplus y = z,$$
where $x,y,z$ are binary variables from $B$, and $\oplus$ denotes the xor operator. An assignment $\mu$ satisfies the xor constraint when $\mu(z)$ coincides with the xor of $\mu(x)$ and $\mu(y)$. The other kind of constraint is an \emph{indicator constraint}, which is of the form:
$$z \equiv a_1 x_1 + \cdots a_n x_n \diamond a_0,$$
where $z$ is a binary variable from $B$, while $a_1 x_1 + \cdots a_n x_n \diamond a_0$ is a linear constraint over $X$ and $B$. The above indicator constraint is satisfied by an assignment $\mu$ when $\mu(z) = 1$ iff $\mu$ satisfies the linear constraint.

It is well-known that xor and indicator constraints can be easily defined by means of linear constraints. Hence, in what follows, we will use these additional kind of constraints directly, in order to simplify the presentation, and we will refer to linear constraints, xor constraints and indicator constraints simply as constraints.
\end{comment}

\subsection{Diverse Why-Provenance as an ILP Maximization Problem}
%\medskip
%\noindent
%\textbf{Diversity as an ILP maximization problem.} 


Having the basics of ILP in place, we can now introduce the general framework for casting $\star\text{-}\mathsf{DiverseWhyProvenance}$, where $\star \in \{\mathsf{ALL},\mathsf{UN}\}$, as an ILP maximization problem based on different ILP encodings in a uniform way. To this end, we first introduce the general notion of ILP encoding of why-provenance.

\begin{definition}[\textbf{ILP Encoding}]\label{def:ilp-encoding-why}
Consider a Datalog query $Q = (\dep,R)$, a database $D = \{\alpha_1,\ldots,\alpha_n\}$ over $\esch{\dep}$, for an integer $n>0$, and a tuple $\bar t \in \adom{D}^{\arity{R}}$. An \emph{ILP encoding of $\starwhy{\bar t}{D}{Q}$}, where $\star \in \{\mathsf{ALL},\mathsf{UN}\}$, is a system $T$ of ILP constraints over a set of integer variables $X$ and a set of binary variables $B$, such that $B$ contains $n$ distinguished variables $x_{\alpha_1},\ldots,x_{\alpha_n}$, called the \emph{database variables of $T$}, and such that, for all databases $D'$ over $\esch{\dep}$, the following are equivalent:
\begin{enumerate}
	\item $D' \in \starwhy{\bar t}{D}{Q}$.
	\item $D' = \{\alpha_i \mid i \in [n] \text{ and } \mu(x_{\alpha_i}) = 1\}$ for some $\mu \in \sol{T}$.
    %, for each $i \in [n]$, $\mu(x_{\alpha_i}) = 1$ if $\alpha_i \in D'$ and $\mu(x_{\alpha_i}) = 0$ if $\alpha_i \not\in D'$. 
    \hfill\markfull
\end{enumerate}
\end{definition}

Therefore, given a Datalog query $Q = (\dep,R)$, a database $D$ over $\esch{\dep}$, and a tuple $\bar t \in \adom{D}^{\arity{R}}$, if we are able to construct an ILP encoding $T$ of $\starwhy{\bar t}{D}{Q}$, then we can compute all the members of $\starwhy{\bar t}{D}{Q}$ by computing the solutions of $T$. 
%
We now proceed explain how to use an ILP encoding for why-provenance as defined above (Definition~\ref{def:ilp-encoding-why}) to solve $\star\text{-}\mathsf{DiverseWhyProvenance}$.


Consider an ILP encoding $T$ of $\starwhy{\bar t}{D}{Q}$ over $X$ and $B$, with $x_{\alpha_1},\ldots,x_{\alpha_n}$ being the database variables of $T$. For an assignment $\mu$ for $X$ and $B$, we denote by $\db{\mu}$ the \emph{database induced by $\mu$}, that is, the database $\{\alpha_i \mid i \in [n] \text{ and } \mu(x_{\alpha_i}) = 1\}$.
%for an assignment $\mu$ whose domain mentions the database variables $x_{\alpha_1},\ldots,x_{\alpha_n}$ of an ILP encoding of $\why{\bar t}{D}{Q}$, we use $\db{\mu}$ to denote the \emph{database induced by $\mu$}, i.e., the database $\{\alpha_i \mid \mu(x_{\alpha_i}) = 1 \text{ and } i \in [n]\}$.
%
%We can now exploit an ILP encoding of $\why{\bar t}{D}{Q}$ to solve $\mathsf{Diversity}$ as follows.
%Consider an ILP encoding $T$ of $\starwhy{\bar t}{D}{Q}$ with database variables $x_{\alpha_1},\ldots,x_{\alpha_n}$. 
For an integer $i > 0$, the \emph{$i$-th copy of $T$}, denoted $\copyof{T}{i}$, is the system of ILP constraints over $\copyof{X}{i} = \{\copyof{x}{i} \mid x \in X\}$ and $\copyof{B}{i} = \{\copyof{x}{i} \mid x \in B\}$ obtained from $T$ by replacing each integer and binary variable $x$ with $\copyof{x}{i}$.
%, where each integer and binary variable $x$ (including the database variables) is replaced with the fresh variable $\copyof{x}{i}$. 
We are now ready to define the ILP maximization problem that allows us to solve $\star\text{-}\mathsf{DiverseWhyProvenance}$.

\begin{definition}[\textbf{Maximization Problem}]\label{def:ilp-maximization-problem}
Consider a Datalog query $Q = (\dep,R)$, a database $D$ over $\esch{\dep}$, a tuple $\bar t \in \adom{D}^{\arity{R}}$, and an integer $k > 0$. Let $T$ be an ILP encoding of $\starwhy{\bar t}{D}{Q}$, for $\star \in \{\mathsf{ALL},\mathsf{UN}\}$, over $X$ and $B$, with $x_{\alpha_1},\ldots,x_{\alpha_n}$ being the database variables of $T$. %
The \emph{$(T,k)$-problem}
%The \emph{$T$-based encoding of $\mathsf{Diversity}$ w.r.t.\ $D$, $Q$, $\bar t$, and $k$}
is the ILP maximization problem $(f,S)$ over $\bigcup_{i \in [k]}\copyof{X}{i}$ and $\bigcup_{i \in [k]}\copyof{B}{i} \cup 
\{\auxvar^{i,j}_\ell \mid 1 \leq \ell \leq n \text{ and } 1 \leq i < j \leq k\}$, where $f$ is defined as the expression
\[
\sum\limits_{1 \leq i < j \leq k} \left(\sum\limits_{1 \leq \ell \leq n} \auxvar^{i,j}_\ell\right),
\]
and
%where $\copyof{X}{i}$ and $\copyof{B}{i}$ are the integer and binary variables of $\copyof{T}{i}$, for each $i \in [k]$, 
$S$ is the system of constraints
\begin{multline*}
\copyof{T}{1} \cup \cdots \cup \copyof{T}{k}\ \cup \\
 \left\{\copyof{x_{\alpha_\ell}}{i} \oplus \copyof{x_{\alpha_\ell}}{j} = \auxvar^{i,j}_\ell \mid 1 \leq \ell \leq n \text{ and } 1 \leq i < j \leq k\right\}\ \cup \\
 \left\{\sum\limits_{1 \leq \ell \leq n} \auxvar^{i,j}_\ell \ge 1 \mid 1 \leq i < j \leq k\right\}.\tag*{\markfull}
\end{multline*}
%and $f$ is the following function:
%\begin{flalign*}
%&& \sum\limits_{i < j \in [k]} \left(\sum\limits^n_{\ell=1} \auxvar^{i,j}_\ell\right).&& \markfull
%\end{flalign*}
%For each $i \in [k]$, we call the variables in the set $\{\copyof{x_{\alpha_\ell}}{i} \mid \ell \in [n]\}$ the \emph{$i$-th database variables of $(f,S)$}.\hfill\markfull
\end{definition}

Intuitively, the $(T,k)$-problem defined above 
%the $T$-based encoding $(f,S)$ of $\mathsf{Diversity}$ w.r.t.\ $D$, $Q$, $\bar t$, and $k$ 
is a maximization problem which enforces the simultaneous satisfaction of $k$ distinct copies $\copyof{T}{1},\ldots,\copyof{T}{k}$ of $T$. This makes a solution $\mu$ of $S$ to be of the form $\mu_1 \cup \cdots \cup \mu_k \cup \mu'$, where $\mu'$ is over the 
%\auxvar$ 
auxiliary variables, while each $\mu_i$ is a solution of $\copyof{T}{i}$. In addition, $S$ forces $\mu_1,\ldots,\mu_k$ to induce pairwise different databases. The latter is guaranteed by the combination of the xor constraints and the additional linear constraints, apart from those of $\copyof{T}{1},\ldots,\copyof{T}{k}$, added to $S$.
Hence, whenever $S$ is feasible, each solution of $S$ induces $k$ different members $D_1,\ldots,D_k$ of $\starwhy{\bar t}{D}{Q}$. The expression $f$ is then used to maximize the diversity of the set $\{D_1,\ldots,D_k\}$ where, for each $i,j \in [k]$ with $i < j$, the inner sum of $f$ encodes the distance between $D_i$ and $D_j$.
%
The above discussion is formalized by the following result.
%Formally, we can show the following technical result.

\begin{theorem}\label{thm:generic-encoding}
	Consider a Datalog query $Q = (\dep,R)$, a database $D$ over $\esch{\dep}$, a tuple $\bar t \in \adom{D}^{\arity{R}}$, and an integer $k > 0$. Let $T$ be an ILP encoding of $\starwhy{\bar t}{D}{Q}$, for $\star \in \{\mathsf{ALL},\mathsf{UN}\}$, over $X$ and $B$, with $x_{\alpha_1},\ldots,x_{\alpha_n}$ being the database variables of $T$. 
    %With $(f,S)$ being the $(T,k)$-problem,
%$T$-based ILP encoding $(f,S)$ of $\mathsf{Diversity}$ w.r.t.\ $D$, $Q$, $\bar t$, and $k$ is such that, 
For every set $\{D_1,\ldots,D_k\}$ of databases over $\esch{\dep}$, the following are equivalent:
	\begin{enumerate}
		\item $\{D_1,\ldots,D_k\} \in \argmax\limits_{\mathcal{S} \in \starwhyk{k}{\bar t}{D}{Q}} \diversity{\mathcal{S}}$. 
		\item There is an optimal solution $\mu$ of the $(T,k)$-problem such that, for each $i \in [k]$, $D_i = \{\alpha_\ell \mid \ell \in [n] \text{ and } \mu(\copyof{x_{\alpha_\ell}}{i}) = 1\}$.
        %, for each $\ell \in [n]$ and $i \in [k]$, $\mu(\copyof{x_{\alpha_\ell}}{i}) = 1$ iff $\alpha_\ell \in D_i$.
        %, and $\mu(\copyof{x_{\alpha_\ell}}{i}) = 0$ if $\alpha_\ell \not \in D_i$.
	\end{enumerate}
\end{theorem}
\begin{proof}
	\textcolor{red}{Missing...}
\end{proof}


%the problem $\mathsf{Diversity}$ by finding an optimal solution of the $T$-based encoding of $\mathsf{Diversity}$, w.r.t.\ the input database $D$, query $Q$, tuple $\bar t$, and integer $k$, where $T$ is any ILP encoding for $\why{\bar t}{D}{Q}$.


==> figures/exact-results.tex <==
\begin{figure*}[t]
\centering
\small

\begin{subfigure}[t]{0.36\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/csda-httpd-exact-arbitrary-hypergraph.pdf}
    \caption{\arbitrary, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/csda-httpd-exact-unambigous-hypergraph.pdf}
    \caption{\unambiguous, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/csda-httpd-exact-unambigous-dag.pdf}
    \caption{\unambiguous, \dagEnc}
\end{subfigure}

\caption{Runtime distribution for the \exact\ strategy on the \httpd\ dataset under the \csda\ scenario.}
\label{fig:csda-httpd-exact}
\end{figure*}

\begin{figure*}[t]
\centering
\small

\begin{subfigure}[t]{0.36\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/csda-postgresql-exact-arbitrary-hypergraph.pdf}
    \caption{\arbitrary, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/csda-postgresql-exact-unambigous-hypergraph.pdf}
    \caption{\unambiguous, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/csda-postgresql-exact-unambigous-dag.pdf}
    \caption{\unambiguous, \dagEnc}
\end{subfigure}

\caption{Runtime distribution for the \exact\ strategy on the \postgres\ dataset under the \csda\ scenario.}
\label{fig:csda-postgresql-exact}
\end{figure*}

\begin{figure*}[t]
\centering
\small

\begin{subfigure}[t]{0.36\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/csda-linux-exact-arbitrary-hypergraph.pdf}
    \caption{\arbitrary, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/csda-linux-exact-unambigous-hypergraph.pdf}
    \caption{\unambiguous, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/csda-linux-exact-unambigous-dag.pdf}
    \caption{\unambiguous, \dagEnc}
\end{subfigure}

\caption{Runtime distribution for the \exact\ strategy on the \linux\ dataset under the \csda\ scenario.}
\label{fig:csda-linux-exact}
\end{figure*}

% =========================
% Graph analytics
% =========================

\begin{figure*}[t]
\centering
\small

\begin{subfigure}[t]{0.36\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/graph_analytics-facebook-exact-arbitrary-hypergraph.pdf}
    \caption{\arbitrary, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/graph_analytics-facebook-exact-unambigous-hypergraph.pdf}
    \caption{\unambiguous, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/graph_analytics-facebook-exact-unambigous-dag.pdf}
    \caption{\unambiguous, \dagEnc}
\end{subfigure}

\caption{Runtime distribution for the \exact\ strategy on the \facebook\ dataset under the \graphanalytics scenario.}
\label{fig:graph-analytics-facebook-exact}
\end{figure*}

\begin{figure*}[t]
\centering
\small

\begin{subfigure}[t]{0.36\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/graph_analytics-bitcoin-exact-arbitrary-hypergraph.pdf}
    \caption{\arbitrary, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/graph_analytics-bitcoin-exact-unambigous-hypergraph.pdf}
    \caption{\unambiguous, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/graph_analytics-bitcoin-exact-unambigous-dag.pdf}
    \caption{\unambiguous, \dagEnc}
\end{subfigure}

\caption{Runtime distribution for the \exact\ strategy on the \bitcoin\ dataset under the \graphanalytics scenario.}
\label{fig:graph-analytics-bitcoin-exact}
\end{figure*}

% =========================
% Doctors
% =========================

\begin{figure*}[t]
\centering
\small

\begin{subfigure}[t]{0.36\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/doctors_q01-100k-exact-arbitrary-hypergraph.pdf}
    \caption{\arbitrary, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/doctors_q01-100k-exact-unambigous-hypergraph.pdf}
    \caption{\unambiguous, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/doctors_q01-100k-exact-unambigous-dag.pdf}
    \caption{\unambiguous, \dagEnc}
\end{subfigure}

\caption{Runtime distribution for the \exact\ strategy on the \factsk\ dataset under the \doctors\ (\texttt{q01}) scenario.}
\label{fig:doctors-q01-100k-exact}
\end{figure*}

\begin{figure*}[t]
\centering
\small

\begin{subfigure}[t]{0.36\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/doctors_q02-100k-exact-arbitrary-hypergraph.pdf}
    \caption{\arbitrary, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/doctors_q02-100k-exact-unambigous-hypergraph.pdf}
    \caption{\unambiguous, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/doctors_q02-100k-exact-unambigous-dag.pdf}
    \caption{\unambiguous, \dagEnc}
\end{subfigure}

\caption{Runtime distribution for the \exact\ strategy on the \factsk\ dataset under the \doctors\ (\texttt{q02}) scenario.}
\label{fig:doctors-q02-100k-exact}
\end{figure*}

\begin{figure*}[t]
\centering
\small

\begin{subfigure}[t]{0.36\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/doctors_q03-100k-exact-arbitrary-hypergraph.pdf}
    \caption{\arbitrary, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/doctors_q03-100k-exact-unambigous-hypergraph.pdf}
    \caption{\unambiguous, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/doctors_q03-100k-exact-unambigous-dag.pdf}
    \caption{\unambiguous, \dagEnc}
\end{subfigure}

\caption{Runtime distribution for the \exact\ strategy on the \factsk\ dataset under the \doctors\ (\texttt{q03}) scenario.}
\label{fig:doctors-q03-100k-exact}
\end{figure*}

\begin{figure*}[t]
\centering
\small

\begin{subfigure}[t]{0.36\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/doctors_q04-100k-exact-arbitrary-hypergraph.pdf}
    \caption{\arbitrary, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/doctors_q04-100k-exact-unambigous-hypergraph.pdf}
    \caption{\unambiguous, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/doctors_q04-100k-exact-unambigous-dag.pdf}
    \caption{\unambiguous, \dagEnc}
\end{subfigure}

\caption{Runtime distribution for the \exact\ strategy on the \factsk\ dataset under the \doctors\ (\texttt{q04}) scenario.}
\label{fig:doctors-q04-100k-exact}
\end{figure*}

\begin{figure*}[t]
\centering
\small

\begin{subfigure}[t]{0.36\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/doctors_q05-100k-exact-arbitrary-hypergraph.pdf}
    \caption{\arbitrary, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/doctors_q05-100k-exact-unambigous-hypergraph.pdf}
    \caption{\unambiguous, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/doctors_q05-100k-exact-unambigous-dag.pdf}
    \caption{\unambiguous, \dagEnc}
\end{subfigure}

\caption{Runtime distribution for the \exact\ strategy on the \factsk\ dataset under the \doctors\ (\texttt{q05}) scenario.}
\label{fig:doctors-q05-100k-exact}
\end{figure*}

\begin{figure*}[t]
\centering
\small

\begin{subfigure}[t]{0.36\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/doctors_q06-100k-exact-arbitrary-hypergraph.pdf}
    \caption{\arbitrary, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/doctors_q06-100k-exact-unambigous-hypergraph.pdf}
    \caption{\unambiguous, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/doctors_q06-100k-exact-unambigous-dag.pdf}
    \caption{\unambiguous, \dagEnc}
\end{subfigure}

\caption{Runtime distribution for the \exact\ strategy on the \factsk\ dataset under the \doctors\ (\texttt{q06}) scenario.}
\label{fig:doctors-q06-100k-exact}
\end{figure*}

\begin{figure*}[t]
\centering
\small

\begin{subfigure}[t]{0.36\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/doctors_q07-100k-exact-arbitrary-hypergraph.pdf}
    \caption{\arbitrary, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/doctors_q07-100k-exact-unambigous-hypergraph.pdf}
    \caption{\unambiguous, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/doctors_q07-100k-exact-unambigous-dag.pdf}
    \caption{\unambiguous, \dagEnc}
\end{subfigure}

\caption{Runtime distribution for the \exact\ strategy on the \factsk\ dataset under the \doctors\ (\texttt{q07}) scenario.}
\label{fig:doctors-q07-100k-exact}
\end{figure*}

% =========================
% Galen
% =========================

\begin{figure*}[t]
\centering
\small

\begin{subfigure}[t]{0.26\textwidth}
    \centering
    \safeincludegraphics[height=3.65cm]{figures/galen-15-k1-all-settings-violin-box-timeouts-blue-multiline.pdf}
    \caption{\fifteen}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.24\textwidth}
    \centering
    \safeincludegraphics[height=3.65cm]{figures/galen-25-k1-all-settings-violin-box-timeouts-blue-multiline.pdf}
    \caption{\twentyfive}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.24\textwidth}
    \centering
    \safeincludegraphics[height=3.65cm]{figures/galen-40-k1-all-settings-violin-box-timeouts-blue-multiline.pdf}
    \caption{\forty}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.24\textwidth}
    \centering
    \safeincludegraphics[height=3.65cm]{figures/galen-50-k1-all-settings-violin-box-timeouts-blue-multiline.pdf}
    \caption{\fifty}
\end{subfigure}

\caption{Runtime distribution for the \exact\ strategy on the datasets under the \galen\ scenario.}
\label{fig:galen-exact}
\end{figure*}


==> figures/experiments-approximate.tex <==
\section{Approximate Computation of Diverse Why-Provenance}
\label{sec:approximate-experiments}

This section evaluates the approximate algorithm introduced in Section~\ref{sec:approximations}. Our goal is to assess both its efficiency and the quality of the explanation sets it produces.

The experimental setting follows that of Section~\ref{sec:exact-experiments}, using the same datasets, scenarios, encodings (hypergraph and DAG), and provenance semantics (arbitrary and unambiguous). This allows for a direct comparison with the exact algorithm. The main difference is that, in addition to runtime, we also evaluate the \emph{diversity} of the returned explanations and compare it against the optimal diversity whenever the exact solution is available. In particular, we report the approximation ratio with respect to the optimum.

We organize the results into three Sections. First, in Section~\ref{sec:approximate-runtime}, we present the runtime of the approximate algorithm and compare it against the exact approach. Second, in Section~\ref{sec:quality} we evaluate the quality of the approximation by measuring how close the produced solutions are to the optimal diversity, where we report the approximation ratio across scenarios, datasets, and values of k. Finally, in Section~\ref{sec:large-k}, we study the scalability of the approximate algorithm for larger values of $k$ (beyond those considered in Section~\ref{sec:exact-experiments}), demonstrating its ability to efficiently construct diverse explanations even when the exact algorithm becomes impractical.

\input{approximate-results}

\subsection{Runtime Analysis} 
\label{sec:approximate-runtime}

Figures~\ref{fig:csda-httpd-approximate}-\ref{fig:galen-50-approximate} report the runtime of the approximate computation across all datasets and configurations. In contrast to the exact computation (Section~\ref{sec:exact-experiments}), the approximate computation scales smoothly as $k$ increases and achieves substantial improvements in runtime.

% point to figures and mention and compare the numbers in the figures

The key observation is that runtime is reduced by several orders of magnitude across all settings. Even as $k$ increases, runtimes remain low, with the vast majority of runs completing well below $10^3$ milliseconds (i.e., under one second). This represents a dramatic improvement over the exact computation and demonstrates that the approximate computation is suitable for practical, interactive settings that require near-real-time responses.

As expected, and similar to the exact algorithm, the approximate algorithm's runtime increases with $k$, reflecting its incremental nature: it constructs explanations one by one and optimizes diversity at each step. However, this growth remains modest and controlled. By avoiding joint optimization over all $k$ explanations, the algorithm avoids the combinatorial explosion inherent in the exact ILP formulation, yielding stable performance and limited variability across instances.

A direct consequence of this improvement is that the vast majority of timeouts observed in the exact algorithm disappear. Only a small number of challenging instances still reach the timeout threshold (e.g., see Figures~\ref{fig:csda-httpd-approximate-b}, ~\ref{fig:graph-analytics-facebook-approximate}, \ref{fig:doctors-q01-100k-approximate-c}, \ref{fig:doctors-q07-100k-approximate-c}, \ref{fig:galen-50-approximate-a}, and \ref{fig:galen-50-approximate-b}), typically in more complex scenarios or for larger values of $k$. 

Regarding differences across encodings and semantics (e.g., hypergraph vs.\ DAG, or arbitrary vs.\ unambiguous), we observe trends similar to those discussed for the exact algorithm (Section~\ref{sec:exact-experiments}), although the differences are significantly less pronounced due to the reduced problem size at each step.

\input{ratios-results}

\subsection{Diversity Quality} \label{sec:quality}

We now assess the quality of the approximate solutions. Figures~\ref{fig:csda-httpd-rate}-\ref{fig:doctors-100k-rate} report the ratio between the optimal diversity and the diversity achieved by the approximate algorithm.

As expected, the ratio is exactly $1$ for $k=1$, since there is only one explanation and the solution is trivially optimal. 
For larger values of $k$, the ratio typically increases slightly above $1$, indicating a small gap between the approximate and optimal solutions.

A consistent pattern across datasets is that the ratio is highest for small values of $k>1$ (often at $k=2$), and then gradually decreases as $k$ increases. 
This behavior can be explained by the greedy nature of the algorithm: early choices are made without knowledge of future selections, which may lead to suboptimal combinations when only a few explanations are selected. 
As $k$ grows, the solution space becomes more constrained, and the greedy choices align more closely with the optimal global structure.

Importantly, the ratios remain very close to $1$ in all cases. 
Even in the most challenging scenarios, the observed gap is small, showing that the approximate algorithm consistently captures a large fraction of the optimal diversity. 
This significantly exceeds the theoretical worst-case guarantee established in Section~\ref{sec:approximations}.

The results highlight a clear trade-off between optimality and efficiency. 
While the exact algorithm provides optimal solutions, its runtime grows rapidly with $k$ and often becomes impractical. 
In contrast, the approximate algorithm scales efficiently, avoids timeouts, and achieves near-optimal diversity in practice.

Overall, the approximation closely follows the theoretical guarantees while delivering substantially better empirical performance, making it the preferred choice for large-scale or real-time applications.


\subsection{Scalability to Larger $k$}
\label{sec:large-k}

\input{approximate-results-10}

To further assess scalability, we evaluate the approximate algorithm for larger values of $k$ on a subset of challenging instances where timeouts were previously observed under the default time limit. In this experiment, we remove the timeout constraint and report the actual runtime required to complete the computation.

The results in Figures~\ref{fig:k10-csda-httpd-approximate}-\ref{fig:k10-graph-analytics-facebook-approximate} show that the approximate algorithm continues to scale gracefully even for larger $k$. While runtime increases as expected with $k$, the growth remains controlled and stable. This experiment demonstrates that the approximate algorithm maintains robust performance beyond the typical operating range of $k$, providing a reliable and scalable solution for generating diverse provenance explanations.

==> figures/experiments-exact.tex <==
\section{Exact Computation of Diverse Why-Provenance}
\label{sec:exact-experiments}
The goal of this section is to experimentally evaluate our ILP-based approach at solving the problem  $\star\text{-}\mathsf{DiverseWhyProvenance}$, for $\star \in \{\mathsf{ALL},\mathsf{UN}\}$. In particular, we implemented 4 different algorithms, one for each pair of a family of proof trees $\star \in \{\mathsf{ALL}, \mathsf{UN}\}$ and desired charaterization $\gamma \in \{\mathsf{hyper}, \mathsf{dag}\}$, where $\mathsf{hyper}$ stands for the hypergraph-based characterization, and $\mathsf{dag}$ stands for the graph-based one. For each such a pair $(\star,\gamma)$, we implemented the algorithm dubbed $\ComputeDiverse{\star}{\gamma}$, shown in Algorithm~\ref{alg:compute-diverse}. 

In particular, regardless of the choice of $\gamma \in \{\mathsf{hyper},\mathsf{dag}\}$, the algorithn $\ComputeDiverse{\star}{\gamma}$ solves $\star\text{-}\mathsf{DiverseWhyProvenance}$. It does so by exploting the ILP encoding $\ilpstargamma{\bar t}{D}{Q}$, and in particular, it exploits Theorem~\ref{thm:generic-encoding}, which, together with the fact that $\ilpstargamma{\bar t}{D}{Q}$ is an ILP encoding for $\starwhy{\bar t}{D}{Q}$ (cf. Theorems~\ref{thm:hyper-correct},\ref{thm:un-hyper-correct},\ref{thm:dag-correct}, and \ref{thm:unambiguous-dag-correct}) guarantees that $\ComputeDiverse{\star}{\gamma}$ always produces the correct output.

With the above in place, we can now move to discuss how we implemented the algorithm $\ComputeDiverse{\star}{\gamma}$, for each $\star \in \{\mathsf{ALL}, \mathsf{UN}\}$, and each $\gamma \in \{\mathsf{hyper}, \mathsf{dag}\}$, and then we will present an experimental evaluation of such implementations. The latter will allow us to asses the running time of our implementations on well-established benchbarks, and in particular, how the running time scales w.r.t.\ the requested number $k$ of members of $\starwhy{\bar t}{D}{Q}$.

%We evaluate the runtime of the \emph{exact} algorithm for computing a set of \(k\) diverse why-provenance explanations using the ILP encoding in Section~\ref{sec:characterizations}. Our goal is to understand how this algorithm scales with \(k\) across databases and configurations, and to identify the regimes where exact optimization remains practical.
%
%We consider three configurations for the algorithm combining proof-tree types and ILP characterizations: (\arbitrary, \hypergraph), (\unambiguous, \hypergraph), and (\unambiguous, \dagEnc). We exclude (\arbitrary, \dagEnc) due to its poor results. In preliminary experiments, we constructed the corresponding ILP instances and evaluated them under the same experimental setting used throughout the paper, including a timeout limit of 10 minutes per instance. However, none of the tested instances in this configuration completed within the timeout. The main reason is the rapid growth of the ILP formulation caused by the need for multiple copies of intensional nodes, which leads to extremely large optimization problems in both time and memory consumption.

%
\begin{algorithm}[t]
	\caption{The algorithm $\ComputeDiverse{\star}{\gamma}$}
	\label{alg:compute-diverse}
	
	\BlankLine
	
	\KwIn{A Datalog query $Q = (\dep,R)$, a database $D = \{\alpha_1,\ldots,\alpha_n\}$ over $\esch{\dep}$, a tuple $\bar t \in \adom{D}^{\arity{R}}$, and an integer $k >0 $.}
	\KwOut{A set of $k$ databases, or \textbf{fail}}
	
	\BlankLine
	
	Construct $\downc{R(\bar t)}{D}{\dep}$\;
	Construct the ILP encoding $T = \ilpstargamma{\bar t}{D}{Q}$ having database variables $x_{\alpha_1},\ldots,x_{\alpha_n}$, using $\downc{R(\bar t)}{D}{\dep}$\;
	Construct the $(T,k)$-problem $(f,S)$\;
	\If{an optimal solution $\mu$ of $(f,S)$ exists}{
		\For{$i = 1$ \textbf{\text{to}} $k$}{
			$D_i := \{\alpha_\ell \mid \ell \in [n] \text{ and } \mu(\copyof{x_{\alpha_\ell}}{i}) = 1\}$\;
		}
		\textbf{return} $\{D_1,\ldots,D_k\}$\;
	}\Else{\textbf{return} \textbf{fail}\;}
\end{algorithm}

\subsection{Implementation Details}
\label{sec:implementation-details}

In what follows, fix a family of proof trees $\star \in \{\mathsf{ALL}, \mathsf{UN}\}$, and a desired charaterization $\gamma \in \{\mathsf{hyper}, \mathsf{dag}\}$. From Algorithm~\ref{alg:compute-diverse}, we see that for a given input $Q = (\dep,R)$, $D$, $\bar t$, and $k$, the main tasks of $\ComputeDiverse{\star}{\gamma}$ are 1) computing the downward closure $\downc{R(\bar t)}{D}{\dep}$; 2) computing the ILP encoding $T = \ilpstargamma{\bar t}{D}{Q}$, together with the $(T,k)$-problem $(f,S)$; 3) solving $(f,S)$.
%
We briefly describe how we implemented the above 3 steps. 

\medskip
\noindent
\textbf{Constructing the Downward Closure.}
Regarding the downward closure, this is a data structure that is orthogonal to the specific ILP encoding employed, and it has already been used in previous works on the why-provenance for Datalog~\cite{ElKM22,CLPS24aaai}. In particular, employ an existing implementation from~\cite{CLPS24aaai} for computing the downward closure which in turn exploits the DLV Datalog engine~\cite{adrian2018dlv}.

\medskip
\noindent
\textbf{Constructing the ILP encoding.}
The construction of the ILP encoding $T = \ilpstargamma{\bar t}{D}{Q}$ and the corresponding $(T,k)$-problem is implemented in C++, and mostly follows Definition~\ref{def:ilp-encoding-why} and Definition~\ref{def:ilp-maximization-problem}. The only differences are related to the database variables of $T$ and how we encode indicator constraints. Regarding the database variables, only the ones corresponding to facts appearing in the downward closure are actually generated in $T$, since by definition of $T = \ilpstargamma{\bar t}{D}{Q}$, all other database variables are always set to $0$, in any solution of $T$. Regarding the indicator constraints, these only occur in $T$ when $\gamma = \mathsf{hyper}$, and they are all of the form
$$ z\ \equiv\ (\ a_1 x_1 + \cdots a_n x_n\ ) \ge 1,$$
where the expression $a_1 x_1 + \cdots a_n x_n$ can never be negative and it is alwasy an integer. Hence, the indicator constraint essentially asks that $z$ is $1$ iff $a_1 x_1 + \cdots a_n x_n$ is non-zero. For
efficiency reasons, we encode the constraint by means of the following set of constraints:
\begin{multline*}
\{z \cdot (\ a_1 x_1 + \cdots a_n x_n\ ) = a_1 x_1 + \cdots a_n x_n, \\
 z \le a_1 x_1 + \cdots a_n x_n\}.
\end{multline*}
%
We note that the first constraint is non-linear, due to the product on the left of the equality, and it might seem that this would result in a worse encoding w.r.t.\ a standard encoding via linear constraints. However, we recall that the standard encoding for the indicator constraint via linear constraints requires finding a constant $M$ that is guaranteed to be larger than $a_1 x_1 + \cdots a_n x_n$, for \emph{all} values of $x_1,\ldots,x_n$. A preliminary analysis has shown that such a constant $M$ would be extremely large, and caused numerical instabilities while solving the ILP encodings, and thus cannot be employed for our implementation. 
%
Nonetheless, as we are going to see next, we will exploit a state-of-the-art solver that natively supports quadratic constraints.

\medskip
\noindent
\textbf{Finding Optimal Solutions.}
For solving the $(T,k)$-problem $(f,S)$ we use Gurobi~\cite{gurobi}, which is a state-of-the-art Mixed-Integer (Quadratic) Programming solver.

%implementation aspects that are not explicit in the formal ILP encoding and its characterizations but are important for interpreting the results. The algorithm first computes the downward closure of the target fact, constructs the corresponding ILP maximization problem in C++, and solves it using Gurobi~\cite{gurobi}. A lightweight Java layer is used only as a wrapper.
%
%Variables are generated only for facts and proof elements appearing in the downward closure. Facts outside this reduced structure cannot participate in any derivation of the target and therefore do not require decision variables. This reduces the size of the optimization problem without affecting correctness.
%
%For the hypergraph-based characterization, we implement the system of constraints directly using integer variables for the multiplicities of hyperedges and binary variables for database facts. Reachability from the target fact is enforced using the flow-based constraints over the directed graph induced by the hyperedges, as described in Section~\ref{sec:hypergraph-based}.
%
%A key practical choice concerns constraints of the form
%$z_\alpha \equiv I_\alpha + O_\alpha \geq 1$. Rather than relying on Gurobi's native indicator constraints, we encode this equivalence explicitly. Here, $I_\alpha$ and $O_\alpha$ are the expressions used in the hypergraph-based characterization to count, respectively, the selected incoming and outgoing hyperedges of the node $\alpha$, and $z_\alpha$ is the binary variable indicating whether $\alpha$ occurs in the selected description. We enforce the equivalence using the constraints $z_\alpha \cdot (I_\alpha + O_\alpha) = I_\alpha + O_\alpha$ and $z_\alpha \leq I_\alpha + O_\alpha.$ These constraints ensure that $z_\alpha = 0$ implies $I_\alpha + O_\alpha = 0$, while $I_\alpha + O_\alpha \geq 1$ implies $z_\alpha = 1$. This avoids introducing large auxiliary constants to simulate conditional constraints and results in a more compact formulation. The same implementation choice is used to link the auxiliary variables $\hat{x}_{(\alpha,T)}$ with the corresponding hyperedge-multiplicity variables $x_{(\alpha,T)}$.
%
%For the graph-based ILP characterization, we implement the system of constraints over binary variables. The variables that are true in a solution induce the nodes and edges of a proof DAG. The diversity objective is implemented as in the $(T,k)$-problem. We create $k$ copies of the chosen base ILP encoding. For each pair of copies and each database variable, an auxiliary binary variable records whether the two induced supports differ on the corresponding database fact. Maximizing the sum of these
%auxiliary variables maximizes the total pairwise symmetric-difference distance, while the additional constraints
%ensure that the $k$ induced supports are pairwise distinct.

\begin{table}[t]
	\centering
	\resizebox{\columnwidth}{!}{%
	\begin{tabular}{lccc}
		\toprule
		Name & Databases & \#Rules & Rec. \\
		\midrule
		
		\multirow{2}{*}{%
		\begin{tabular}{@{}l@{}}
		\graphanalytics \\
		(transitive closure)
		\end{tabular}}
		& \bitcoin~\cite{kumar2016edge} \text{(235K)} & \multirow{2}{*}{2} & \multirow{2}{*}{Yes} \\
		& \facebook~\cite{snap} \text{(88.2K)} & & \\
		
		\midrule
		
		\doctors(1--7)~\cite{elhalawati2022existential}
		& \factsk \text{(100K)} & 6 & No \\
		
		\midrule
		
		\multirow{2}{*}{\galen~\cite{elhalawati2022existential}}
		& \fifteen \text{(26.5K)}, \forty \text{(67K)} & \multirow{2}{*}{14} & \multirow{2}{*}{Yes} \\
		& \twentyfive \text{(30.5K)}, \fifty \text{(82K)} & & \\
		
		\midrule
		
		\multirow{2}{*}{\csda~\cite{fan2019scaling}}
		& \httpd \text{(10M)}, \linux \text{(44M)} & \multirow{2}{*}{2} & \multirow{2}{*}{Yes} \\
		& \postgres \text{(34.8M)} & & \\
		
		\bottomrule
	\end{tabular}%
	}
	\medskip
	\caption{Experimental scenarios. For each database, we give in parenthesis the number of tuples. ``Rec.'' indicates whether the rule set is recursive.}
	\label{tab:scenarios}
\end{table}

\subsection{Experimental Setup} 

We now describe the databases, procedure, and system configuration used in our evaluation.

\medskip
\noindent \textbf{Experimental Scenarios.} We consider the scenarios listed in Table~\ref{tab:scenarios}; sources for all scenarios and datasets are given in the table. The \graphanalytics\ scenario consists of a simple transitive-closure workload evaluated over real-world graph datasets (\bitcoin\ and \facebook). The \csda\ scenario also involves recursive queries over large real-world databases such as \httpd, \postgres, and \linux. The \doctors\ and \galen\ scenarios contain richer rule sets with varying database sizes. Together, these represent standard benchmark scenarios from the Datalog literature.

\medskip
\noindent \textbf{Procedure.} For each scenario $D$ and $Q$, we compute $Q(D)$ using DLV~\cite{adrian2018dlv} and uniformly select 100 answer tuples at random from the query result. For each selected tuple, we construct its downward closure, i.e., the sub-hypergraph capturing all possible derivations relevant to the tuple. Following~\cite{CLPS24aaai}, the downward closure is computed by evaluating a modified Datalog query over a modified database, whose answers coincide with the hyperedges of the downward closure. This allows us to use the same Datalog engine both for query answering and for explanation construction. We then generate the corresponding ILP formulation and solve the resulting optimization problem using Gurobi to compute a set of $k$ explanations maximizing diversity. Each run is subject to a timeout of 10 minutes per tuple.

\medskip
\noindent \textbf{System Details.} All experiments were conducted on a server running Fedora Linux 39 (Cloud Edition), provisioned with 20 vCPUs (Intel Xeon Processor, Cascadelake) and 117GB of RAM. The ILP models are constructed in C++ and solved using Gurobi11.0.0~\cite{gurobi}. Python 3.12.7 is used for preprocessing.

\input{exact-results}

\subsection{Experimental Results} \label{sec:exp-results-exact}
    
Figures~\ref{fig:csda-httpd-exact}--\ref{fig:galen-exact} show the runtime distribution of the exact method as $k$ increases, across different databases and configurations. Each figure includes violin/box plots and individual runtime points. Black points show successful runs, while red points show timeouts; the red percentages report the timeout rate. For clarity, boxplots are shown without outliers.

To compare different values of $k$ fairly, we only include goal tuples with at least five explanations. Goals with fewer explanations would make larger values of $k$ infeasible and bias the results. As a result, very few \galen goals remained, since most \galen goals have only one explanation. Therefore, for \galen, Figure~\ref{fig:galen-exact} reports results only for $k=1$.


The results show that the exact algorithm performs well for small values of $k$, where optimal diverse explanations can be computed within short runtimes. However, as predicted by the theoretical analysis (Theorem~\ref{the:diverse-answers}), scalability quickly degrades as $k$ increases. For $k=4$ and $k=5$, many runs reach the 10-minute timeout limit, often dominating the results (e.g., Figure~\ref{fig:graph-analytics-facebook-exact}). This behavior is driven by the combinatorial nature of the problem: as $k$ increases, the number of possible combinations of explanations and interactions among them grows rapidly, substantially enlarging the search space explored by the optimizer. While the ILP formulation also becomes larger as $k$ increases, the dominant factor is the exponential growth in the underlying solution space rather than the encoding size itself. As a result, runtimes grow from milliseconds to seconds and minutes, often exhibiting an exponential trend as $k$ increases (all plots use a log scale). The increasing fraction of timeouts, shown by the red percentages in the figures, confirms the scalability limitations of the exact approach and motivates the approximate methods evaluated in Section~\ref{sec:approximate-experiments}.

A further observation from Figures~\ref{fig:csda-httpd-exact}-\ref{fig:galen-50-exact} is that, when comparing arbitrary and unambiguous proofs under the same characterization (i.e., the hypergraph-based characterization, since for the DAG-based characterization we have only results for unambiguous proofs), the runtimes are often very similar and in many cases nearly overlap. This is encouraging, as it indicates that generating unambiguous explanations---which are generally more informative and avoid redundant derivations---incurs little additional cost compared to arbitrary explanations that consider all derivations. Thus, obtaining higher-quality explanations through unambiguous semantics appears to come almost for free in practice. We observe a similar behavior later for the approximate algorithm, suggesting that the cost of enforcing unambiguity remains limited across both the exact and approximate algorithms.

Another observation is that \dagEnc and \hypergraph have comparable runtimes in many scenarios. However, Figure~\ref{fig:timeouts} highlights cases where \dagEnc underperforms and produces many timeouts, meaning that it cannot generate explanations within the time limit. In contrast, \hypergraph generates the explanations without timing out in these cases. The figure reports the number of variables in \dagEnc. A larger number of variables makes the cycle-checking component of the encoding more expensive. The timeouts are mainly observed when the number of variables is large, suggesting that this cycle-checking step is a key bottleneck of \dagEnc compared with \hypergraph.

Overall, the exact algorithm is effective for finding diverse explanations for small values of $k$, where runtimes remain low across most scenarios. At the same time, the observed exponential growth trend and the rapidly increasing number of timeouts confirm that exact algorithm becomes infeasible for larger values of $k$. This motivates the need for approximate methods, which is the subject of the next section.

\input{downward-results}

==> figures/experiments.tex <==
\section{Experiments}

We now proceed to experimentally evaluate the SAT-based framework for computing diverse why-provenance explanations. Our evaluation has three main objectives. First, we compare the two solution strategies introduced earlier, namely the \emph{optimal} approach that computes a diversity-maximizing set of explanations in a single step, and the \emph{greedy} approach that incrementally constructs such a set, in terms of both runtime and achieved diversity. Second, we assess the impact of the underlying encoding technique used for constructing the Boolean formula, namely the \emph{DAG-based} encoding and the \emph{hypergraph-based} encoding, on performance and scalability. Third, we study the effect of the provenance semantics, by comparing standard why-provenance with its refinement based on unambiguous proof trees (see Section~\ref{sec:why-prov}), on both the size and the quality of the generated explanations.

\medskip
\noindent \textbf{Experimental Setup.}

\smallskip
\noindent \emph{Datasets.}
We consider a variety of scenarios from the Datalog literature consisting of a query $Q = (\dep,R)$ and a family of databases $\mathcal{D}$ over $\esch{\dep}$. All the considered scenarios are summarized in Table~\ref{tab:scenarios}; further details about the scenarios can be found in the appendix.

\smallskip
\noindent \emph{Configurations.}
Our evaluation considers all combinations of the design choices introduced in the previous sections. In particular, we compare the \emph{optimal} and \emph{greedy} strategies for computing a set of $k$ explanations, two alternative encodings of the problem into Boolean formulas, namely the \emph{DAG-based} and \emph{hypergraph-based} encodings, and two provenance semantics, namely standard why-provenance and its restriction to unambiguous proof trees. Each experimental result corresponds to one such configuration.

\smallskip
\noindent \emph{Evaluation Measures.}
We evaluate each configuration along two main dimensions. The first is \emph{runtime}, measured as the total end-to-end time required to compute a set of $k$ explanations for a given answer tuple, including the construction of the downward closure, the generation of the Boolean formula, and the execution of the SAT solver. The second is \emph{diversity}, measured using the diversity function $\delta(\cdot)$ defined in Section~4, which captures the pairwise symmetric differences between the selected explanations. When full enumeration is not feasible, we also report the number of explanations generated within the given time budget.

\smallskip
\noindent \emph{Procedure.}
For each scenario $s$ and each $D \in \mathcal{D}$, we compute $Q(D)$ using DLV and select 100 tuples $\bar t^1_{s,D},\ldots,\bar t^{100}_{s,D}$ uniformly at random, leading to a total of 1500 why-provenance instances. For each tuple $\bar t^i_{s,D}$, we construct the downward closure of $R(\bar t^i_{s,D})$ with respect to $D$ and $\dep$ by first computing the adapted query $Q_{\downarrow}$ and database $D_{\downarrow}$ via a Python 3 implementation, and then evaluating it using DLV. Based on the resulting closure, we generate a Boolean formula $\phi_{(\bar t^i_{s,D},D,Q)}$ using a C++ implementation.

We then invoke the SAT solver \emph{Glucose} (version 4.2.1)~\cite{Audemard18} to enumerate explanations. Depending on the configuration, the solver is used either to compute an optimal set of $k$ explanations or to iteratively construct such a set via the greedy strategy. Since the size of the why-provenance can be extremely large, we limit the enumeration phase to at most 10K explanations or a timeout of 5 minutes per tuple, whichever occurs first.

\smallskip
\noindent \emph{System Details.}
All experiments were conducted on a laptop equipped with an Intel(R) Core(TM) i7-10750H CPU @ 2.60GHz and 32GB of RAM, running Fedora Linux 37. The Python components were executed using Python 3.11.2, while the C++ code was compiled with \texttt{g++} 12.2.1 using the \texttt{-O3} optimization flag.

{\footnotesize 
	\begingroup
	\setlength{\tabcolsep}{5pt} % Default value: 6pt
	\renewcommand{\arraystretch}{1.4} % Default value: 1
	\begin{table}[t]
		\centering
		\begin{tabular}{|c||c|c|c|}
			\hline
			\small \textbf{Scenario} & \small \textbf{Databases} & \small \textbf{\#Rules} & \small \textbf{Recursive}\\ \hline
			\hline
			$\substack{\mathsf{TransClosure}}$ & $\substack{D_\mathsf{bitcoin} \text{(235K)}, D_\mathsf{facebook} \text{(88.2K)}}$ & \small 2 & \small {51}\\ \hline
			$\substack{\mathsf{Doctors\text{-}}i,\\ i \in [7]}$& $\substack{D_1 \text{(100K)}}$ & \small 6 & \small {55}\\ \hline
			$\substack{\mathsf{Galen}}$ & $\substack{D_1 \text{(26.5K)}, D_2 \text{(30.5K)},\\D_3 \text{(67K)}, D_4 \text{(82K)}}$ & \small 14 & \small {51}\\ \hline
			$\substack{\mathsf{Andersen}}$ & $\substack{D_1 \text{(68K)}, D_2 \text{(340K)},\\D_3 \text{(680K)}, D_4 \text{(3.4M)}, D_5 \text{(6.8M)}}$ & \small4 & \small {51}\\ \hline
			$\substack{\mathsf{CSDA}}$ & $\substack{D_\mathsf{httpd} \text{(10M)}, D_\mathsf{postgresql} \text{(34.8M)},\\ D_\mathsf{linux} \text{(44M)}}$ & \small 2 & \small {51}\\ \hline
		\end{tabular}
		\caption{Experimental scenarios. For each database $D$, we give in parenthesis the number of tuples occurring in $D$.}
		\label{tab:scenarios}
	\end{table}
	\endgroup
}



\medskip
\noindent \textbf{Experimental Results.} 
Missing...

\input{exact-exp}

\input{approximate-exp}

\input{ratios-exp}








==> figures/extras.tex <==
% With not much additional overhead, we can find useful, unambiguous ones

% downward closure size and its impact on, trying plots with downward closure size in x and time in y

% Beyond the overall scalability trend, the results also reveal differences in runtime variability and encoding behavior. For small values of $k$, runtimes are tightly concentrated, indicating stable and predictable performance (e.g., Figures~\ref{fig:csda-postgresql-exact} and~\ref{fig:csda-linux-exact}). As $k$ increases, the distributions become wider and more skewed, showing substantially higher variance across instances, even before reaching the timeout threshold, which is typical for combinatorial optimization problems such as ILP.

% The number of evaluated goals also varies across configurations. In general, arbitrary semantics produce more explanations than unambiguous semantics, making larger values of $k$ more likely. Consequently, some settings contain more evaluated goals under arbitrary semantics (e.g., the \forty and \fifty databases in \galen; Figures~\ref{fig:galen-40-exact} and~\ref{fig:galen-50-exact}).

% Finally, there is no consistent winner between the hypergraph- and DAG-based encodings. Hypergraph encodings are faster in some cases (e.g., \doctors in Figures~\ref{fig:doctors-q01-100k-exact}-\ref{fig:doctors-q07-100k-exact}), while DAG encodings perform better in others (e.g., Figures~\ref{fig:csda-linux-exact} and~\ref{fig:galen-50-exact}). This suggests that performance depends more on the structure of the downward closure and the resulting ILP instance than on the encoding itself.

==> figures/introduction.tex <==
\section{Introduction}
Missing...

==> figures/macros.tex <==
\newcommand{\from}[3]{\textbf{FROM} #1 \textbf{TO} #2: #3}
\DeclareMathOperator*{\argmax}{arg\,max}
%Complexity classes
\def\FP{\text{\rm FP}}
\def\FL{\text{\rm FL}}
\def\spanL{\text{\rm SpanL}}
\def\spanLL{\text{\rm SpanLL}}
\def\sharpP{\text{\rm \#P}}
\def\sharpL{\text{\rm \#L}}
\def\NL{\text{\rm NL}}
\def\PTIME{\text{\rm P}}
\def\PH{\text{\rm PH}}
\def\NP{\text{\rm NP}}
\def\LOGSPACE{\text{\rm L}}
\def\NSPACE{\rm NSPACE}
\def\NTIME{\rm NTIME}
\def\co{\rm co\text{-}}
\def\PSPACE{\rm PSPACE}
\def\EXPTIME{\rm EXPTIME}
\def\NEXP{\rm NEXPTIME}
\def\TWOEXPTIME{\rm 2EXPTIME}
\def\AEXSPACE{\rm AEXSPACE}
\def\ACZ{\rm AC_0}
\def\hard{\rm \text{-}hard}
\def\complete{\text{-{\rm complete}}}
\def\assign{ \text{:--} }
%\def\assign{\leftarrow}

\newcommand\sem[1]{{[\![ #1 ]\!]}}
\newcommand{\db}[1]{\mathsf{db}(#1)}
\newcommand{\depth}[1]{\mathsf{depth}(#1)}
\newcommand{\scount}[1]{\mathsf{scount}(#1)}
\newcommand{\mintdepth}[3]{\mathsf{min\!-\!tree\!-\!depth}(#1,#2,#3)}
\newcommand{\mingdepth}[3]{\mathsf{min\!-\!dag\!-\!depth}(#1,#2,#3)}
\newcommand{\mintrees}[3]{\mathsf{min\!-\!trees}(#1,#2,#3)}
\newcommand{\hmintrees}[3]{\mathsf{hmin\!-\!trees}(#1,#2,#3)}
\newcommand{\mindags}[3]{\mathsf{min\!-\!dags}(#1,#2,#3)}
\newcommand{\hmindags}[3]{\mathsf{hmin\!-\!dags}(#1,#2,#3)}
\newcommand{\tuptrees}[3]{\mathsf{trees}(#1,#2,#3)}
\newcommand{\tupdags}[3]{\mathsf{dags}(#1,#2,#3)}
\newcommand{\rank}[2]{\mathsf{rank}_{#2}(#1)}
\newcommand{\sdepth}[1]{\star\text{-}\mathsf{depth}(#1)}
\newcommand{\mh}[1]{\mathsf{mh}(#1)}
\newcommand{\ma}[1]{\mathsf{ma}(#1)}
\newcommand{\md}[1]{\mathsf{md}(#1)}
\newcommand{\smd}[1]{\star\text{-}\mathsf{md}(#1)}
\newcommand{\omd}[1]{\obl\text{-}\mathsf{md}(#1)}
%graph structures
\newcommand{\gforest}[1]{\mathsf{gforest}(#1)}
\newcommand{\gtree}[1]{\mathsf{gtree}(#1)}
\newcommand{\slinpath}[1]{simple linear $#1$-path}
\newcommand{\linpath}[1]{linear $#1$-path}
\newcommand{\guardedpath}[1]{guarded $#1$-path}
\newcommand{\stickypath}[1]{sticky $#1$-path}
\newcommand{\R}{\mathcal{R}}
\newcommand{\Lang}{\mathcal{L}}
\newcommand{\mi}[1]{\mathit{#1}}
\newcommand{\ins}[1]{\mathbf{#1}}
\newcommand{\adom}[1]{\mathsf{dom}(#1)}
%\renewcommand{\paragraph}[1]{\textbf{#1}}
\newcommand{\ra}{\rightarrow}
\newcommand{\fr}[1]{\mathsf{fr}(#1)}
\newcommand{\dep}{\Sigma}
\newcommand{\sch}[1]{\mathsf{sch}(#1)}
\newcommand{\esch}[1]{\mathsf{edb}(#1)}
\newcommand{\isch}[1]{\mathsf{idb}(#1)}
\newcommand{\sign}{\ins{S}}
\newcommand{\body}[1]{\mathsf{body}(#1)}
\newcommand{\head}[1]{\mathsf{head}(#1)}
\newcommand{\guard}[1]{\mathsf{guard}(#1)}
\newcommand{\class}[1]{\mathsf{#1}}
\newcommand{\pos}[1]{\mathsf{pos}(#1)}
\newcommand{\spos}[1]{\mathsf{spos}(#1)}
%\newcommand{\app}[2]{\xrightarrow{#1,#2}}
\newcommand{\app}[2]{\langle #1,#2 \rangle}
\newcommand{\tup}[1]{\langle #1 \rangle}
\newcommand{\crel}[1]{\prec_{#1}}
\newcommand{\tcrel}[1]{\prec_{#1}^{\star}}
\newcommand{\rctaa}{\class{CT}_{\forall \forall}^{\mathsf{res}}}
\newcommand{\rctaapr}{\mathsf{CT}_{\forall \forall}^{\mathsf{res}}}
\newcommand{\rctae}{\class{CT}_{\forall \exists}^{\mathsf{res}}}
\newcommand{\rctaepr}{\mathsf{CT}_{\forall \exists}^{\mathsf{res}}}
\newcommand{\base}[1]{\mathsf{base}(#1)}
\newcommand{\eqt}[1]{\mathsf{eqtype}(#1)}
\newcommand{\var}[1]{\mathsf{var}(#1)}
\newcommand{\vr}[1]{\langle #1 \rangle}
\newcommand{\const}[1]{\mathsf{const}(#1)}
\newcommand{\result}[2]{\mathsf{result}(#1,#2)}
\newcommand{\soresult}[2]{\sobl\text{-}\mathsf{result}(#1,#2)}
\newcommand{\oresult}[2]{\obl\text{-}\mathsf{result}(#1,#2)}
\newcommand{\sresult}[2]{\star\text{-}\mathsf{result}(#1,#2)}

\newcommand{\diff}[2]{\Delta(#1,#2)}
\newcommand{\dist}[2]{d(#1,#2)}
\newcommand{\diversity}[1]{\delta(#1)}
\newcommand{\diversitytup}[1]{\delta(#1)}

\newcommand{\lsign}[1]{\mathsf{b}(#1)}
\newcommand{\lvar}[1]{\mathsf{v}(#1)}

\newcommand{\reach}[1]{\rightsquigarrow_{#1}}
%\newcommand{\terms}[1]{\mathsf{terms}(#1)}
\newcommand{\obl}{\mathsf{o}}
\newcommand{\sobl}{\mathsf{so}}
\newcommand{\std}{\mathsf{std}}
\newcommand{\cta}[1]{\class{CT}_{\forall \forall}^{#1}}
\newcommand{\cte}[1]{\class{CT}_{\forall \exists}^{#1}}

\newcommand{\ctda}[2]{\class{CT}_{\forall,#2}^{#1}}
\newcommand{\ctde}[2]{\class{CT}_{\exists,#2}^{#1}}

\newcommand{\ct}[1]{\class{CT}_{\forall}^{#1}}
\newcommand{\ctd}[2]{\class{CT}^{#1}_{#2}}
\newcommand{\ctapr}[1]{\mathsf{CT}_{\forall \forall}^{#1}}
\newcommand{\ctepr}[1]{\mathsf{CT}_{\forall \exists}^{#1}}
\newcommand{\ctdapr}[1]{\mathsf{CT}_{\forall}^{#1}}
\newcommand{\ctdepr}[1]{\mathsf{CT}_{\exists}^{#1}}
\newcommand{\ctpr}[1]{\mathsf{CT}_{\forall}^{#1}}
\newcommand{\ctdpr}[1]{\mathsf{CT}^{#1}}
\newcommand{\cri}[1]{\mathsf{cr}(#1)}
\newcommand{\lin}[1]{\mathsf{Lin_{\class{S}}}(#1)}
\newcommand{\ling}[1]{\mathsf{lin}(#1)}
\newcommand{\shape}[1]{\mathsf{shape}(#1)}
\newcommand{\svar}[1]{\mathsf{svar}(#1)}
\newcommand{\constfree}[1]{\mathsf{c\text{-}free}(#1)}
\newcommand{\id}[2]{\mathsf{id}_{#1}(#2)}
\newcommand{\unique}[1]{\mathsf{unique}(#1)}
\newcommand{\simple}[1]{\mathsf{simple}(#1)}
\newcommand{\gsimple}[1]{\mathsf{gsimple}(#1)}
\def\sub{\sqsubseteq}
\def\substrict{\sqsubset}

\newcommand{\rew}[1]{\hat{#1}}
\newcommand{\whichver}[1]{#1^w}
\newcommand{\support}[1]{\mathsf{support}(#1)}
\newcommand{\bagsupport}[1]{\mathsf{bagsupport}(#1)}
\newcommand{\indegree}[2]{\mathsf{in}_{#2}(#1)}
\newcommand{\outdegree}[2]{\mathsf{out}_{#2}(#1)}
\newcommand{\inflow}[1]{\mathcal{F}^{\mathsf{in}}_{#1}}
\newcommand{\outflow}[1]{\mathcal{F}^{\mathsf{out}}_{#1}}
%\newcommand{\C}[1]{\mathsf{C}(#1)}
\newcommand{\norm}[1]{\mathsf{Norm}(#1)}
\newcommand{\depg}[1]{\mathsf{dg}(#1)}
\newcommand{\edepg}[1]{\mathsf{edg}(#1)}
\newcommand{\sodg}[1]{\mathsf{so\text{-}dg}(#1)}
\newcommand{\odg}[1]{\mathsf{o\text{-}dg}(#1)}
\newcommand{\ex}[1]{\mathsf{exvar}(#1)}
\newcommand{\mgu}[2]{\mathsf{mgu}(#1,#2)}
\newcommand{\res}[1]{\mathsf{res}(#1)}
\newcommand{\f}[2]{f_{#1}(#2)}
\newcommand{\arity}[1]{\mathsf{ar}(#1)}
\newcommand{\atoms}[1]{\mathsf{atoms}(#1)}
\newcommand{\lfacts}[1]{\mathsf{LFacts}(#1)}
\newcommand{\why}[3]{\mathsf{why}(#1,#2,#3)}
\newcommand{\whyk}[4]{\mathsf{why}^{#1}(#2,#3,#4)}
\newcommand{\trio}[3]{\mathsf{trio}(#1,#2,#3)}
\newcommand{\which}[3]{\mathsf{which}(#1,#2,#3)}
\newcommand{\whichnr}[3]{\mathsf{which}_{\mathsf{NR}}(#1,#2,#3)}
\newcommand{\whichun}[3]{\mathsf{which}_{\mathsf{UN}}(#1,#2,#3)}
\newcommand{\whichstar}[3]{\mathsf{which}_{\star}(#1,#2,#3)}
\newcommand{\posbool}[3]{\mathsf{posbool}(#1,#2,#3)}
\newcommand{\posboolnr}[3]{\mathsf{posbool}_{\mathsf{NR}}(#1,#2,#3)}
\newcommand{\posboolun}[3]{\mathsf{posbool}_{\mathsf{UN}}(#1,#2,#3)}
\newcommand{\bx}[3]{\mathbb{B}(#1,#2,#3)}
\newcommand{\bxnr}[3]{\mathbb{B}_{\mathsf{NR}}(#1,#2,#3)}
\newcommand{\bxun}[3]{\mathbb{B}_{\mathsf{UN}}(#1,#2,#3)}
\newcommand{\nx}[3]{\mathbb{N}(#1,#2,#3)}
\newcommand{\nrwhy}[3]{\mathsf{why}_{\mathsf{NR}}(#1,#2,#3)}
\newcommand{\mdwhy}[3]{\mathsf{why}_{\mathsf{MD}}(#1,#2,#3)}
\newcommand{\mtd}[3]{\mathsf{min\text{-}tree\text{-}depth}(#1,#2,#3)}
\newcommand{\mgd}[3]{\mathsf{min\text{-}dag\text{-}depth}(#1,#2,#3)}
\newcommand{\starwhy}[3]{\mathsf{why}_{\star}(#1,#2,#3)}
\newcommand{\starwhyk}[4]{\mathsf{why}_{\star}^{#1}(#2,#3,#4)}
\newcommand{\allwhy}[3]{\mathsf{why}_{\mathsf{ALL}}(#1,#2,#3)}
\newcommand{\unwhy}[3]{\mathsf{why}_{\mathsf{UN}}(#1,#2,#3)}
\newcommand{\unwhyk}[4]{\mathsf{why}_{\mathsf{UN}}^{#1}(#2,#3,#4)}
\newcommand{\nrtrio}[3]{\mathsf{trio}_{\mathsf{NR}}(#1,#2,#3)}
\newcommand{\untrio}[3]{\mathsf{trio}_{\mathsf{UN}}(#1,#2,#3)}
\newcommand{\precnode}[1]{\prec_{#1}}
\newcommand{\repr}[2]{\mathsf{repr}_{#2}(#1)}
\newcommand{\reprtree}[2]{\mathsf{reprTrees}^{#1}(#2)}
\newcommand{\childlabels}[1]{\mathsf{child\textrm{-}labels}(#1)}
\newcommand{\birth}[2]{\mathsf{birth}_{#1}(#2)}
\newcommand{\OMIT}[1]{}
\newcommand{\crt}[1]{\texttt{cr}(#1)}
\newcommand{\precd}[1]{\prec_{#1}}
\newcommand{\level}[2]{\mathsf{lvl}_{#2}(#1)}
\newcommand{\lvl}[2]{\texttt{lv}_{#1}(#2)}
\newcommand{\posvar}[2]{\mathsf{pos}(#1,#2)}
\newcommand{\posterm}[2]{\mathsf{pos}(#1,#2)}
\newcommand{\varpos}[2]{\mathsf{var}(#1,#2)}
\newcommand{\termpos}[2]{\mathsf{term}(#1,#2)}
\newcommand{\CT}[2]{\mathsf{CT}^{#1}_{#2}}
\newcommand{\frpos}[1]{\mathsf{frpos}(#1)}
\newcommand{\dom}{\mathbf{C}}
\newcommand{\freshdom}{\mathbf{N}}
\newcommand{\frontier}[1]{\mathsf{fr}(#1)}
\newcommand{\eqtype}[1]{\mathsf{eqtype}(#1)}

\newcommand{\whymult}[3]{\mathsf{whymult}_{\mathsf{ALL}}(#1,#2,#3)}
\newcommand{\nrwhymult}[3]{\mathsf{whymult}_{\mathsf{NR}}(#1,#2,#3)}
\newcommand{\unwhymult}[3]{\mathsf{whymult}_{\mathsf{UN}}(#1,#2,#3)}
\newcommand{\vecenc}[1]{\mathsf{vec}(#1)}
\newcommand{\ground}[2]{\mathsf{gg}(#1,#2)}
\newcommand{\groundh}[2]{\mathsf{gh}(#1,#2)}
\newcommand{\multiset}[1]{\{\!\{ #1 \}\!\}}
\newcommand{\card}[2]{|#2(#1)|}
\newcommand{\nodes}[1]{V_{#1}}
\newcommand{\hypergraphof}[1]{\mathcal{H}_{#1}}

\newcommand{\cliques}[2]{\mathsf{cliques}^{#1}(#2)}
\newcommand{\ilphypergraph}[3]{\mathsf{hyper\text{-}ILP}_{\mathsf{ALL}}(#1,#2,#3)}
\newcommand{\ilpunhypergraph}[3]{\mathsf{hyper\text{-}ILP}_{\mathsf{UN}}(#1,#2,#3)}
\newcommand{\ilpstarhypergraph}[3]{\mathsf{hyper\text{-}ILP}_{\star}(#1,#2,#3)}
\newcommand{\ilpproofdag}[3]{\mathsf{dag\text{-}ILP}_{\mathsf{ALL}}(#1,#2,#3)}
\newcommand{\ilpunproofdag}[3]{\mathsf{dag\text{-}ILP}_{\mathsf{UN}}(#1,#2,#3)}
\newcommand{\ilpstarproofdag}[3]{\mathsf{dag\text{-}ILP}_{\star}(#1,#2,#3)}
\newcommand{\ilpstargamma}[3]{\mathsf{\gamma\text{-}ILP}_{\star}(#1,#2,#3)}

\newcommand{\ComputeDiverse}[2]{(#1,#2)\text{-}\mathsf{ComputeDiverse}}

\newcommand{\boundall}[3]{\mathsf{bound}_{\mathsf{ALL}}(#1,#2,#3)}
\newcommand{\boundun}[3]{\mathsf{bound}_{\mathsf{UN}}(#1,#2,#3)}

\newcommand{\sol}[1]{\mathsf{sol}(#1)}
\newcommand{\opt}[1]{\mathsf{opt}(#1)}
\newcommand{\solon}[2]{\mathsf{sol}(#1)_{|#2}}
\newcommand{\opton}[2]{\mathsf{opt}(#1)_{|#2}}
\newcommand{\proj}[2]{#1_{|#2}}
\newcommand{\copyof}[2]{#1^{(#2)}}
\newcommand{\auxvar}{\mathsf{aux}}
\newcommand{\hammd}[2]{\mathsf{hd}(#1,#2)}
\newcommand{\ansk}[3]{\mathsf{ans}^{#1}(#2,#3)}

\def\iso{\simeq}
\newcommand{\can}[1]{\mathsf{can}(#1)}
%\newcommand{\proj}[2]{\Pi_{#1}(#2)}
\newcommand{\pred}[1]{\mathit{pred}(#1)}
\newcommand{\predt}[1]{[#1]}
\newcommand{\atom}[1]{\underline{#1}}
\newcommand{\tuple}[1]{\bar{#1}}
\newcommand{\resolv}[1]{[#1]}
\newcommand{\parent}[1]{\mathit{par}(#1)}
\newcommand{\dept}[1]{\mathit{depth}(#1)}
\newcommand{\chase}[2]{\mathsf{chase}(#1,#2)}
\newcommand{\chasesize}[2]{\mathsf{chsize}(#1,#2)}
\newcommand{\starchasei}[3]{\star\text{-}\mathsf{chase}^{#3}(#1,#2)}
\newcommand{\starchase}[2]{\star\text{-}\mathsf{chase}(#1,#2)}
\newcommand{\sochasei}[3]{\sobl\text{-}\mathsf{chase}^{#3}(#1,#2)}
\newcommand{\sochase}[2]{\sobl\text{-}\mathsf{chase}(#1,#2)}
\newcommand{\ochasei}[3]{\obl\text{-}\mathsf{chase}^{#3}(#1,#2)}
\newcommand{\ochase}[2]{\obl\text{-}\mathsf{chase}(#1,#2)}
\newcommand{\completion}[2]{\mathsf{complete}(#1,#2)}
\newcommand{\mar}[1]{\hat{#1}}
\newcommand{\nullobl}[3]{\bot^{#1}_{#2,#3}}
\newcommand{\nullsobl}[3]{\bot^{#1}_{#2,#3_{|\frontier{#2}}}}
\newcommand{\startype}[1]{\star\textrm{-}\mathsf{type}(#1)}
\newcommand{\type}[2]{\mathsf{type}_{#1}(#2)}
\newcommand{\types}[2]{#1\textrm{-}\mathsf{types}(#2)}
\newcommand{\src}[1]{\mathsf{src}(#1)}
\newcommand{\IDTGD}{\class{ID}}
\newcommand{\DLLITETGD}{\mathsf{DL\textrm{-}Lite^{TGD}}}
\newcommand{\SLTGD}{\class{SL}}
\newcommand{\LDAT}{\class{LDat}}
\newcommand{\NRDAT}{\class{NRDat}}
\newcommand{\GDAT}{\class{G}}
\newcommand{\WGTGD}{\class{WG}}
\newcommand{\RATGD}{\class{RA}}
\newcommand{\LARATGD}{\class{LARA}}
\newcommand{\LCRATGD}{\class{LCRA}}
\newcommand{\LCWATGD}{\class{LCWA}}
\newcommand{\WATGD}{\class{WA}}
\newcommand{\DAT}{\class{Dat}}
\newcommand{\UCQ}{\class{UCQ}}
\newcommand{\SLRATGD}{\class{SLRA}}
\newcommand{\SLWATGD}{\class{SLWA}}
\newcommand{\LRATGDP}{\class{LRA}^{+}}
\newcommand{\LWATGDP}{\class{LWA}^{+}}
\newcommand{\oblrew}[1]{\mathsf{enrichment}(#1)}

\def\eqtree{\approx}
\newcommand{\downof}[2]{#1_{\downarrow#2}}
\newcommand{\gri}[2]{\mathsf{gri}(#1,#2)}
\newcommand{\downc}[3]{\mathsf{down}(#1,#2,#3)}
\newcommand{\quot}[1]{#1_{/\eqtree}}
\newcommand{\leaves}[1]{\mathsf{leaves}(#1)}
\newcommand{\dgt}[1]{\mathsf{dag}(#1)}
\newcommand{\cq}[1]{\mathsf{cq}(#1)}
\newcommand{\cqs}[2]{\mathsf{cq}(#1,#2)}
\newcommand{\cqsu}[2]{\mathsf{cq}(#1,#2)}
\newcommand{\cqseq}[2]{\mathsf{cq}^{=}(#1,#2)}
\newcommand{\cqeq}[1]{\mathsf{cq}^{\approx}(#1)}
\newcommand{\cqeqs}[1]{\mathsf{cqs}^{=}(#1)}
\newcommand{\fo}[1]{\Psi_{#1}}
\newcommand{\fod}[1]{\Xi_{#1}}
\newcommand{\cnf}[3]{\phi_{#1,#2,#3}}
\newcommand{\trees}[1]{\mathsf{TR}(#1)}
\newcommand{\treesf}{\mathsf{TR}}
\newcommand{\utrees}[1]{\mathsf{UTR}(#1)}
\newcommand{\utreesf}{\mathsf{UTR}}
\newcommand{\spec}[1]{\mathsf{sp}(#1)}

\newcommand{\usupportp}[1]{\mathsf{USUPPORT}[#1]}
\newcommand{\nrsupportp}[1]{\mathsf{NRSUPPORT}[#1]}
\newcommand{\asupportp}[1]{\mathsf{SUPPORT}[#1]}
\newcommand{\mdsupportp}[1]{\mathsf{MDSUPPORT}[#1]}
\newcommand{\hmdsupportp}[1]{\mathsf{HMDSUPPORT}[#1]}
\def\usupportpname{\mathsf{USUPPORT}}
\def\nrsupportpname{\mathsf{NRSUPPORT}}
\def\asupportpname{\mathsf{SUPPORT}}
\def\mdsupportpname{\mathsf{MDSUPPORT}}
\def\hmdsupportpname{\mathsf{HMDSUPPORT}}

\newcommand{\qap}[1]{\mathsf{QA}[#1]}
\newcommand{\termeq}{\equiv}
\newcommand{\skolem}[3]{\bot_{#1,#2}^{#3}}
%%%%%%%%%%%%%%%%%%%%%%%%% Environment delimiters

\def\qed{\hfill{\qedboxempty}      % qed with empty box
  \ifdim\lastskip<\medskipamount \removelastskip\penalty55\medskip\fi}

\def\qedboxempty{\vbox{\hrule\hbox{\vrule\kern3pt
                 \vbox{\kern3pt\kern3pt}\kern3pt\vrule}\hrule}}

\def\qedfull{\hfill{\qedboxfull}   % qed with full box
  \ifdim\lastskip<\medskipamount \removelastskip\penalty55\medskip\fi}

\def\qedboxfull{\vrule height 4pt width 4pt depth 0pt}

\newcommand{\markfull}{\qedboxfull}
\newcommand{\markempty}{\qed} 

\newtheorem{manualtheoreminner}{Theorem}
\newenvironment{manualtheorem}[1]{%
  \renewcommand\themanualtheoreminner{#1}%
  \manualtheoreminner
}{\endmanualtheoreminner}

\newtheorem{manualpropositioninner}{Proposition}
\newenvironment{manualproposition}[1]{%
  \renewcommand\themanualpropositioninner{#1}%
  \manualpropositioninner
}{\endmanualpropositioninner}

\newtheorem{manuallemmainner}{Lemma}
\newenvironment{manuallemma}[1]{%
  \renewcommand\themanuallemmainner{#1}%
  \manuallemmainner
}{\endmanuallemmainner}

\newcommand{\triox}{\mathsf{Trio}[X]}












% ================================
% Plot / figure label macros
% ================================

% Wrapper (change here if you want different style later)
\newcommand{\plotlabel}[1]{\texttt{#1}\xspace}

% ----------------
% Strategies
% ----------------
\newcommand{\exact}{\plotlabel{exact}}
\newcommand{\approximate}{\plotlabel{approximate}}

% ----------------
% Provenance types
% ----------------
\newcommand{\arbitrary}{\plotlabel{arbitrary}}
\newcommand{\unambiguous}{\plotlabel{unambiguous}}

% ----------------
% Encodings
% ----------------
\newcommand{\dagEnc}{\plotlabel{dag}}
\newcommand{\hypergraph}{\plotlabel{hypergraph}}

% ----------------
% Combined labels (most useful)
% ----------------
\newcommand{\arbhyper}{\plotlabel{arbitrary-hypergraph}}
\newcommand{\unambhyper}{\plotlabel{unambiguous-hypergraph}}
\newcommand{\unambdag}{\plotlabel{unambiguous-dag}}

% ----------------
% Scenarios / datasets (optional)
% ----------------
\newcommand{\csda}{\plotlabel{csda}}
\newcommand{\galen}{\plotlabel{galen}}
\newcommand{\doctors}{\plotlabel{doctors}}
\newcommand{\graphanalytics}{\plotlabel{graphanalytics}}

% Example instance-level datasets (facts)
\newcommand{\httpd}{\plotlabel{httpd}}
\newcommand{\postgres}{\plotlabel{postgresql}}
\newcommand{\linux}{\plotlabel{linux}}
\newcommand{\facebook}{\plotlabel{facebook}}
\newcommand{\bitcoin}{\plotlabel{bitcoin}}
\newcommand{\factsk}{\plotlabel{100k}}
\newcommand{\fifteen}{\plotlabel{D15}}
\newcommand{\twentyfive}{\plotlabel{D25}}
\newcommand{\forty}{\plotlabel{D40}}
\newcommand{\fifty}{\plotlabel{D50}}


==> figures/preliminaries.tex <==
\section{Preliminaries}\label{sec:preliminaries}
%

We consider the disjoint countably infinite sets $\ins{C}$ and $\ins{V}$ of {\em constants} and {\em variables}, respectively. We may refer to constants and variables as {\em terms}. For an intgere $n > 0$, we write $[n]$ for the set of integers $\{1,\ldots,n\}$. In what follows, we adopt the terminology and notation from the recent work~\cite{CLPS24}, where the data complexity of why-provenance for Datalog queries has been studied.

\medskip


\noindent 
\textbf{Relational Databases.} A {\em schema} $\ins{S}$ is a finite set of relation names (or predicates) with associated arity. We write $R/n$ to say that $R$ has arity $n \ge 0$; we may also write $\arity{R}$ for $n$.
%
A {\em (relational) atom} $\alpha$ over $\ins{S}$ is an expression of the form $R(\bar t)$, where $R/n \in \ins{S}$ and $\bar t$ is an $n$-tuple of terms. By abuse of notation, we may treat tuples as the \emph{set} of their elements. A {\em fact} is an atom with only constants.
%
A {\em database} over $\ins{S}$ is a finite set of facts over $\ins{S}$. The {\em active domain} of a database $D$, denoted $\adom{D}$, is the set of constants in $D$.

\medskip
\noindent
\textbf{Syntax of Datalog Programs.} A {\em (Datalog) rule} $\sigma$ over a schema $\ins{S}$ is an expression of the form
\begin{eqnarray*}
R_0(\bar x_0) &\assign& R_1(\bar x_1),\ldots,R_n(\bar x_n)
\end{eqnarray*}
for $n \geq 1$, where $R_i(\bar x_i)$ is a (constant-free) relational atom over $\ins{S}$ for $i \in \{0,\ldots,n\}$, and each variable in $\bar x_0$ occurs in $\bar x_k$ for some $k \in [n]$.
%
We refer to $R_0(\bar x_0)$ as the {\em head} of $\sigma$, denoted $\head{\sigma}$, and to the expression $R_1(\bar x_1),\ldots,R_n(\bar x_n)$ as the {\em body} of $\sigma$, denoted $\body{\sigma}$, which we may treat as the set of its atoms.
%
A {\em Datalog program} over a schema $\ins{S}$ is a finite set $\dep$ of Datalog rules over $\ins{S}$. A predicate $R$ occurring in $\dep$ is called {\em extensional} if there is no rule in $\dep$ having $R$ in its head, and {\em intentional} if there exists at least one rule in $\dep$ with $R$ in its head.
%
The {\em extensional (database) schema} of $\dep$, denoted $\esch{\dep}$, is the set of all extensional predicates in $\dep$, while the {\em intentional
schema} of $\dep$, denoted $\isch{\dep}$, is the set of all intensional predicates in $\dep$. Note that, by definition, $\esch{\dep} \cap \isch{\dep} = \emptyset$. The {\em schema} of $\dep$, denoted $\sch{\dep}$, is the set $\esch{\dep} \cup \isch{\dep}$, which is in general a subset of $\ins{S}$ since some predicates of $\ins{S}$ may not appear in $\dep$.


\medskip
\noindent
\textbf{Semantics of Datalog Programs.}
The semantics of Datalog programs can be equivalently defined in three different ways: model-theoretically, via a fixpoint procedure, and proof-theoretically; see, e.g.,~\cite{AbHV95}. We proceed to recall the proof-theoretic semantics of Datalog programs. To this end, we need the key notion of proof tree of a fact, which will anyway play a crucial role in our work.
%
For a database $D$ and a Datalog program $\dep$, let $\base{D,\dep}$ be the set that collects 
%= \{R(\bar t) \mid R \in \sch{\dep} \text{ and } \bar t \in \adom{D}^{\arity{R}}\}$ that collects 
all the facts that can be formed using predicates of $\sch{\dep}$ and constants of $\adom{D}$.


\begin{definition}[\textbf{Proof Tree}]\label{def:proof-tree}
	Consider a Datalog program $\dep$, a database $D$ over $\esch{\dep}$, and a fact $\alpha$ over $\sch{\dep}$. 
	%
	A {\em proof tree of $\alpha$ w.r.t.~$D$ and $\dep$} is a finite labeled rooted tree $T=(V,E,\lambda)$, with $\lambda : V \ra \base{D,\dep}$, such that the following hold:
	\begin{enumerate}
		\item If $v \in V$ is the root, then $\lambda(v) = \alpha$.
		
		\item If $v \in V$ is a leaf, then $\lambda(v) \in D$.
		
		\item If $v \in V$ has $n\ge1$ children $u_1,\ldots,u_n$, then there exists a rule $R_0(\bar x_0)\ \assign\ R_1(\bar x_1),\ldots,R_n(\bar x_n) \in \dep$ and a function $h : \bigcup_{i \in [n]} \bar x_i \ra \ins{C}$ such that $\lambda(v) = R_0(h(\bar x_0))$, and $\lambda(u_i) = R_i(h(\bar x_i))$ for each $i \in [n]$. \hfill\markfull
	\end{enumerate} 
\end{definition}


Essentially, a proof tree of a fact $\alpha$ w.r.t.~$D$ and $\dep$ indicates that we can prove $\alpha$ using $D$ and $\dep$, i.e., we can derive $\alpha$ starting from $D$ end executing the rules of $\dep$. Here is a simple example from~\cite{CLPS24}.


\begin{example}\label{exa:proof-tree}
	Consider the Datalog program $\dep$ consisting of
	\[
	A(x)\ \assign\ S(x) \quad \text{ and } \quad A(x)\ \assign\ A(y), A(z),T(y,z,x)
	\]
	that encodes the {\em path accessibility problem}~\cite{Cook74}. The predicate $S$ represents source nodes, $A$ represents nodes that are accessible from the source nodes, and $T$ represents accessibility conditions, that is, $T(y,z,x)$ means that if both $y$ and $z$ are accessible from the source nodes, then so is $x$.
	%
	Let also
	\[
	D\ =\ \{S(a), T(a,a,b),T(a,a,c), T(a,a,d), T(b,c,a)\}.
	\]
	A simple proof tree of the fact $A(d)$ w.r.t.~$D$ and $\dep$ follows:
	
	\centerline{\includegraphics[width=.24\textwidth]{proof-tree-1.pdf}}
	
	\noindent The following is another, slightly more complex, proof tree of the fact $A(d)$ w.r.t.~$D$ and $\dep$:
	
	\centerline{
	\includegraphics[width=.46\textwidth]{proof-tree-2.pdf}}

	\noindent Note that the above are only two out of the many proof trees of $A(d)$ w.r.t.~$D$ and $\dep$. In fact, there are infinitely many as one can build larger and larger such proof trees: whenever we encounter a node labeled by $A(a)$, we can choose to apply the recursive rule $A(x)\ \assign\ A(y), A(z),T(y,z,x)$. \hfill\markfull
\end{example}


Now, given a Datalog program $\dep$ and a database $D$ over $\sch{\dep}$, the {\em semantics of $\dep$ on $D$} is the set
\[
\dep(D)\ =\ \{\alpha \mid \text{ there is a proof tree of } \alpha \text{ w.r.t. } D \text{ and } \dep\},
\]
that is, the set of facts that can be proven using $D$ and $\dep$.


\medskip
\noindent
\textbf{Datalog Queries.} Having the syntax and the semantics of Datalog programs in place, it is now straightforward to recall the syntax and the semantics of Datalog queries.
%
A {\em Datalog query} is a pair $Q = (\dep,R)$, where $\dep$ is a Datalog program and $R$ a predicate of $\isch{\dep}$.
%
Now, for a database $D$ over $\esch{\dep}$, the {\em answer} to $Q$ over $D$ is defined as the set of tuples
\[
Q(D)\ =\ \left\{\bar t \in \adom{D}^{\arity{R}} \mid R(\bar t) \in \dep(D)\right\},
\]
i.e., all those tuples $\bar t$ such that the fact $R(\bar t)$ can be proven using $D$ and $\dep$. The class of all the Datalog queries is denoted $\DAT$. 

==> figures/ratios-results.tex <==
\begin{figure*}[t]
\centering
\small

\begin{subfigure}[t]{0.36\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/rate-csda-httpd-arbitrary-hypergraph.pdf}
    \caption{\arbitrary, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/rate-csda-httpd-unambigous-hypergraph.pdf}
    \caption{\unambiguous, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/rate-csda-httpd-unambigous-dag.pdf}
    \caption{\unambiguous, \dagEnc}
\end{subfigure}

\caption{Ratio (optimal / greedy) distribution across $k$ for the \httpd\ dataset under the \csda\ scenario.}
\label{fig:csda-httpd-rate}
\end{figure*}


\begin{figure*}[t]
\centering
\small

\begin{subfigure}[t]{0.36\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/rate-csda-linux-arbitrary-hypergraph.pdf}
    \caption{\arbitrary, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/rate-csda-linux-unambigous-hypergraph.pdf}
    \caption{\unambiguous, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/rate-csda-linux-unambigous-dag.pdf}
    \caption{\unambiguous, \dagEnc}
\end{subfigure}

\caption{Ratio (optimal / greedy) distribution across $k$ for the \linux\ dataset under the \csda\ scenario.}
\label{fig:csda-linux-rate}
\end{figure*}


\begin{figure*}[t]
\centering
\small

\begin{subfigure}[t]{0.36\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/rate-csda-postgresql-arbitrary-hypergraph.pdf}
    \caption{\arbitrary, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/rate-csda-postgresql-unambigous-hypergraph.pdf}
    \caption{\unambiguous, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/rate-csda-postgresql-unambigous-dag.pdf}
    \caption{\unambiguous, \dagEnc}
\end{subfigure}

\caption{Ratio (optimal / greedy) distribution across $k$ for the \postgres\ dataset under the \csda\ scenario.}
\label{fig:csda-postgresql-rate}
\end{figure*}


\begin{figure*}[t]
\centering
\small

\begin{subfigure}[t]{0.36\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/rate-graph_analytics-facebook-arbitrary-hypergraph.pdf}
    \caption{\arbitrary, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/rate-graph_analytics-facebook-unambigous-hypergraph.pdf}
    \caption{\unambiguous, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/rate-graph_analytics-facebook-unambigous-dag.pdf}
    \caption{\unambiguous, \dagEnc}
\end{subfigure}

\caption{Ratio (optimal / greedy) distribution across $k$ for the \facebook\ dataset under the \graphanalytics\ scenario.}
\label{fig:graphanalytics-facebook-rate}
\end{figure*}


\begin{figure*}[t]
\centering
\small

\begin{subfigure}[t]{0.36\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/rate-graph_analytics-bitcoin-arbitrary-hypergraph.pdf}
    \caption{\arbitrary, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/rate-graph_analytics-bitcoin-unambigous-hypergraph.pdf}
    \caption{\unambiguous, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/rate-graph_analytics-bitcoin-unambigous-dag.pdf}
    \caption{\unambiguous, \dagEnc}
\end{subfigure}

\caption{Ratio (optimal / greedy) distribution across $k$ for the \bitcoin\ dataset under the \graphanalytics\ scenario.}
\label{fig:graphanalytics-bitcoin-rate}
\end{figure*}





\begin{figure*}[t]
\centering
\small

\begin{subfigure}[t]{0.36\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/rate-galen-40-arbitrary-hypergraph.pdf}
    \caption{\arbitrary, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/rate-galen-40-unambigous-hypergraph.pdf}
    \caption{\unambiguous, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/rate-galen-40-unambigous-dag.pdf}
    \caption{\unambiguous, \dagEnc}
\end{subfigure}

\caption{Ratio (optimal / greedy) distribution across $k$ for the 40 dataset under the \galen\ scenario.}
\label{fig:galen-40-rate}
\end{figure*}


\begin{figure*}[t]
\centering
\small

\begin{subfigure}[t]{0.36\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/rate-galen-50-arbitrary-hypergraph.pdf}
    \caption{\arbitrary, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/rate-galen-50-unambigous-hypergraph.pdf}
    \caption{\unambiguous, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/rate-galen-50-unambigous-dag.pdf}
    \caption{\unambiguous, \dagEnc}
\end{subfigure}

\caption{Ratio (optimal / greedy) distribution across $k$ for the 50 dataset under the \galen\ scenario.}
\label{fig:galen-50-rate}
\end{figure*}


\begin{figure*}[t]
\centering
\small

\begin{subfigure}[t]{0.36\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/rate-doctors_q01-100k-arbitrary-hypergraph.pdf}
    \caption{\arbitrary, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/rate-doctors_q01-100k-unambigous-hypergraph.pdf}
    \caption{\unambiguous, \hypergraph}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \safeincludegraphics[height=4.8cm]{figures/rate-doctors_q01-100k-unambigous-dag.pdf}
    \caption{\unambiguous, \dagEnc}
\end{subfigure}

\caption{Ratio (optimal / greedy) distribution across $k$ for the 100k dataset under the \doctors\ scenario.}
\label{fig:doctors-100k-rate}
\end{figure*}

==> figures/related-work.tex <==
1- Efficient provenance tracking for datalog using top-k queries
2- DIVERSITY OF ANSWERS TO CONJUNCTIVE QUERIES
3- Query Answering Under Volume-Based Diversity Functions
4- Query Refinement for Diverse Top-k Selection
5- Efficient provenance tracking for datalog using top-k queries


==> figures/why-provenance.tex <==
\section{Why-Provenance for Datalog}\label{sec:why-provenance}
%

Why-provenance is a standard way of explaining why a query result is obtained. It essentially collects all the subsets of the database that can be used as a whole to prove (or derive) a query result. We proceed to recall the details following~\cite{CLPS24}.
%
Given a proof tree $T = (V,E,\lambda)$ (of some fact w.r.t.~some database and Datalog program), the {\em support} of $T$ is the family of sets of atoms
\[
\support{T}\ =\ \left\{\lambda(v) \mid v \in V \text{ is a leaf of } T\right\},
\] 
i.e., the set of facts that label the leaves of the proof tree $T$. Note that $\support{T}$ is a subset of the underlying database since, by definition, the leaves of a proof tree are labeled with database atoms.
%
The formal definition of why-provenance follows.


\begin{definition}[\textbf{Why-Provenance for Datalog}]\label{def:why-provenance}
	Consider a Datalog query  $Q = (\dep,R)$, a database $D$ over $\esch{\dep}$, and a tuple $\bar t \in \adom{D}^{\arity{R}}$. The {\em why-provenance of $\bar t$ w.r.t.~$D$ and $Q$} is defined as the family of sets of facts 
	\[
	\{\support{T} \mid T \text{ is a proof tree of } R(\bar t) \text{ w.r.t. } D \text{ and } \dep\}
	\]
	which we denote by $\why{\bar t}{D}{Q}$. \hfill\markfull
\end{definition}

 
Intuitively, a set of facts $D' \subseteq D$ from $\why{\bar t}{D}{Q}$ should be understood as a ``real'' reason why the tuple $\bar t$ is an answer to the query $Q$ over $D$, i.e., $D'$ explains why $\bar t \in Q(D)$. By ``real'' we mean that all the facts of $D'$ are really used in order to derive the tuple $\bar t$ as an answer. Here is a simple example of why-provenance.

\begin{example}\label{exa:why-provenance}
	Let $Q = (\dep,A)$, where $\dep$ is the program that encodes the path accessibility problem as in Example~\ref{exa:proof-tree}, and let $D$ be the database from Example~\ref{exa:proof-tree}. 
	%
	It is easy to verify that the why-provenance of the unary tuple $(d)$ w.r.t.~$D$ and $Q$ consists of $\{S(a), T(a,a,d)\}$ and the database $D$ itself. The former set is actually the support of the first proof tree given in Example~\ref{exa:proof-tree}, while $D$ is the support of the second proof tree. \hfill\markfull
\end{example}


\medskip
\noindent
\textbf{Refined Why-Provenance.} Although the notion of proof tree introduced above is the standard one used to define the notion of why-provennace for Datalog queries, it has been observed in the literature (see, e.g.,~\cite{BBPT22,CLPS24,CLPS24aaai}) that there are counterintuitive proof trees, which in turn lead to counterintuitive explanations based on why-provenance. Such a proof tree is the second one in Example~\ref{exa:proof-tree} that suffers from ``ambiguity''. In particular, there are two nodes labeled with $A(a)$, but their subtrees differ, which means that, according to the proof tree in question, it is ambiguous how $A(a)$ is derived starting from the database $D$. The above observation led to the class of unambiguous proof trees, which essentially forces a fact to be consistently proven via a certain derivation~\cite{CLPS24aaai}; 
see, e.g., the first proof tree in Example~\ref{exa:proof-tree}. To formalize this simple idea we need the notion of isomorphism among rooted trees.


Two rooted trees $T=(V,E,\lambda)$ and $T' = (V',E',\lambda')$ are {\em isomorphic}, denoted $T \eqtree T'$, if there is a bijection $h : V \ra V'$ such that, for each $v \in V$, $\lambda(v) = \lambda'(h(v))$, and for each $u,v \in V$, $(u,v) \in E$ iff $(h(u),h(v)) \in E'$. Let $T[v]$ be the subtree of the proof tree $T$ rooted at node $v$. The definition of unambiguous proof trees follows.


\begin{definition}[\textbf{Unambiguous Proof Tree}]\label{def:unambiguous-proof-tree}
	Consider a Datalog program $\dep$, a database $D$ over $\esch{\dep}$, and a fact $\alpha$. An {\em unambiguous proof tree of $\alpha$ w.r.t.~$D$ and $\dep$} is a proof tree $T = (V,E,\lambda)$ of $\alpha$ w.r.t.~$D$ and $\dep$ such that, for all $v,u \in V$, $\lambda(v) = \lambda(u)$ implies $T[v] \eqtree T[u]$. \hfill\markfull
\end{definition}


Having the notion of unambiguous proof tree in place, we can then refine the notion of why-provenance for Datalog queries by considering only unambiguous proof trees; the formal definition is omitted since it is identical to Definition~\ref{def:why-provenance} with the difference that we only collect the supports of unambiguous proof trees.
%
Given a Datalog query  $Q = (\dep,R)$, a database $D$ over $\esch{\dep}$, and a tuple $\bar t \in \adom{D}^{\arity{R}}$, we refer to the {\em why-provenance of $\bar t$ w.r.t.~$D$ and $Q$ relative to unambiguous proof trees}, denoted $\unwhy{\bar t}{D}{Q}$.
%
To be able to treat in a uniform way the notion of why-provenance relative to arbitrary proof trees (as given in Definition~\ref{def:why-provenance}) and the notion of why-provenance relative to unambiguous proof trees, in the rest of the paper we will write $\allwhy{\bar t}{D}{Q}$ instead of $\why{\bar t}{D}{Q}$ for the why-provenance of $\bar t$ w.r.t.~$D$ and $Q$.

At this point, let us clarify that why-provenance relative to unambiguous proof trees is indeed a refinement of why-provenance (relative to arbitrary proof trees). Indeed, given a Datalog query $Q = (\dep,R)$, a database $D$ over $\esch{\dep}$, and a tuple $\bar t \in \adom{D}^{\arity{R}}$, we have $\unwhy{\bar t}{D}{Q} \subseteq \allwhy{\bar t}{D}{Q}$.
%
Let us stress, however, that this is not the case when it comes to the semantics of Datalog. In other words, whenever there is a proof tree of a fact $\alpha$ w.r.t.~$D$ and $\dep$, then there is an unambiguous one. This is a desirable property since it implies the following: if $\bar t \in Q(D)$, then $\unwhy{\bar t}{D}{Q} \neq \emptyset$, which is what we expect from an explainability notion for Datalog.
